From Imitation to Refinement -- Residual RL for Precise Assembly

Recent advances in Behavior Cloning (BC) have made it easy to teach robots new tasks. However, we find that the ease of teaching comes at the cost of unreliable performance that saturates with increasing data for tasks requiring precision. The performance saturation can be attributed to two critical factors: (a) distribution shift resulting from the use of offline data and (b) the lack of closed-loop corrective control caused by action chucking (predicting a set of future actions executed open-loop) critical for BC performance. Our key insight is that by predicting action chunks, BC policies function more like trajectory "planners" than closed-loop controllers necessary for reliable execution. To address these challenges, we devise a simple yet effective method, ResiP (Residual for Precise Manipulation), that overcomes the reliability problem while retaining BC's ease of teaching and long-horizon capabilities. ResiP augments a frozen, chunked BC model with a fully closed-loop residual policy trained with reinforcement learning (RL) that addresses distribution shifts and introduces closed-loop corrections over open-loop execution of action chunks predicted by the BC trajectory planner. Videos, code, and data: https://residual-assembly.github.io.

==> Archive/conclusion.tex <==
% \section{Limitations and Conclusion}


==> Archive/experiment.tex <==
\section{Experimental Results}
\label{sec:experiments}

Our experimental evaluation focuses on three key aspects. First, we analyze how augmenting a behavior-cloned policy with residual RL enables reliable execution of precision-critical manipulation tasks (\autoref{sec:experiments-fine-tuning}). Second, through ablation studies, we identify design choices crucial for \methodname{}'s performance gains (\autoref{sec:resip-ablations}). Finally, we evaluate our method on physical robot hardware (\autoref{sec:experiments-real-world}), demonstrating improved real-world performance through teacher-student distillation, while identifying key bottlenecks in the policy distillation process.

\subsection{Augmenting Trajectory Planning with Reactive Control}
\label{sec:experiments-fine-tuning}
In simulation experiments, we first evaluate the fundamental limitations of state-of-the-art BC methods on precision-critical tasks. Using a suite of 6 assembly tasks and 50 demonstrations per task, we find that the Diffusion Policy (DP) architecture struggles with high-precision requirements. For example, in the \peghole{} task with 0.2mm clearance, DP achieves only a 5\% success rate despite the task's relatively short horizon of 100 timesteps.

\pulkit{Build up the story -- say one might think one can improve performance with data -- we did that -- here is the result, then one might think distribution shift is the issue -- we did that -- here is the result and so on..}

Our residual learning approach, \methodname{}, significantly improves upon these baseline results. Using the same 50 demonstrations per task, \methodname{} achieves consistent performance gains across all precision-critical scenarios: success rates in the \peghole{} task improve from 5\% to 99\%, while the \oneleg{} task shows improvements from 54\% to 98\%. These gains substantially outperform alternative RL approaches: directly fine-tuning the base MLP-C policy with PPO achieves 70\% success on \oneleg{}, while IDQL~\cite{hansen-estruch_idql_2023} reaches 57\%. \autoref{tab:performance_comparison} provides a complete comparison across our task suite, consistently showing \methodname{}'s strong performance compared to both BC baselines and the alternative RL-based approaches considered \pulkit{Trying to say too many things here-- I am not sure what is the MLP-C policy comparison buying here? What is the context of IDQL comparison?}.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/round_table_failure_modes.pdf}
    \caption{A qualitative analysis of the failure modes between the pre-trained BC policy and the fine-tuned residual policy for the \roundtable{} task on medium randomness. For the pre-trained policy, a large portion of the failures (40\%) relates to the table leg's insertion precision. In the fine-tuned policy, this share dropped to 0\%.}
    \label{fig:round-table-failure-modes}
    \vspace{-15pt}
\end{figure}

\subsubsection{Analyzing Failure Modes}
To understand where the large performance improvements stem from, we analyzed the common failure modes of the DP policies, shown in \autoref{fig:common-errors} and \autoref{fig:overview} (Left). In the low randomization setting, we observe that DP's failures primarily arise from small but imprecisions: a common error is pushing the leg down before achieving perfect alignment with the hole. Consequently, the object's pose shifts slightly in the gripper, causing an out-of-distribution grasp pose. The residual policy reliably corrects these errors through minimal adjustments---performing small sideways translations while avoiding premature downward motions, and typically only allowing insertion once proper alignment is achieved. We also find the residual policy makes subtle improvements to initial grasps that enable more precise downstream alignment between the grasped object and the receptacle.
%
Based on these observations, we posit that \methodname{}'s significant performance improvements stem from its ability to provide small but crucial adjustments---a natural fit for precision assembly tasks where minor misalignments often cause failure. While the base DP policy struggles with precise alignments and insertions, the learned residual component maintains proper alignment through minimal corrective actions.


However, even for our method, the performance saturates at 70\%-77\% in the medium randomization settings, where parts can be initially placed up to $\pm$5cm from their nominal positions. This drop in performance aligns with the intuition of the residual policy as a local correction mechanism that learns to make minor adjustments to the base DP policy's actions to improve precision and reactivity. When parts are placed far from their nominal positions, the DP policy may generate trajectories that deviate too far for the local correction mechanism to correct, leading failures not easily corrected. Even if the failures can be corrected, the resulting states may be out-of-distribution for the DP policy, making corrections infeasible.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/scaling_round_table.pdf}
    \caption{Scaling behavior comparison on the harder \roundtable{} task mirrors the trends observed for \oneleg{} (\autoref{fig:overview} (right)), but with lower overall performance. Just as in \oneleg{}, increasing the number of demonstrations for BC training leads to diminishing returns, saturating at 56\% success rate. While DAgger's online data collection performs better, it also plateaus at 71\%, well below \methodname{}'s 94\% success rate. This consistent pattern across tasks, with lower saturation points for the more complex tasks, highlights the limitations of offline approaches and the benefits of learning closed-loop control online.}
    \label{fig:scaling-round-table}
    \vspace{-15pt}
\end{figure}



To better understand the failure modes of DP and \methodname{} in this higher randomness setting, we manually analyzed 75 randomly sampled trajectories for the \roundtable{} task on medium randomness (see the \website{} for videos). We categorized the observed failures into four primary types:

\begin{enumerate}
    \item `Peg Precision' failures that occur during picking, inserting, or screwing operations with the table leg
    \item `Foot Precision' failures during similar operations with the foot
    \item `Out-of-Distribution' failures when parts are unreachable by the policy
    \item `Other' failures are attributed to contact-modeling issues in simulation (e.g., object penetration causing unrealistic accelerations) or timeout conditions.
\end{enumerate}

Our qualitative analysis of these failure modes and recovery behaviors for the \roundtable{} task, shown in \autoref{fig:round-table-failure-modes}, shows that \methodname{} significantly improves reliability during precise insertion phases compared to the baseline approach, and eliminates the precision errors for ``Peg Precision'' entirely but that the `Out-of-Distribution' increases in share.



Surprisingly, \methodname{} also leads to the emergence of qualitatively different behaviors compared to the nominal DP policy. We refer to the \website{}'s uncut videos of rollouts for both policies. In these videos, we observe that \methodname{} has discovered alternative grasping strategies not present in the demonstration data---while demonstrations only showed grasping the table foot from above its center, \methodname{} learned to grasp from the side when the center was unreachable. Additionally, \methodname{} exhibits more decisive recovery behaviors, making deliberate adjustments that lead to successful task completion where the nominal BC policy would ineffectively oscillate back and forth.




\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/online_perturbation_comparison.pdf}
    \caption{Performance robustness when introducing random force perturbations during evaluation. At each timestep, we randomly apply forces to the objects in the environment, simulating unexpected disturbances. Our method (\methodname{}), which makes per-timestep corrections, shows greater resilience with only a 12\% performance drop compared to nominal conditions. In contrast, chunk-based methods (DP, DP-DAgger, and \methodname{}-C) see larger drops of 19-26\%. This difference in robustness highlights the value of closed-loop control for handling dynamic disturbances not seen during training. All methods were evaluated across 1024 episodes, both with and without perturbations.}
    \label{fig:online_perturbation_comparison}
    \vspace{-15pt}
\end{figure}





\subsection{What drives performance of \methodname{}?}
\label{sec:resip-ablations}



This section investigates different aspects of \methodname{} that improves task performance: (1) training stability and sample efficiency across RL methods, (2) the impact of addressing distribution shift through online data collection, (3) the benefits of closed-loop control compared to chunk-based execution, and (4) robustness to dynamic perturbations.

\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{Training data} & \multicolumn{2}{c}{Corner} & \multicolumn{2}{c}{Grasp} & \multicolumn{2}{c}{Insert} & \multicolumn{2}{c}{Screw} & \multicolumn{2}{c}{Complete} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
     & Part & Obs & Part & Obs & Part & Obs & Part & Obs & Part & Obs \\
    \midrule
    10 Real-Only & 5/10 & 5/10 & 5/10 & 7/10 & 2/10 & 3/10 & 0/10 & 2/10 & 0/10 & 2/10 \\
    10 Real+Sim & 9/10 & 9/10 & 7/10 & 8/10 & 0/10 & 3/10 & 0/10 & 3/10 & 0/10 & 3/10 \\
    \addlinespace[.5ex]
    \hdashline
    \addlinespace[1ex]
    40 Real-Only & 10/10 & 8/10 & 9/10 & 8/10 & 6/10 & 3/10 & 2/10 & 3/10 & 2/10 & 3/10\\
    40 Real+Sim & 10/10 & 10/10 & 9/10 & 10/10 & 6/10 & 7/10 & 5/10 & 6/10 & 5/10 & 6/10\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparing the effect of combining real-world demonstrations with simulation trajectories from our RL-trained residual policies. Co-training with real and synthetic data improves motion quality and success rate on the \oneleg{} task.}
    \label{tab:real-world-real-cotrain}
    % \vspace{-15pt}
\end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_3.pdf}
    \caption{\textbf{(A)} Examples of successful real world assembly from RGB. Co-training with simulation data reduces jerkiness and improves insertion robustness by containing a higher diversity of part poses and insertion locations (see Table~\ref{tab:real-world-real-cotrain}). \textbf{(B)} Example failure: difficulty adjusting the insertion angle/position when grasps lead to unseen in-hand part poses.}
    \label{fig:real-world-sequences}
    \vspace{-15pt}
\end{figure*}



\subsubsection{Training Stability and Sample Efficiency}

In addition to improved success rates, we observed distinct training behavior and robustness across \methodname{}, direct MLP fine-tuning (PPO-C), and IDQL. First, direct chunked MLP fine-tuning (PPO-C) was unstable and required KL regularization to avoid collapse. In contrast, \methodname{} demonstrated robust training, allowing for several gradient steps for each collected trajectory, decreasing sample complexity. \methodname{} also performed well across a broad range of hyperparameters. Second, for IDQL, the base DP model produced actions with low variance even with $\eta=1$ in the Denoising Diffusion Implicit Model (DDIM) sampler~\cite{song2020denoising}---the iterative denoising procedure in diffusion models that converts noise into actions, where $\eta$ controls the stochasticity of this process. Despite setting this stochasticity parameter to its maximum value, the generated actions lacked sufficient exploration, which inhibited Q-learning and constrained the potential for policy improvement.

In contrast, \methodname{} training was very stable, as its architecture is naturally biased towards predicting small delta corrections to the base policy's poses rather than operating in the full workspace coordinate frame. This local prediction scope, combined with the residual network's small parameter count, prevents the large policy updates that typically destabilize deep RL training~\cite{kumar2020conservative, schulman2015trust}. This stability is demonstrated in \autoref{fig:alpha-ablation}, showing consistent learning across hyperparameters.




\subsubsection{Impact of Distribution Shift}

To probe the impact of mitigating distribution shift, we compared the baseline DP against DP-DAgger trained using online data collection via DAgger~\cite{ross2011_dagger} as described in \autoref{sec:baselines}. While DP-DAgger significantly outperforms the baseline DP (see yellow vs. red lines in \autoref{fig:overview} (right) and \autoref{fig:scaling-round-table}), it still trails \methodname{} (blue line) by 9\% and 23\% for the \oneleg{} and \roundtable{} tasks, respectively. The remaining performance gap suggests that reducing distribution shift with online data collection does not fully explain \methodname{}'s performance benefits.






\subsubsection{Impact of Closed-Loop Control}
\label{sec:closed-loop-results}

To quantify the benefits of per-timestep corrections, we compared \methodname{} against \methodname{}-C, which predicts corrections at the chunk level as described in \autoref{sec:closed-loop-ablation}. Our experiments reveal that chunk-level corrections lead to significantly slower learning progress, with \methodname{}-C requiring significantly more environment interactions to achieve comparable performance (\autoref{fig:chunked-residual-ablation} in \appref{app:closed-loop-ablation}). Moreover, even with extended training, \methodname{}-C's performance saturates at 92\% compared to \methodname{}'s 98\% on the \oneleg{} task. This performance gap suggests that the ability to make frequent corrections not only accelerates learning but also enables higher terminal performance.


\subsubsection{Robustness to Dynamic Perturbations} To further evaluate the benefits of closed-loop control, we compare the performance degradation of different methods under dynamic disturbances as described in \autoref{sec:evaluation-protocol}. As shown in \autoref{fig:online_perturbation_comparison}, methods using chunk-based execution---DP, DP-DAgger, and \methodname{}-C---experience significant performance drops of 19-26 percentage points under these perturbations. In contrast, \methodname{}, with its ability to make per-timestep corrections, maintains a more robust performance with only a 12\% drop. This substantial difference in robustness (7-14 percentage points) provides further evidence for the value of closed-loop control in precise manipulation tasks.





% ====== Start new distillation/real-world section ======
% \input{fig_text/real_results_table}

\subsection{Real-World Deployment}
\label{sec:experiments-real-world}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_Black_1.pdf}
    \caption{\textbf{(A)} When changing the part appearances from white to black, the policy trained on real data only (\textbf{Real-Only}) seizes to function. The behavior becomes erratic, and all trials ended with the robot hitting a velocity limit. \textbf{(B)} When mixing in synthetic data with more diverse colors (see \autoref{fig:synthetic-data}), the policy (\textbf{Real+Sim-DR}) regains the ability to complete the task, though with lower performance than for white parts.}
    \label{fig:real-black-parts}
    \vspace{-15pt}
\end{figure}



\subsubsection{Real-World Performance}


Our sim-to-real experiments, following the protocol described in \autoref{sec:evaluation-protocol}, demonstrate that \textbf{Real+Sim} policies achieve significantly higher success rates (50-60\%) compared to \textbf{Real-Only} baselines (20-30\%) on the \oneleg{} task (\autoref{tab:real-world-real-cotrain}).

Qualitatively, the co-trained policy exhibits smoother behavior with fewer erratic movements that exceed robot hardware limits. \autoref{fig:real-world-sequences} shows typical behaviors: Row (A) shows successful assembly sequences, while Row (B) demonstrates the primary failure mode---imprecise alignment before release, mirroring challenges observed in simulation.



To assess robustness to visual variations, we tested a variant where we changed part colors from the white used in data collection to an unseen black. Unsurprisingly, the \textbf{Real-Only} policy fails catastrophically, triggering velocity limits on every trial, as shown in \autoref{fig:real-black-parts} (A). In contrast, \textbf{Real+Sim-DR}, trained with the same real-world data but with color-randomized synthetic data (see \autoref{fig:real-black-parts}), maintains basic functionality though with reduced performance compared to the original color scheme. While highlighting the benefits of synthetic data augmentation, this also indicates opportunities for improving sim-to-real transfer. See \appref{app:experiments-real-world} for more detailed analysis.



\subsubsection{Understanding Performance Limitations}

To understand the gap between simulation and real-world performance, we hypothesize two potential limiting factors: the change from state- to vision-based policies and the policy distillation process. Comparative experiments between image and state-based students show similar performance gaps from the teacher's 98\% success rate (\autoref{fig:bc_vs_rl_distillation}), suggesting the bottleneck lies in the distillation process rather than the change of observation modality from state to vision-based. Our scaling analysis further supports this hypothesis: even increasing synthetic trajectories from 10k to 100k only marginally improves success rates from 78\% to 80\% (\autoref{fig:overview}; right). These results indicate fundamental limitations in the policy distillation process that encourages investigations into leveraging online learning and closed-loop control better for vision-based policies. See \appref{app:distillation-analysis} for detailed analysis.





\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/distillation.pdf}
    \caption{A comparison of performance between state and vision policies in policy distillation. The Diffusion Policy (DP) baseline achieves similar performance with both state and vision inputs when trained directly on the same 50 demonstrations (left), indicating that the vision modality does not inherently limit performance. However, we observe a significant performance gap when distilling our state-based \methodname{} policy into a vision-based policy (right). This consistent performance gap suggests the challenge lies in the distillation process rather than the vision modality, as direct vision-based training shows no such degradation.}
    \label{fig:bc_vs_rl_distillation}
    \vspace{-15pt}
\end{figure}






==> Archive/experiment_old.tex <==
% \vspace{-5pt}
\section{Experimental Results}
\label{sec:experiments}

% \lars{Ensure this reflects the actual contents of the experiments: i.e., the first section presenting results in simulation and the second section everything regarding sim-to-real (distillation included here).}

% First, we investigate the requirement of complex BC methods \pulkit{what is complex BC methods?} and the impact of our residual reinforcement learning approach on improving the success rates of policies trained with behavior cloning in \autoref{sec:experiments-fine-tuning}. Next, we study the performance of downstream distillation from synthetic RL data, examining the relationship between the quantity and quality of the data and the resulting performance of the distilled vision-based policies in \autoref{sec:experiments-distillation-scaling} \pulkit{Not sure what we want to say here}. Finally, we evaluate our method in the real world \autoref{sec:experiments-real-world}.

Our experimental evaluation focuses on two key aspects. First, we analyze how augmenting a behavior-cloned policy with a residual RL component enables reliable execution of precise manipulation tasks \autoref{sec:experiments-fine-tuning}. Then, we demonstrate the practical applicability of our method by transferring these policies to real-world hardware through a simple combination of synthetic data generation and co-training with real demonstrations in \autoref{sec:experiments-real-world}.


% \paragraph{Evaluation protocol}
% %
% We evaluate all methods by executing the policy from an initial state sampled from the same initial state distribution for collecting demonstrations. We follow the default randomization protocol used in FurnitureBench~\cite{heo_furniturebench_2023}: at the beginning of every episode, objects are randomly offset from their nominal positions by $\Delta x, \Delta y \in [-1.5, 1.5]$ cm in the horizontal plane (with fixed height $z$) for low randomization settings and by $\Delta x, \Delta y \in [-5, 5]$ cm for medium randomization. For the U-shaped fixture used to stabilize parts during assembly (the three-sided white ``wall'' surrounding the parts in the left-most three columns in \autoref{fig:task-overview}), we apply additional offsets of $\Delta x, \Delta y \in [-2, 2]$ cm and $\Delta x, \Delta y \in [-4, 4]$ cm from its nominal position for low and medium settings respectively. The success rate is calculated as the average success over 1024 rollouts. The training data for human demonstrations and online RL is generated with the same initial state distribution.

\subsection{Augmenting Trajectory Planning with Reactive Control}
\label{sec:experiments-fine-tuning}

% \paragraph{Why Action Chunking and Diffusion Policies?}

% Simple feed-forward MLPs of modest size have shown impressive performance in many domains when trained with RL~\cite{kumar2021rma,lee2020learning,torne2024reconciling_rialto}, and offer a natural starting point for RL fine-tuning after BC pre-training. However, the standard MLP policies trained to directly output single action control instead of a trajectory plan through an action chunk (MLP-S) fail across all tasks we consider. Therefore, we also trained MLP policies with action chunking (MLP-C). When we introduce chunking, MLP performance improves drastically, as shown in \autoref{tab:performance_comparison}. However, we also find that the more complex Diffusion Policy (DP) architecture generally outperforms MLPs, especially in tasks of intermediate difficulty. For example, an improvement from 10\% success rate to 26\% for the \oneleg{} task on medium randomness makes subsequent fine-tuning far easier.

% In one case, \lamp{} on low randomness, MLP-C outperformed DP. In qualitative evaluations, we find that DP has smoother and faster actions, which is generally beneficial. Still, it seems to hurt performance in this case, as it tends to retract before the gripper fully grasps the lamp base. We also find that all methods struggle with the most challenging tasks, on which MLP-C and DP both achieve less than 5\% success rate, indicating that there is still room for improvement in BC methods. The \peghole{} task, despite its relatively short horizon of $\sim$100 timesteps, proved particularly challenging for BC methods. This task involves a $\sim$0.2 mm tolerance insertion, resulting in a 5\% success rate. This poor performance on a short yet precise task lends credence to the hypothesis that BC methods are ill-equipped to handle high-precision requirements.


% Another interesting finding is that the DP is significantly more robust to noise, an important property for an adequate base policy for residual fine-tuning. In contrast, we observed performance collapse when using MLP-C as the base, further reinforcing the utility of using powerful generative models for BC pre-training. See more analysis in \appref{app:residual-base-ablation}.




\paragraph{Online Policy Fine-Tuning Comparison}

Our experiments employ the Diffusion Policy (DP) architecture as the base BC policy, as we find it provides more robust and reliable behavior compared to simpler architectures (detailed analysis in \appref{app:residual-base-ablation}). The base DP policy crucially achieves nonzero success on our manipulation tasks but struggles with high-precision requirements---for instance, achieving only a 5\% success rate on a sub-millimeter tolerance insertion task despite its relatively short horizon.

We investigate the effectiveness of our residual RL approach, \methodname{}, in improving the performance of policies trained with BC. We train residual policies using PPO~\cite{schulman_proximal_2017} on top of the diffusion policy and compare it to two baselines---(1) directly fine-tune the MLP-C with PPO while regarding every action chunk as one concatenated action and (2) a chunked version of the IDQL algorithm~\cite{hansen-estruch_idql_2023}. In the IDQL algorithm, multiple action chunks are sampled from the diffusion policy, and the action chunk to execute is chosen based on its Q-value. We have found that learning a good Q-value estimator from offline data alone, as proposed in IDQL, is challenging with only 50 demonstrations. Therefore, we learn it in on-policy matter similar to~\cite{shenfeld2024value}.

The results in \autoref{tab:performance_comparison} show that our residual RL approach significantly improves success rates over BC and outperforms alternative RL fine-tuning methods. For tasks with lower initial randomization, such as the \oneleg{} task, the residual policy increases the success rate from 54\% to 98\%.
%
Even more drastically, for the \peghole{} task, \methodname{} improved the success rate from 5\% to 99\%.

However, even for our method, the performance saturates at 70\%-77\% in the medium randomization settings, where parts can be initially placed up to $\pm$5cm from their nominal positions. This drop in performance aligns with our intuition of the residual policy as a local correction mechanism that learns to make minor adjustments to the base BC policy's actions to improve precision and reactivity. When parts are placed far from their nominal positions, the BC policy may generate trajectories that deviate too far for the local correction mechanism to correct, leading to more failures.

We show some qualitative examples of the most common failure modes of the BC policies in \autoref{fig:common-errors} and \autoref{fig:overview} (Left).
%
For instance, a typical error mode of the BC policy is pushing down the leg before it is aligned with the hole. Consequently, the object's pose changes in the gripper, causing the policy to diverge due to the out-of-distribution grasp pose.
%
The residual policy reliably corrects these errors by performing small sideways translations while avoiding premature downward motions. It typically only allows the leg to be inserted once it is appropriately above the hole.
%
We also find the residual policy is better at performing initial grasps that allow accurate downstream alignment between the grasped object and the receptacle. On the other hand, the BC policies more often grasp the object at angles that make insertion more difficult.
%
% In \autoref{fig:round-table-failure-modes}, we qualitatively analyze this \pulkit{what does "this" refer to?} for the \roundtable{} task and find that the residual \pulkit{use the name of our method \methodname{}} makes the precise insertion part of the task significantly more reliable. To understand failure modes of \methodname{}(see the \website{} for videos), we manually categorized 75 randomly sampled failures into three categories: `Peg Precision' failures occur while picking, inserting, or screwing the table leg, `Foot Precision' failures occur during same operations with the foot, and `Out-of-Distribution' failures occur when parts are unreachable by the policy. The remaining failures are attributed to simulation issues \pulkit{what kind of simulation issues?} or timeouts.

To understand failure modes of \methodname{}, we manually analyzed 75 randomly sampled trajectories (see the \website{} for videos). We categorized the observed failures into three primary types: `Peg Precision' failures that occur during picking, inserting, or screwing operations with the table leg; `Foot Precision' failures during similar operations with the foot; and `Out-of-Distribution' failures when parts are unreachable by the policy. The remaining failures were attributed to contact-modeling issues in simulation (e.g., object penetration causing unrealistic accelerations) or timeout conditions. Our qualitative analysis of these failure modes and recovery behaviors for the \roundtable{} task, shown in \autoref{fig:round-table-failure-modes}, shows that \methodname{} significantly improves reliability during precise insertion phases compared to the baseline approach, and eliminates the precision errors for the first task phase (leg precision).


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/BCFailRLSucc_V2.png}
    \caption{Examples of the common failures made by BC policies in tasks requiring precise part alignments. These failures can be mitigated by small corrections, making our residual framework, \methodname{}, well-suited to improve the reliability of the nominal BC policy.}
    \label{fig:common-errors}
    \vspace{-15pt}
\end{figure}

% Surprisingly, the residual RL procedure also leads to the emergence of qualitatively different behaviors. We refer to the \href{https://residual-assembly.github.io/}{website}'s uncut videos of rollouts for the pre-trained and fine-tuned policies \pulkit{What do we mean by pre-trained and fine-tuned policies}. In these videos, we observe that the fine-tuned policy \pulkit{Fine-tuning is not the appropriate word -- let's call it nominal BC policy, and \methodname{} policy} has learned new grasps of the table foot that were not demonstrated \pulkit{what do we mean by new grasp?}, as well as more persistent retrying behavior and recovery.

Surprisingly, \methodname{} also leads to the emergence of qualitatively different behaviors compared to the nominal BC policy (DP). We refer to the \href{https://residual-assembly.github.io/}{website}'s uncut videos of rollouts for both policies. In these videos, we observe that \methodname{} has discovered alternative grasping strategies not present in the demonstration data---while demonstrations only showed grasping the table foot from above its center, \methodname{} learned to grasp from the side when the center was unreachable. Additionally, \methodname{} exhibits more decisive recovery behaviors, making deliberate adjustments that lead to successful task completion where the nominal BC policy would ineffectively oscillate back and forth.

% In addition to improved success rates, we observed different training dynamics \pulkit{what do we mean by training dynamics?} across each method \pulkit{which methods?}.
%
% First, direct MLP-C fine-tuning (PPO-C) proved unstable and required KL-regularization to avoid collapse. Second, the trained DP produced actions with low variance, even with $\eta=1$ in the DDIM \pulkit{what is DDIM -- tell the full name and what it does at least intuitively} sampler~\cite{song2020denoising}, inhibiting Q-learning and constraining the potential for policy improvement.

In addition to improved success rates, we observed distinct training behavior and robustness across \methodname{}, direct MLP fine-tuning (PPO-C), and IDQL. First, direct chunked MLP fine-tuning (PPO-C) was unstable and required KL regularization to avoid collapse. In contrast, \methodname{} demonstrated robust training, tolerating high update-to-data ratios without performance degradation and performing well across a broad range of hyperparameters. Second, for IDQL, the base DP model produced actions with low variance even with $\eta=1$ in the Denoising Diffusion Implicit Model (DDIM) sampler~\cite{song2020denoising}---the iterative denoising procedure in diffusion models that converts noise into actions, where $\eta$ controls the stochasticity of this process. Despite setting this stochasticity parameter to its maximum value, the generated actions lacked sufficient exploration, which inhibited Q-learning and constrained the potential for policy improvement.

% Finally, residual policy training was very stable, likely because it is constrained to operate on a local scale \pulkit{how is this constrain imposed?}, which prevents large deviations that can make RL unstable and has a small parameter count compared to the base policy~\cite{kumar2020conservative, schulman2015trust} \pulkit{Why cite CQL or TRPO here?}. \pulkit{Are there any plots in the Appendix that show this?}

In contrast, \methodname{} training was very stable, as its architecture naturally constrains it to predict small delta corrections to the base policy's poses rather than operating in the full workspace coordinate frame. This local prediction scope, combined with the residual network's small parameter count, prevents the large policy updates that typically destabilize deep RL training~\cite{kumar2020conservative, schulman2015trust}. This stability is demonstrated in \autoref{fig:alpha-ablation}, showing consistent learning across hyperparameters.



\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/round_table_failure_modes.pdf}
    \caption{A qualitative analysis of the failure modes between the pre-trained BC policy and the fine-tuned residual policy for the \roundtable{} task on medium randomness. For the pre-trained policy, a large portion of the failures (40\%) relates to the table leg's insertion precision. In the fine-tuned policy, this share dropped to 0\%.}
    \label{fig:round-table-failure-modes}
    \vspace{-15pt}
\end{figure}


\paragraph{What drives performance of \methodname{}?}

We hypothesized that the performance of BC could be improved by training on policy and by training a closed-loop reactive component. We analyzed these factors in improving the performance of \methodname{} over the nominal BC policy. 
%To understand the contribution of what drives the residual RL fine-tuning approach's performance, we try to decompose it into an on-policy component and a closed-loop, reactive component.

% To probe the impact of on-policy learning, we compared the performance of policies trained with the same amount of data gathered offline versus online using DAgger~\cite{ross2011_dagger} from an expert policy. \pulkit{How do we get the expert to apply DAGGER}. Unsurprisingly, a DAgger-trained policy performs significantly better than a policy trained with offline data, as reported in \autoref{fig:overview} (right) and \autoref{fig:scaling-round-table}. However, on-policy training doesn't fully explain the performance benefits enjoyed by \methodname{} and trails by 9\% and 23\% for the \oneleg{} and \roundtable{} tasks, respectively.

To probe the impact of on-policy learning, we compared policies trained with offline data versus online data collected via DAgger~\cite{ross2011_dagger}. For this experiment, we used \methodname{} as the expert policy for DAgger, as it achieves near-perfect success rates. While the DAgger-trained policy significantly outperforms the offline-trained policy (see yellow vs. red lines in \autoref{fig:overview} (right) and \autoref{fig:scaling-round-table}), it still trails \methodname{} (blue line) by 9\% and 23\% for the \oneleg{} and \roundtable{} tasks, respectively. This under-performance suggests that on-policy learning alone does not fully explain \methodname{}'s performance benefits and highlights a practical limitation of DAgger: it requires access to an expert policy, creating a circular dependency in many applications.


% On the other hand, we also find the residual policy's closed-loop, single-step nature helpful \pulkit{What is the significance of single-step nature?}. First, when trying to learn a residual policy for whole chunks \pulkit{What does this mean? Predicting the residual for the entire chunk, instead of per action?}, the resulting policy learns significantly more slowly, and the performance saturates at a lower level than that of the full closed-loop policy \pulkit{good to give a sense of how much lower}. See \appref{app:closed-loop-ablation} for details.

We also find the residual policy's closed-loop, per-timestep correction nature helpful. While the base BC model predicts action chunks, \methodname{} provides corrections at every timestep. When we instead implement an ablated version (\methodname{}-C) that predicts corrections at the same chunk-level frequency as the base policy, the resulting policy learns significantly more slowly, and performance saturates at 92\% compared to \methodname{}'s 98\%. See \appref{app:closed-loop-ablation} for details.

% To further probe the value of closed-loop control, we conduct an experiment where random force perturbations are applied during execution, introducing dynamic disturbances not seen during training. As shown in \autoref{fig:online_perturbation_comparison}, our per-timestep approach maintains robust performance with only a 12\% drop under perturbations, while methods executing actions in chunks suffer more significant degradation. This includes both the pre-trained BC and DAgger policies and an ablated version of our method that predicts residuals \pulkit{Its good to give names to method -- e.g., \methodname{}, \methodname{}-chunked and call by them -- its much easier to follow, otherwise its quite confusing} for entire chunks rather than individual timesteps, all of which drop 19-26 percentage points from their nominal performance. These results demonstrate the importance of frequency close-loop corrections for handling unexpected and dynamic disturbances.

To further probe the value of closed-loop control, we conduct an experiment where random force perturbations are applied during execution, introducing dynamic disturbances not seen during training. As shown in \autoref{fig:online_perturbation_comparison}, \methodname{} maintains robust performance with a 12\% drop under perturbations, while action-chunked methods suffer more significant degradation. Specifically, the nominal BC policy (DP), DAgger policy, and \methodname{}-C (our method modified to predict chunk-level residuals) drop 19-26 percentage points from their nominal performance. These results demonstrate the importance of frequent closed-loop corrections for handling unexpected and dynamic disturbances.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/online_perturbation_comparison.pdf}
    \caption{Performance robustness when introducing random force perturbations during evaluation. Our method (\methodname{}), which makes per-timestep corrections, shows greater resilience with only a 12\% performance drop compared to nominal conditions. In contrast, methods executing actions in chunks (including an ablation of our method that learns to predict residuals for entire chunks with online RL) see larger drops of 19-26\%. This difference highlights the value of closed-loop control for handling dynamic disturbances. See \appref{app:closed-loop-ablation} for details.}
    \label{fig:online_perturbation_comparison}
    \vspace{-15pt}
\end{figure}


The Diffusion Policy (DP) demonstrates significantly greater robustness to noise compared to the chunked MLP-C, making it particularly well-suited as a base policy for residual RL fine-tuning. While using DP as the base policy leads to stable performance improvements during training, attempting the same residual learning with MLP-C results in performance collapse. \autoref{fig:residual-base-ablation} shows that using a pre-trained ACT model~\cite{zhao_rss23_aloha} as the base achieves similar training stability to DP, reinforcing the advantages of using powerful generative models for BC pre-training. See \appref{app:residual-base-ablation} for further analysis.








% ====== Start new distillation/real-world section ======

\subsection{Real-World Deployment}
\label{sec:experiments-real-world}
\input{fig_text/real_results_table}

To deploy our policies on physical hardware, we apply a simple teacher-student policy distillation approach combining synthetic data generation with real-world demonstrations~\cite{chen2023visual, kumar2021rma, shenfeld2023tgrl, chen2020learning, torne2024reconciling_rialto} (\autoref{fig:pipeline}). Our strategy involves collecting successful trajectories from the \methodname{} teacher across varied initial states, rendering these with photorealistic cameras in IsaacSim~\cite{mittal2023orbit}, and co-training with a small set of real demonstrations.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/distillation.pdf}
    \caption{A comparison of performance between state and vision policies in policy distillation. The Diffusion Policy (DP) baseline achieves similar performance with both state and vision inputs when trained directly on the same 50 demonstrations (left), indicating that the vision modality does not inherently limit performance. However, we observe a significant performance gap when distilling our state-based \methodname{} policy into a vision-based policy (right). This consistent performance gap suggests the challenge lies in the distillation process rather than the vision modality, as direct vision-based training shows no such degradation.}
    \label{fig:bc_vs_rl_distillation}
    \vspace{-15pt}
\end{figure}



To assess the transferability of our RL-learned behaviors before real-world deployment, we first conduct experiments in simulation comparing different policy distillation approaches. A vision-based policy distilled from $\sim$1,000 synthetic trajectories achieves 73\% success on \oneleg{}, significantly outperforming the 50\% baseline when training directly on human demonstrations (see \autoref{fig:bc_vs_rl_distillation}). While this shows the benefit of distilling from our RL expert, a performance gap remains from the teacher's 98\% success rate. Comparative experiments between image and state-based students yield similar performance gaps, suggesting the bottleneck lies in the distillation process rather than the visual modality. This hypothesis is further supported by our scaling experiments with state-based students: increasing synthetic trajectories from 10k to 100k only marginally improves success rates from 78\% to 80\% (\autoref{fig:overview}; right), indicating that simply adding more data does not bridge the performance gap. See \appref{app:distillation-analysis} for detailed analysis.


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/scaling_round_table.pdf}
    \caption{Scaling behavior comparison on the harder \roundtable{} task mirrors the trends observed for \oneleg{} (\autoref{fig:overview} (right)), but with lower overall performance. Just as in \oneleg{}, increasing the number of demonstrations for BC training leads to diminishing returns, saturating at 56\% success rate. While DAgger's online data collection performs better, it also plateaus at 71\%, well below \methodname{}'s 94\% success rate. This consistent pattern across tasks, with lower saturation points for the more complex tasks, highlights the limitations of offline approaches and the benefits of learning closed-loop control online.}
    \label{fig:scaling-round-table}
    \vspace{-15pt}
\end{figure}



% Given these insights, we evaluate a pragmatic approach: co-training with synthetic data and a small set of real-world demonstrations (10/40 examples)~\cite{wang_poco_2024, torne2024reconciling_rialto}. We compare two variants: \textbf{Real+Sim} combines real demos with rendered synthetic data, while \textbf{Real-Only} uses just the real demonstrations. Results in \autoref{tab:real-world-real-cotrain} on the \oneleg{} task across randomized initial object poses and obstacle (white ``wall'' around the workspace) pose shows that incorporating simulation data improves real-world performance, increasing task completion from 20-30\% to 50-60\%.

Our simulation experiments demonstrate that distilling behaviors from our RL-trained expert significantly improves performance over learning from demonstrations alone. Next, we investigate deploying policies on physical hardware through the straightforward co-training approach outlined in \autoref{sec:sim-to-real-pipeline-method}, combining synthetic data with a small set of real-world demonstrations (10/40 examples)~\cite{wang_poco_2024, torne2024reconciling_rialto}. We compare two variants: \textbf{Real+Sim} combines real demos with rendered synthetic data, while \textbf{Real-Only} uses just the real demonstrations. Striving to perform similar randomization as our simulation experiments, we evaluate these policies on the \oneleg{} task across a grid of initial object and obstacle poses, matching the ranges used in our low randomization simulation setting. Results in \autoref{tab:real-world-real-cotrain} show that incorporating simulation data improves real-world performance, increasing task completion from 20-30\% to 50-60\%.


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/Synthetic_Data.pdf}
    \caption{Ephotorealistico-realistic rendering and domain randomization for sim-to-real transfer. In the first row, we show our nominal experiment setting of rendering parts in the original white color while varying the position, brightness, and hue of the lighting in the scene. In the bottom row, we also introduce variations in the part colors to see how that can help the final policy adapt to unseen part appearances without collecting any additional data.}
    \label{fig:synthetic-data}
    \vspace{-15pt}
\end{figure}

\input{fig_text/real_world_qual}


Qualitatively, the co-trained policy exhibits smoother behavior with fewer erratic movements that exceed robot hardware limits. \autoref{fig:real-world-sequences} shows typical behaviors: Row (A) shows successful assembly sequences, while Row (B) demonstrates the primary failure mode---imprecise alignment before release, mirroring challenges observed in simulation.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_Black_1.pdf}
    \caption{\textbf{(A)} When changing the part appearances from white to black, the policy trained on real data only (\textbf{Real-Only}) seizes to function. The behavior becomes erratic, and all trials ended with the robot hitting a velocity limit. \textbf{(B)} When mixing in synthetic data with more diverse colors (see \autoref{fig:synthetic-data}), the policy (\textbf{Real+Sim-DR}) regains the ability to complete the task, though with lower performance than for white parts.}
    \label{fig:real-black-parts}
    \vspace{-15pt}
\end{figure}

To assess robustness to visual variations, we tested a variant where part colors change from black to white. The \textbf{Real-Only} policy fails catastrophically, triggering velocity limits on every trial, as shown in \autoref{fig:real-black-parts} (A). In contrast, \textbf{Real+Sim-DR}, trained with color-randomized synthetic data (see \autoref{fig:real-black-parts}), maintains basic functionality though with reduced performance compared to the original color scheme. While highlighting the benefits of synthetic data augmentation, this also indicates opportunities for improving sim-to-real transfer. See \appref{app:experiments-real-world} for more detailed analysis.


% ====== End new distillation/real-world section ======






% ====== Start old distillation/real-world section ======

% \subsection{Training Vision Policies}
% \label{sec:experiments-distillation-scaling}


% \input{fig_text/real_results_table}


% \pulkit{There is too much emphasis on distillation -- why is that?}

% Next, we study how the quantity and quality of data generated by a \methodname{} policy impact the performance of vision-based student policies in real-world evaluations. We generate this data by collecting successful trajectories from the \methodname{} teacher across varied initial states and rendering corresponding camera observations. A vision-based student policy---which shares the same architecture as the teacher but includes an additional image encoder---distilled from $\sim$1,000 teacher trajectories reached 73\% success on \oneleg{}, outperforming the 50\% achieved by training the vision policy directly on human demos (see \autoref{fig:bc_vs_rl_distillation}). However, we observe a performance gap between the RL-trained \methodname{} teacher (98\%) and the distilled vision-based student (73\%), even after performance saturates with additional data. To investigate whether this gap stems from the change to visual input, we compared distillation performance between image-based and state-based students using the same number of trajectories. Their comparable performance suggests that the modality shift is not the primary cause of the performance gap. While DAgger-style online distillation might improve performance, we focused on offline distillation as it better reflects real-world deployment constraints.



% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{fig/distillation.pdf}
%     \caption{Comparison of performance between state and vision policies in policy distillation. The Diffusion Policy (DP) baseline achieves similar performance with both state and vision inputs when trained directly on the same 50 demonstrations (left), indicating that the vision modality does not inherently limit performance. However, we observe a significant performance gap when distilling our state-based \methodname{} policy into a vision-based policy (right). This suggests the challenge lies in the distillation process rather than the vision modality, as direct vision-based training shows no such degradation.}
%     \label{fig:bc_vs_rl_distillation}
% \end{figure}



% Therefore, we examine the impact of the distillation dataset size. Here, we scale up the number of state-based rollouts from the trained RL policy and distill these to a state-based student. In \autoref{fig:overview} (Right), we observe that performance increases with more data, from 78\% success rate at 10k trajectories to 80\% at 100k trajectories, though not reaching the teacher policy's 98\% success rate. The same trend is evident in \autoref{fig:scaling-round-table} (though the saturation occurs earlier). These results demonstrate how simulation-based distillation can complement existing training approaches by enabling the rapid generation of large-scale synthetic datasets at a minimal cost. Beyond the data volume advantages, our RL teacher exhibits qualitatively different behaviors, such as faster movements and improved corrective actions, suggesting that this synthetic data captures valuable task strategies that could be expensive or impractical to demonstrate manually.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{fig/scaling_round_table.pdf}
%     \caption{Scaling behavior comparison on the more complex \roundtable{} task mirrors the trends observed for \oneleg{} (\autoref{fig:overview} (right)), but with lower overall performance. Just as in \oneleg{}, increasing the number of demonstrations for BC training leads to diminishing returns, saturating at 56\% success rate. While DAgger's online data collection helps achieve better performance, it also plateaus at 71\%, well below our method's 94\% success rate. This consistent pattern across tasks, with lower saturation points for the more complex tasks, highlights the limitations of pure imitation approaches and the benefits of learning closed-loop control online.}
%     \label{fig:scaling-round-table}
% \end{figure}



% While DAgger~\cite{ross2011reduction} demonstrates strong sample efficiency - achieving better performance than BC with just $\sim$10k gradient steps (800 rollouts)---it requires an expert policy for online data collection. Although we could theoretically apply DAgger in simulation using our RL-trained expert policy (as demonstrated by~\cite{torne2024reconciling_rialto} for point cloud inputs), this introduces significant complexity to the pipeline and its effectiveness for RGB image-based distillation remains an open question for future work. Instead, we demonstrate that a simple approach combining offline rendering of synthetic trajectories with real-world co-training can achieve reasonable performance.


% \subsection{Real-World Evaluation}
% \label{sec:experiments-real-world}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{fig/Synthetic_Data.pdf}
%     \caption{Ephotorealistico-realistic rendering and domain randomization for sim-to-real transfer. In the first row, we show our nominal experiment setting of rendering parts in the original white color while varying the position, brightness, and hue of the lighting in the scene. In the bottom row, we also introduce variations in the part colors to see how that can help the final policy adapt to unseen part appearances without collecting any additional data.}
%     \label{fig:synthetic-data}
% \end{figure}

% \input{fig_text/real_world_qual}

% Finally, we evaluate the real-world performance of a sim-to-real policy trained on a mixture of a few (10/40) real-world demonstrations (\textbf{Real+Sim}) and simulation data generated by the trained residual RL policy. We compare the co-trained policy to a baseline model trained only on real-world demonstrations (\textbf{Real-Only}). We compare the success rates achieved by each policy on two sets of 10 trials for the \oneleg{} task. In the first set, we randomize part poses, while in the second set, we randomize obstacle poses (i.e., insertion location in the workspace).

% We compare the co-trained policy to a baseline model trained only on real-world demonstrations. We define an evaluation grid spanning the same ranges as the low randomization setting from the FurnitureBench simulation environment. We evaluate each policy on two sets of 10 trials for the \oneleg{} task, with grid points sampling either part poses or obstacle poses (i.e., insertion location in the workspace). Each method is evaluated on the same set of grid positions to ensure fair comparison.


% The results in \autoref{tab:real-world-real-cotrain} show that incorporating simulation data improves real-world performance (e.g., increasing task completion rate from 20-30\% to 50-60\%). Qualitatively, the sim-to-real policy exhibits smoother behavior and makes fewer erratic movements that might exceed the robot's physical limits. \autoref{fig:real-world-sequences} illustrates this through example trajectories: Row (A) shows successful executions where the robot completes the full assembly sequence, while Row (B) demonstrates the most common failure mode where, despite successfully grasping and transporting the parts, the policy fails to achieve precise alignment between the table leg and the hole before releasing. This misalignment failure pattern mirrors what we observe in the simulation, suggesting consistent challenges in achieving the required precision for insertion tasks.

% To further probe the robustness conferred by training in simulation, we created a task variation where the part colors are changed from black to white. When rolling out the policy trained on real demos of white parts, \textbf{Real-Only}, the robot exhibited erratic behavior that caused the hardware to reach velocity limits on every trial we ran, as shown in \autoref{fig:real-black-parts} (A). When including synthetic data rendered with parts in black, the resulting policy (\textbf{Real+Sim-DR}) can perform the task again (see \autoref{fig:real-black-parts}). The resulting performance was still inferior to the performance on white parts, which motivates further work on closing the sim-to-real gap.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_Black_1.pdf}
%     \caption{\textbf{(A)} When changing the part appearances from white to black, the policy trained on real data only (\textbf{Real-Only}) seizes to function. The behavior becomes erratic, and all trials ended with the robot hitting a velocity limit. \textbf{(B)} When mixing in synthetic data with more diverse colors (see \autoref{fig:synthetic-data}), the policy (\textbf{Real+Sim-DR}) regains the ability to complete the task, though with lower performance than for white parts.}
%     \label{fig:real-black-parts}
% \end{figure}


% ====== End old distillation/real-world section ======

==> Archive/experiment_setup.tex <==
\section{Experimental Setup}

\subsection{Tasks and Environment}
%
We evaluate our method on a set of challenging assembly tasks of \oneleg{}, \roundtable{}, and \lamp{} from the FurnitureBench~\cite{heo_furniturebench_2023} task suite, the \peghole{} task from~\cite{yash_factory2022_rss}, a custom mug-hanging task we call \mugrack{}, and a custom bimanual precise insertion task we call \bimaninsert{}. Examples of all tasks are shown in \autoref{fig:task-overview}. Visualizations of initial state distributions and detailed task descriptions are provided in \appref{app:tasks-and-environment}, and task rollouts can be seen on the \website{}.
 
Multi-part tight-tolerance assembly interactions are simulated using the SDF-based collision geometry representations provided as part of the Factory~\cite{yash_factory2022_rss} extension of Nvidia's IsaacGym simulator~\cite{makoviychuk2021isaac}, with demos collected using a \href{https://3dconnexion.com/us/product/spacemouse-wireless/}{SpaceMouse}. The \bimaninsert{} task is implemented using the MuJoCo simulator~\cite{todorov2012mujoco}, with the demos provided using the DART teleoperation system from~\cite{park2024dexhub}.

We define a simple, sparse task-completion reward set to 1 for each task when a pair of parts has been fully assembled and 0 otherwise. For example, in the \lamp{} task, the policy receives two binary rewards: the first when the bulb is fully screwed in and the second when the lamp shade is successfully placed. Some of our tasks are long horizon (up to $\sim$750-1000 steps at 10Hz) and require sequencing of behaviors such as 6-Degree-of-Freedom (DoF) grasping, reorientation, insertion, and screwing (see \autoref{fig:overview}; Left).


\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}c@{}lccccccccc@{}}
        \toprule
        & \multirow{2}{*}{Methods} & \multicolumn{2}{c}{\oneleg{}} & \multicolumn{2}{c}{\roundtable{}} & \multicolumn{2}{c}{\lamp{}} & \multicolumn{1}{c}{\mugrack{}} & \multicolumn{1}{c}{\peghole{}} & \multicolumn{1}{c}{\bimaninsert{}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11}
        & & Low & Med & Low & Med & Low & Med & Low & Low & Low  \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{BC}}\hspace{0.5em}}
        & MLP-S & 0  &  0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 \\
        & MLP-C & 45 & 10 & 5 & 2 & 8 & 1 & 21 & 2 & 7 \\
        & DP   & \textbf{54} & \textbf{26} & \textbf{12} & 4 & 7 & 2 & \textbf{26} & \textbf{5} & \textbf{33} \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{RL}}\hspace{0.5em}}
        & PPO-C & 70 & 28 & 38 & 6 & 32 & 2 & 23 & 4 & 30 \\
        & IDQL & 57 & 27 & 18 & 3 & 11 & 1 & 31 & 3 & 40 \\
        & \methodname{} (ours) & \textbf{98} & \textbf{76} & \textbf{94} & \textbf{77} & \textbf{97} & \textbf{70} & \textbf{88} & \textbf{99} & \textbf{93} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Success rates (percentage of successful completions over 1024 evaluation episodes using each method's best-performing checkpoint) for different policy architectures across our task suite. \textbf{Top:} Baseline BC methods, where Diffusion Policies (DP) generally outperform MLPs with chunking (MLP-C), while MLPs without chunking (MLP-S) are unable to solve all tasks except \peghole{}. \textbf{Bottom:} RL-based methods, where our proposed residual policy (\methodname{}) provides significant improvements in success rates over the base BC policy, improvements not seen from the alternative RL methods.}
    \label{tab:performance_comparison}
    \vspace{-15pt}
\end{table*}



\subsection{System Configuration}
The policy operates at 10Hz on a 7 Degrees-of-Freedom (DoF) Franka Emika Panda robot arm for all tasks but \bimaninsert{}, which operates at 50Hz on two Franka Panda arms (i.e., 14 DoF). The action space consists of the desired end-effector pose $\xform{}^{\text{des}} \in$ \sethree{} (i.e., both position and orientation) and a binary gripper command for opening/closing the parallel-jaw gripper. These desired end-effector poses are converted to joint position targets using differential inverse kinematics~\cite{manipulation}, then tracked using a low-level PD controller running at 1KHz with manually specified stiffness and dampening parameters tuned to balance compliance with accurate trajectory tracking.



\subsection{Evaluation protocol}
\label{sec:evaluation-protocol}


\subsubsection{Primary Evaluation}

We evaluate all methods by executing the policy from an initial state sampled from the same initial state distribution used for collecting demonstrations. We follow the default randomization protocol used in FurnitureBench~\cite{heo_furniturebench_2023}: at the beginning of each episode, objects are randomly offset from their nominal positions by $\Delta x, \Delta y \in [-1.5, 1.5]$ cm in the horizontal plane (with fixed height $z$) for low randomization settings and by $\Delta x, \Delta y \in [-5, 5]$ cm for medium randomization. For the U-shaped fixture used to stabilize parts during assembly (the three-sided white ``wall'' surrounding the parts in the left-most three columns in \autoref{fig:task-overview}), we apply additional offsets of $\Delta x, \Delta y \in [-2, 2]$ cm and $\Delta x, \Delta y \in [-4, 4]$ cm from its nominal position for low and medium settings respectively. 

We define task success as achieving the target geometric alignment between pairs of parts, as specified by the task reward function in \autoref{sec:problem-formulation}. For each method, we report the success rate calculated over 1024 evaluation episodes using the best-performing checkpoint, as our goal is to demonstrate the potential capabilities of each architectural approach rather than average performance across training runs.


\subsubsection{Robustness to Dynamic Disturbances}

To further evaluate robustness to dynamic disturbances, we also perform a version of the above evaluation that includes random force perturbations during policy execution. At each timestep, we randomly sample 1\% of the objects in the environment and apply a perturbation corresponding to the same randomization described above for initialization. These perturbations simulate unexpected contact forces and dynamic disturbances not seen during training. We evaluate each method's performance degradation under these conditions by comparing success rates with/without perturbations across 1024 rollouts.


\subsubsection{Real-World Evaluation Protocol}

For sim-to-real transfer, we use IsaacSim~\cite{mittal2023orbit} to render photorealistic trajectories of our simulation data, as it provides better rendering capabilities than IsaacGym. We evaluate policies across a grid of initial object and obstacle poses for real-world experiments that match our low randomization simulation setting ($\Delta x, \Delta y \in [-1.5, 1.5]$ cm). We perform 10 trials for each method and ensure that each method is tested on the same initial object states. Success criteria remain consistent with our simulation experiments: achieving target geometric alignment between assembly parts.


\subsection{Baselines and Ablations}
\label{sec:baselines}
\pulkit{Lars, my recommendation is to simplify this and mention the experiments we did with DP and fine-tuning DP with RL in many ways. Is there a specific point you want to make with IL on MLP-S and MLP-C -- again lets not call it IL, but call it BC -- also see notation in Table 1, it should be BC and not IL. MLP-S/MLP-C are just adding confusion; move them to the appendix totally}
% We outline the set of methods and ablations we test below. More details and hyperparameters are included in \appref{sec:implementation-details}.

We evaluate our method against several baselines to analyze the importance of action chunking, policy architecture, and reinforcement learning. Implementation details and hyperparameters are provided in \appref{sec:implementation-details}.



\subsubsection{Behavior Cloning Baselines}


We first evaluate the impact of action chunking by comparing a standard BC approach using an MLP (MLP-S) with a version that predicts action chunks (MLP-C). We find the Diffusion Policy architecture~\cite{chi_diffusion_2023} provides the strongest BC performance and use it as both our primary baseline and the foundation for \methodname{}.




\subsubsection{Distribution Shift Analysis}

To assess the impact of distribution shifts, we implement \textbf{DP-DAgger}~\cite{ross2011reduction}, which iteratively queries an expert policy to gather corrective demonstrations in states visited by the learned policy. Our experiments use \methodname{} as the expert. The DAgger policy is trained with the same BC loss as the nominal DP policy.


\subsubsection{Reinforcement Learning Comparisons}


Building on our BC policies, we compare two approaches for RL fine-tuning. First, we evaluate PPO fine-tuning of our chunked MLP policy (PPO-C)~\cite{schulman_proximal_2017}, treating each action chunk as a single concatenated action. For our diffusion-based policy, we implement IDQL~\cite{hansen-estruch_idql_2023}, where multiple action chunks are sampled from the diffusion policy and selected based on learned Q-values using the on-policy method of~\cite{shenfeld2024value}.




\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/BCFailRLSucc_V2.png}
    \caption{Examples of the common failures of our DP policies in tasks requiring precise part alignments. These failures can be mitigated by small corrections, making our residual framework, \methodname{}, well-suited to improve the reliability of the nominal DP policy.}
    \label{fig:common-errors}
    \vspace{-15pt}
\end{figure}


\subsubsection{Closed-Loop Control Ablation}
\label{sec:closed-loop-ablation}


To study the importance of per-timestep corrections, we implement \textbf{\methodname{}-C}, a variant of our method that predicts residual corrections at the same temporal resolution as the base policy's action chunks. Specifically, while the standard \methodname{} observes the current state and predicts a correction for each timestep, \methodname{}-C observes the current state and all actions in the predicted chunk and predicts a correction of all actions in the chunk. \methodname{}-C uses the same online PPO training procedure as \methodname{}. This chunked correction makes the learning problem more challenging as the residual policy predicts corrections for future timesteps without access to the intermediate states. See \autoref{app:closed-loop-ablation} for details.


\subsubsection{Real-World Baselines}

We compare the real-world performance of two policies: (1) \textbf{DP-Real-Only}: Diffusion policies trained exclusively on real-world demonstrations $\mathcal{D}_{\text{real}}$, using either 10 or 40 demonstrations, e.g., denoted 10 Real-Only. (2) \textbf{DP-Real+Sim}: Following our sim-to-real approach described in \autoref{sec:sim-to-real-pipeline-method}, we combine the same real-world demonstrations with our synthetic rendered dataset, e.g., denoted 10 Real+Sim.




==> Archive/experiment_v2.tex <==
% \vspace{-5pt}
\section{Experiments and Results}
\label{sec:experiments}

% \lars{Ensure this reflects the actual contents of the experiments: i.e., the first section presenting results in simulation and the second section everything regarding sim-to-real (distillation included here).}

% First, we investigate the requirement of complex BC methods \pulkit{what is complex BC methods?} and the impact of our residual reinforcement learning approach on improving the success rates of policies trained with behavior cloning in \autoref{sec:experiments-fine-tuning}. Next, we study the performance of downstream distillation from synthetic RL data, examining the relationship between the quantity and quality of the data and the resulting performance of the distilled vision-based policies in \autoref{sec:experiments-distillation-scaling} \pulkit{Not sure what we want to say here}. Finally, we evaluate our method in the real world \autoref{sec:experiments-real-world}.

Our experimental evaluation focuses on two key aspects. First, in Section IV-A, we analyze how augmenting a behavior-cloned policy with a residual RL component enables reliable execution of precise manipulation tasks, showing significant improvements over both standard BC approaches and traditional RL fine-tuning methods. Then, in Section IV-B, we demonstrate the practical applicability of our method by transferring these policies to real-world hardware through a simple yet effective combination of synthetic data generation and co-training with real demonstrations.


\paragraph{Evaluation protocol}
%
We evaluate all methods by executing the policy from an initial state sampled from the same initial state distribution for collecting demonstrations. We follow the default randomization protocol used in FurnitureBench~\cite{heo_furniturebench_2023}: at the beginning of every episode, objects are randomly offset from their nominal positions by $\Delta x, \Delta y \in [-1.5, 1.5]$ cm in the horizontal plane (with fixed height $z$) for low randomization settings and by $\Delta x, \Delta y \in [-5, 5]$ cm for medium randomization. For the U-shaped fixture used to stabilize parts during assembly (the three-sided white ``wall'' surrounding the parts in the left-most three columns in \autoref{fig:task-overview}), we apply additional offsets of $\Delta x, \Delta y \in [-2, 2]$ cm and $\Delta x, \Delta y \in [-4, 4]$ cm from its nominal position for low and medium settings respectively. The success rate is calculated as the average success over 1024 rollouts. The training data for human demonstrations and online RL is generated with the same initial state distribution.

\subsection{Augmenting Trajectory Planning with Reactive Control}
\label{sec:experiments-fine-tuning}

% \paragraph{Why Action Chunking and Diffusion Policies?}

% Simple feed-forward MLPs of modest size have shown impressive performance in many domains when trained with RL~\cite{kumar2021rma,lee2020learning,torne2024reconciling_rialto}, and offer a natural starting point for RL fine-tuning after BC pre-training. However, the standard MLP policies trained to directly output single action control instead of a trajectory plan through an action chunk (MLP-S) fail across all tasks we consider. Therefore, we also trained MLP policies with action chunking (MLP-C). When we introduce chunking, MLP performance improves drastically, as shown in \autoref{tab:performance_comparison}. However, we also find that the more complex Diffusion Policy (DP) architecture generally outperforms MLPs, especially in tasks of intermediate difficulty. For example, an improvement from 10\% success rate to 26\% for the \oneleg{} task on medium randomness makes subsequent fine-tuning far easier.

% In one case, \lamp{} on low randomness, MLP-C outperformed DP. In qualitative evaluations, we find that DP has smoother and faster actions, which is generally beneficial. Still, it seems to hurt performance in this case, as it tends to retract before the gripper fully grasps the lamp base. We also find that all methods struggle with the most challenging tasks, on which MLP-C and DP both achieve less than 5\% success rate, indicating that there is still room for improvement in BC methods. The \peghole{} task, despite its relatively short horizon of $\sim$100 timesteps, proved particularly challenging for BC methods. This task involves a $\sim$0.2 mm tolerance insertion, resulting in a 5\% success rate. This poor performance on a short yet precise task lends credence to the hypothesis that BC methods are ill-equipped to handle high-precision requirements.


% Another interesting finding is that the DP is significantly more robust to noise, an important property for an adequate base policy for residual fine-tuning. In contrast, we observed performance collapse when using MLP-C as the base, further reinforcing the utility of using powerful generative models for BC pre-training. See more analysis in \appref{app:residual-base-ablation}.




\paragraph{Online Policy Fine-Tuning Comparison}

Our experiments employ the Diffusion Policy (DP) architecture as the base BC policy, as we find it provides more robust and reliable behavior compared to simpler architectures (detailed analysis in \appref{app:residual-base-ablation}). The base DP policy achieves partial success on our manipulation tasks but struggles with high-precision requirements---for instance, achieving only a 5\% success rate on a sub-millimeter tolerance insertion task despite its relatively short horizon.

We investigate the effectiveness of our residual RL approach, \methodname{}, in improving the performance of policies trained with BC. We train residual policies using PPO~\cite{schulman_proximal_2017} on top of the diffusion policy and compare it to two baselines -- (1) directly fine-tune the MLP-C with PPO while regarding every action chunk as one concatenated action and (2) a chunked version of the IDQL algorithm~\cite{hansen-estruch_idql_2023}. In the IDQL algorithm, multiple action chunks are sampled from the diffusion policy, and one chooses the action chunk to execute based on its Q-value. We have found that learning a good Q-value estimator from offline data alone, as proposed in IDQL, is challenging with only 50 demonstrations. Therefore, we learn it in on-policy matter similar to~\cite{shenfeld2024value}.

The results in \autoref{tab:performance_comparison} show that our residual RL approach significantly improves success rates over BC and outperforms alternative RL fine-tuning methods. For tasks with lower initial randomization, such as the \oneleg{} task, the residual policy increases the success rate from 54\% to 98\%.
%
Even more drastically, for the \peghole{} task, \methodname{} improved the success rate from 5\% to 99\%.
%

However, even for our method, the performance saturates at $\sim$70\% in the medium randomization settings, where parts can be initially placed up to $\pm$5cm from their nominal positions. This drop in performance aligns with our intuition of the residual policy as a local correction mechanism that learns to make minor adjustments to the base BC policy's actions to improve precision and reactivity. When parts are placed far from their nominal positions, the BC policy may generate trajectories that deviate too far for the local correction mechanism to correct, leading to more failures.

We show some qualitative examples of the most common failure modes of the BC policies in \autoref{fig:common-errors} and \autoref{fig:overview} (Left). 
%
For instance, a typical error mode of the BC policy is pushing down the leg before it's aligned with the hole. Consequently, the object's pose changes while held in the gripper, causing the policy to diverge due to the out-of-distribution grasp pose.
%
The residual policy reliably corrects these errors by performing small sideways translations while avoiding premature downward motions. It typically only allows the leg to be inserted once it is appropriately above the hole.
%
We also find the residual policy is better at performing initial grasps that allow accurate downstream alignment between the grasped object and the receptacle. On the other hand, the BC policies more often grasp the object at angles that make insertion more difficult.
%
% In \autoref{fig:round-table-failure-modes}, we qualitatively analyze this \pulkit{what does "this" refer to?} for the \roundtable{} task and find that the residual \pulkit{use the name of our method \methodname{}} makes the precise insertion part of the task significantly more reliable. To understand failure modes of \methodname{}(see the \website{} for videos), we manually categorized 75 randomly sampled failures into three categories: `Peg Precision' failures occur while picking, inserting, or screwing the table leg, `Foot Precision' failures occur during same operations with the foot, and `Out-of-Distribution' failures occur when parts are unreachable by the policy. The remaining failures are attributed to simulation issues \pulkit{what kind of simulation issues?} or timeouts.
%
In \autoref{fig:round-table-failure-modes}, we qualitatively analyze these failure modes and recovery behaviors for the \roundtable{} task and find that \methodname{} makes the precise insertion part of the task significantly more reliable. To understand failure modes of \methodname{} (see the \website{} for videos), we manually categorized 75 randomly sampled failures into three categories: `Peg Precision' failures occur while picking, inserting, or screwing the table leg, `Foot Precision' failures occur during same operations with the foot, and `Out-of-Distribution' failures occur when parts are unreachable by the policy. The remaining failures are attributed to contact-modeling issues in simulation (such as object penetration causing unrealistic object acceleration) or timeouts.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/BCFailRLSucc_V2.png}
    \caption{Examples of the common failures made by BC policies in tasks requiring precise part alignments. These failures can be mitigated by small corrections, making our residual framework, \methodname{}, well-suited to improve the reliability of the nominal BC policy.}
    \label{fig:common-errors}
\end{figure}

% Surprisingly, the residual RL procedure also leads to the emergence of qualitatively different behaviors. We refer to the \href{https://residual-assembly.github.io/}{website}'s uncut videos of rollouts for the pre-trained and fine-tuned policies \pulkit{What do we mean by pre-trained and fine-tuned policies}. In these videos, we observe that the fine-tuned policy \pulkit{Finetuning is not the appropriate word -- let's call it nominal BC policy, and \methodname{} policy} has learned new grasps of the table foot that were not demonstrated \pulkit{what do we mean by new grasp?}, as well as more persistent retrying behavior and recovery.

Surprisingly, \methodname{} leads to the emergence of qualitatively different behaviors compared to the nominal BC policy (DP). We refer to the \href{https://residual-assembly.github.io/}{website}'s uncut videos of rollouts for both policies. In these videos, we observe that \methodname{} has discovered alternative grasping strategies not present in the demonstration data—while demonstrations only showed grasping the table foot from above its center, \methodname{} learned to grasp from the side when the center was unreachable. Additionally, \methodname{} exhibits more decisive recovery behaviors, making deliberate adjustments that lead to successful task completion where the nominal BC policy would ineffectively oscillate back and forth.

% In addition to improved success rates, we observed different training dynamics \pulkit{what do we mean by training dynamics?} across each method \pulkit{which methods?}.
%
% First, direct MLP-C fine-tuning (PPO-C) proved unstable and required KL-regularization to avoid collapse. Second, the trained DP produced actions with low variance, even with $\eta=1$ in the DDIM \pulkit{what is DDIM -- tell the full name and what it does at least intuitively} sampler~\cite{song2020denoising}, inhibiting Q-learning and constraining the potential for policy improvement.

In addition to improved success rates, we observed distinct training behavior and robustness across \methodname{}, direct MLP finetuning (PPO-C), and IDQL. First, direct MLP-C fine-tuning (PPO-C) proved unstable and required KL-regularization to avoid collapse. In contrast, \methodname{} demonstrated robust training, tolerating high update-to-data ratios without performance degradation and performing well across a broad range of hyperparameters. Second, for IDQL, the base DP model used for sampling produced actions with low variance even with $\eta=1$ in the Denoising Diffusion Implicit Model (DDIM) sampler~\cite{song2020denoising}---the iterative denoising procedure in diffusion models that converts noise into actions, where $\eta$ controls the stochasticity of this process. Despite setting this stochasticity parameter to its maximum value, the generated actions lacked sufficient exploration, which inhibited Q-learning and constrained the potential for policy improvement.

% Finally, residual policy training was very stable, likely because it is constrained to operate on a local scale \pulkit{how is this constrain imposed?}, which prevents large deviations that can make RL unstable and has a small parameter count compared to the base policy~\cite{kumar2020conservative, schulman2015trust} \pulkit{Why cite CQL or TRPO here?}. \pulkit{Are there any plots in the Appendix that show this?}

Finally, \methodname{} training was very stable, as its architecture naturally constrains it to predict small delta corrections to the base policy's poses, rather than operating in the full workspace coordinate frame. This local prediction scope, combined with the residual network's small parameter count, prevents the large policy updates that typically destabilize deep RL training~\cite{kumar2020conservative, schulman2015trust}. This stability is demonstrated in \autoref{fig:alpha-ablation}, showing consistent learning across hyperparameter settings.



\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/round_table_failure_modes.pdf}
    \caption{A qualitative analysis of the failure modes between the pre-trained BC policy and the fine-tuned residual policy for the \roundtable{} task on medium randomness. For the pre-trained policy, a large portion of the failures (40\%) relates to the table leg's insertion precision. In the fine-tuned policy, this share dropped to 0\%.}
    \label{fig:round-table-failure-modes}
\end{figure}


\paragraph{What drives performance of \methodname{}?}
We hypothesized that the performance of BC can be improved by training on-policy and by training a closed-loop reactive component. We analyzed the contribution of these two factors in improving the performance of \methodname{} over the nominal BC policy. 
%To understand the contribution of what drives the residual RL fine-tuning approach's performance, we try to decompose it into an on-policy component and a closed-loop, reactive component.

% To probe the impact of on-policy learning, we compared the performance of policies trained with the same amount of data gathered offline versus online using from DAgger~\cite{ross2011_dagger} from an expert policy. \pulkit{How do we get the expert to apply DAGGER}. Unsurprisingly, DAgger trained policy performs significantly better than a policy trained with offline data as reported in \autoref{fig:overview} (right) and \autoref{fig:scaling-round-table}. However, on-policy training doesn't fully explain the performance benefits enjoyed by \methodname{} and trails by 9\% and 23\% for the \oneleg{} and \roundtable{} tasks, respectively.

To probe the impact of on-policy learning, we compared performances between policies trained with offline data versus online data collected via DAgger~\cite{ross2011_dagger}. For this experiment, we used \methodname{} itself as the expert policy for DAgger, as it achieves near-perfect success rates. While the DAgger-trained policy significantly outperforms the offline-trained policy (see yellow vs. red lines in \autoref{fig:overview} (right) and \autoref{fig:scaling-round-table}), it still trails \methodname{} (blue line) by 9\% and 23\% for the \oneleg{} and \roundtable{} tasks, respectively. This suggests that on-policy learning alone does not fully explain \methodname{}'s performance benefits, and moreover, highlights a practical limitation of DAgger: it requires access to an expert policy, creating a circular dependency in many applications.


% On the other hand, we also find the residual policy's closed-loop, single-step nature helpful \pulkit{What is the significance of single-step nature?}. First, when trying to learn a residual policy for whole chunks \pulkit{What does this mean? Predicting the residual for the entire chunk, instead of per action?}, the resulting policy learns significantly more slowly, and the performance saturates at a lower level than that of the full closed-loop policy \pulkit{good to give a sense of how much lower}. See \appref{app:closed-loop-ablation} for details.

On the other hand, we also find the residual policy's closed-loop, per-timestep correction nature helpful. While the base BC model predicts action chunks, \methodname{} provides corrections at every timestep. When we instead implement an ablated version (\methodname{}-C) that predicts corrections at the same chunk-level frequency as the base policy, the resulting policy learns significantly more slowly and performance saturates at 92\% compared to \methodname{}'s 98\%. See \appref{app:closed-loop-ablation} for details.

% To further probe the value of closed-loop control, we conduct an experiment where random force perturbations are applied during execution, introducing dynamic disturbances not seen during training. As shown in \autoref{fig:online_perturbation_comparison}, our per-timestep approach maintains robust performance with only a 12\% drop under perturbations, while methods executing actions in chunks suffer more significant degradation. This includes both the pre-trained BC and DAgger policies and an ablated version of our method that predicts residuals \pulkit{Its good to give names to method -- e.g., \methodname{}, \methodname{}-chunked and call by them -- its much easier to follow, otherwise its quite confusing} for entire chunks rather than individual timesteps, all of which drop 19-26 percentage points from their nominal performance. These results demonstrate the importance of frequency close-loop corrections for handling unexpected and dynamic disturbances.

To further probe the value of closed-loop control, we conduct an experiment where random force perturbations are applied during execution, introducing dynamic disturbances not seen during training. As shown in \autoref{fig:online_perturbation_comparison}, \methodname{} maintains robust performance with a 12\% drop under perturbations, while chunk-based methods suffer more significant degradation. Specifically, the nominal BC policy (DP), DAgger policy, and \methodname{}-C (our method modified to predict chunk-level residuals) drop 19-26 percentage points from their nominal performance. These results demonstrate the importance of frequent closed-loop corrections for handling unexpected and dynamic disturbances.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/online_perturbation_comparison.pdf}
    \caption{Performance robustness when introducing random force perturbations during evaluation. Our method (\methodname{}), which makes per-timestep corrections, shows greater resilience with only a 12\% performance drop compared to nominal conditions. In contrast, methods executing actions in chunks (including an ablation of our method that learns to predict residuals for entire chunks with online RL) see larger drops of 19-26\%. This highlights the value of closed-loop control for handling dynamic disturbances. See \appref{app:closed-loop-ablation} for details.}
    \label{fig:online_perturbation_comparison}
\end{figure}


Another interesting finding is that the DP is significantly more robust to noise, an important property for an adequate base policy for residual fine-tuning. In contrast, we observed performance collapse when using MLP-C as the base, further reinforcing the utility of using powerful generative models for BC pre-training. See more analysis in \appref{app:residual-base-ablation}.


\subsection{Training Vision Policies}
\label{sec:experiments-distillation-scaling}

\input{fig_text/real_results_table}

\pulkit{There is too much emphasis on distillation -- why is that?}
% Next, we study how synthetic RL data quantity and quality \pulkit{What is meant by synthetic RL data?} impact the performance of vision-based policies. A vision-based policy distilled from the RL-trained teacher reached 73\% on \oneleg{}, outperforming the 50\% achieved by training the vision policy directly on human demos, see \autoref{fig:bc_vs_rl_distillation} \pulkit{evaluation in sim or in the real-world?}. However, we also observe a performance gap between the RL-trained teacher (98\%) and distilled vision-based student policy (73\%) \pulkit{With how much data? Is the performance improving with data? Is the distillation performed offline or online DAGGER style? If not DAGGER style then why not?}. We consider whether this gap may be caused by training the student to operate on images. Upon examination, we find that distilling the same number of teacher rollouts into an image-based student and a state-based student results in comparable performance \pulkit{what is a student? Have we defined it anywhere? How much data is used for distillation?}. This leads us to conclude that the change in modality is not the primary source of the performance gap.

Next, we study how the quantity and quality of data generated by a \methodname{} policy impacts the performance of vision-based student policies in real-world evaluations. We generate this data by collecting successful trajectories from the \methodname{} teacher across varied initial states and rendering corresponding camera observations. A vision-based student policy---which shares the same architecture as the teacher but includes an additional image encoder---distilled from $\sim$1,000 teacher trajectories reached 73\% success on \oneleg{}, outperforming the 50\% achieved by training the vision policy directly on human demos (see \autoref{fig:bc_vs_rl_distillation}). However, we observe a performance gap between the RL-trained \methodname{} teacher (98\%) and the distilled vision-based student (73\%), even after performance saturates with additional data. To investigate whether this gap stems from the change to visual input, we compared distillation performance between image-based and state-based students using the same number of trajectories. Their comparable performance suggests that the modality shift is not the primary cause of the performance gap. We note that while DAgger-style online distillation might improve performance, we focused on offline distillation as it better reflects real-world deployment constraints.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/distillation.pdf}
    \caption{Comparison of performance between state and vision policies in policy distillation. The Diffusion Policy (DP) baseline achieves similar performance with both state and vision inputs when trained directly on the same 50 demonstrations (left), indicating that the vision modality does not inherently limit performance. However, we observe a significant performance gap when distilling our state-based \methodname{} policy into a vision-based policy (right). This suggests the challenge lies in the distillation process rather than the vision modality, as direct vision-based training shows no such degradation.}
    \label{fig:bc_vs_rl_distillation}
\end{figure}


% Therefore, we also examine the impact of the distillation dataset size. Here, we scale up the number of state-based rollouts from the trained RL policy and distill these to a state-based student. In \autoref{fig:overview} (Right), we see that performance increases with more data but still does not reach the performance achieved by the teacher policy, with a gap of 20 percentage points between the best student policy (80\% success rate) and the teacher policy (98\% success rate) at 100k trajectories (with only a minor improvement from 78\% at 10k trajectories). The same trend is evident in \autoref{fig:scaling-round-table} (though the saturation occurs earlier). Nevertheless, the improved performance obtained by training with more data highlights the advantage of using simulation for obtaining large-scale synthetic datasets \pulkit{It doesn't really highlight the benefits -- in the real world, one would train directly from images}.

Therefore, we examine the impact of the distillation dataset size. Here, we scale up the number of state-based rollouts from the trained RL policy and distill these to a state-based student. In \autoref{fig:overview} (Right), we observe that performance increases with more data, from 78\% success rate at 10k trajectories to 80\% at 100k trajectories, though not reaching the teacher policy's 98\% success rate. The same trend is evident in \autoref{fig:scaling-round-table} (though the saturation occurs earlier). These results demonstrate how simulation-based distillation can complement existing training approaches by enabling the rapid generation of large-scale synthetic datasets at a minimal cost. Beyond the data volume advantages, our RL teacher exhibits qualitatively different behaviors, such as faster movements and improved corrective actions, suggesting that this synthetic data captures valuable task strategies that could be expensive or impractical to demonstrate manually.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/scaling_round_table.pdf}
    \caption{Scaling behavior comparison on the more complex \roundtable{} task mirrors the trends observed for \oneleg{} (\autoref{fig:overview} (right)), but with lower overall performance. Just as in \oneleg{}, increasing the number of demonstrations for BC training leads to diminishing returns, saturating at 56\% success rate. While DAgger's online data collection helps achieve better performance, it also plateaus at 71\%, well below our method's 94\% success rate. This consistent pattern across tasks, with lower saturation points for the more complex tasks, highlights the limitations of pure imitation approaches and the benefits of learning closed-loop control online.}
    \label{fig:scaling-round-table}
\end{figure}


% DAgger~\cite{ross2011reduction} demonstrates significantly greater sample and computational efficiency than pure BC. As shown in \autoref{fig:overview} (right), DAgger achieves superior performance to BC trained on 50 human demos in just $\sim$10k gradient steps (with 800 rollouts) and surpasses our best BC distillation results at $\sim$20k steps (with $\sim$1.5k demonstrations). These results underscore the advantages of interactive learning over passive offline learning and point towards effective online distillation techniques to help close the gap between the state-based RL-trained experts and the distilled real-world policies deployed on real hardware (see \autoref{sec:experiments-real-world}) \pulkit{I am not sure what the takeaway here is}.

While DAgger~\cite{ross2011reduction} demonstrates strong sample efficiency - achieving better performance than BC with just $\sim$10k gradient steps (800 rollouts)---it requires an expert policy for online data collection. Although we could theoretically apply DAgger in simulation using our RL-trained expert policy (as demonstrated by~\cite{torne2024reconciling_rialto} for point cloud inputs), this introduces significant complexity to the pipeline and its effectiveness for RGB image-based distillation remains an open question for future work. Instead, we demonstrate that a simple approach combining offline rendering of synthetic trajectories with real-world co-training can achieve reasonable performance.


\subsection{Real-World Evaluation}
\label{sec:experiments-real-world}

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/Synthetic_Data.pdf}
    \caption{Examples of photo-realistic rendering and domain randomization for sim-to-real transfer. In the first row, we show our nominal experiment setting of rendering parts in the original white color while varying the position, brightness, and hue of the lighting in the scene. In the bottom row, we also introduce variations in the part colors to see how that can help the final policy adapt to unseen part appearances without collecting any additional data.}
    \label{fig:synthetic-data}
\end{figure}
\input{fig_text/real_world_qual}

Finally, we evaluate the real-world performance of a sim-to-real policy trained on a mixture of a few (10/40) real-world demonstrations (\textbf{Real+Sim}) and simulation data generated by the trained residual RL policy. We compare the co-trained policy to a baseline model trained only on real-world demonstrations (\textbf{Real-Only}). We compare the success rates achieved by each policy on two sets of 10 trials for the \oneleg{} task. In the first set, we randomize part poses, while in the second set, we randomize obstacle poses (i.e., insertion location in the workspace).

We compare the co-trained policy to a baseline model trained only on real-world demonstrations. We define an evaluation grid spanning the same ranges as the low randomization setting from the FurnitureBench simulation environment. We evaluate each policy on two sets of 10 trials for the \oneleg{} task, with grid points sampling either part poses or obstacle poses (i.e., insertion location in the workspace). Each method is evaluated on the same set of grid positions to ensure fair comparison.


The results in \autoref{tab:real-world-real-cotrain} show that incorporating simulation data improves real-world performance (e.g., increasing task completion rate from 20-30\% to 50-60\%). Qualitatively, the sim-to-real policy exhibits smoother behavior and makes fewer erratic movements that might exceed the robot's physical limits. \autoref{fig:real-world-sequences} illustrates this through example trajectories: Row (A) shows successful executions where the robot completes the full assembly sequence, while Row (B) demonstrates the most common failure mode where, despite successfully grasping and transporting the parts, the policy fails to achieve precise alignment between the table leg and the hole before releasing. This misalignment failure pattern mirrors what we observe in the simulation, suggesting consistent challenges in achieving the required precision for insertion tasks.

To further probe the robustness conferred by training in simulation, we created a task variation where the part colors are changed from black to white. When rolling out the policy trained on real demos of white parts, \textbf{Real-Only}, the robot exhibited erratic behavior that caused the hardware to reach velocity limits on every trial we ran, as shown in \autoref{fig:real-black-parts} (A). When including synthetic data rendered with parts in black, the resulting policy (\textbf{Real+Sim-DR}) can perform the task again (see \autoref{fig:real-black-parts}). The resulting performance was still inferior to the performance on white parts, which motivates further work on closing the sim-to-real gap.


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_Black_1.pdf}
    \caption{\textbf{(A)} When changing the part appearances from white to black, the policy trained on real data only (\textbf{Real-Only}) seizes to function. The behavior becomes erratic, and all trials ended with the robot hitting a velocity limit. \textbf{(B)} When mixing in synthetic data with more diverse colors (see \autoref{fig:synthetic-data}), the policy (\textbf{Real+Sim-DR}) regains the ability to complete the task, though with lower performance than for white parts.}
    \label{fig:real-black-parts}
\end{figure}




==> Archive/fig_text/bc_fail_rl_succ.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{fig/BCFailRLSucc_V1.pdf}
%     \caption{Representative failures from BC policies (images show separate episodes). A common BC-policy error is to push down before the leg is aligned with the hole. This often results in a shift of the object in the grasp, which causes the policy to diverse due to the out of distribution grasp pose. We observe the residual policy regularly counteracts these premature downward motions, typically only allowing the leg to be inserted once its properly above the hole.}
%     % \caption{\textbf{(A)} Representative failures from BC policies. \textbf{(B)} Examples of how the RL-trained residual policy reduces the frequency of the common errors made by BC-trained policies. For example, a common BC-policy error is to push down before aligning the leg with the hole, causing the grasp the shift and the policy to diverse due to the out of distribution grasp pose. We observe the residual policy counteracts these premature downward motions, oftentimes only allowing the leg to be inserted once its properly above the hole. \anthony{make it clear that left to right is not the same episode}}
%     \label{fig:bc-failure-rl-success}
% \end{figure}


% \begin{wrapfigure}{r}{0.4\textwidth}
%   \centering
%   \vspace{-20pt}
%   \includegraphics[width=0.4\textwidth]{fig/BCFailRLSucc_V2.pdf}
%   \caption{Representative failures from BC policies. RL-trained residual policies dramatically improve succcess rate by correcting for these errors.} % A common BC-policy error is to push down before the leg is aligned with the hole. This often results in a shift of the object in the grasp, which causes the policy to diverse due to the out of distribution grasp pose. We observe the residual policy regularly counteracts these premature downward motions, typically only allowing the leg to be inserted once its properly above the hole.} % for sim2real.}
%   \vspace{-5pt}
%   \label{fig:bc-failure-rl-success}
% \end{wrapfigure}


% \begin{figure}[h]
%   \centering
%   % \vspace{-20pt}
%   \includegraphics[width=0.4\textwidth]{fig/BCFailRLSucc_V2.png}
%   \caption{Representative failures from BC policies. RL-trained residual policies dramatically improve the success rate by correcting for these errors.}
%   \label{fig:bc-failure-rl-success}
%   \vspace{-10pt}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   % \vspace{-20pt}
%   \includegraphics[width=0.4\textwidth]{fig/Task overview.png}
%   \caption{Representative failures from BC policies. RL-trained residual policies dramatically improve the success rate by correcting for these errors.}
%   \label{fig:bc-failure-rl-success}
%   \vspace{-10pt}
% \end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.48\textwidth]{fig/ResidualDiffusionDiagram_2.png}
  \caption{Overview of \methodname{}. A pretrained \textcolor{bccolor}{chunked base policy} predicts an action chunk of $T_a$ future actions. For every timestep, the \textcolor{rlcolor}{residual model} observes the current state $s_t$ and predicted base action $a_t^{\text{base}}$ and corrects.} 
  \label{fig:residual-diffusion}
  \vspace{-15pt}
\end{figure}



==> Archive/fig_text/distillation.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{fig/distillation.pdf}
  \captionof{figure}{Comparison of distilled performance from BC and RL-based teacher.}
  \label{fig:bc_vs_rl_distillation}
\end{figure}

==> Archive/fig_text/main_perf_table.tex <==

% \begin{figure*}[t]
%     \begin{minipage}[t]{0.74\textwidth}
%         \vspace{0pt}  % This ensures alignment to the very top
%         \centering
%         \resizebox{\linewidth}{!}{%
%         \begin{tabular}{@{}c@{}lccccccccc@{}}
%             \toprule
%             & \multirow{2}{*}{Methods} & \multicolumn{2}{c}{\oneleg{}} & \multicolumn{2}{c}{\roundtable{}} & \multicolumn{2}{c}{\lamp{}} & \multicolumn{1}{c}{\mugrack{}} & \multicolumn{1}{c}{\texttt{peg-hole}} & \multicolumn{1}{c}{\bimaninsert{}} \\
%             \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}
%             & & Low & Med & Low & Med & Low & Med & Low & Low & Low  \\
%             \midrule
%             \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{IL}}\hspace{0.5em}}
%             & MLP-S & 0  &  0 & 0 & 0 & 0 & 0 & 0 & 2 &  \\
%             & MLP-C & 45 & 10 & 5 & 2 & \textbf{8} & 1 & 21 & 2 &  \\
%             & DP   & \textbf{54} & \textbf{29} & \textbf{12} & \textbf{4} & 7 & \textbf{2} & \textbf{29} & \textbf{5} & 3 \\
%             \midrule
%             \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{RL}}\hspace{0.5em}}
%             & MLP-C + PPO & 70 & 28 & 38 & 6 & 32 & 2 & 23 & 4 &  \\
%             & DP + IDQL & 52 & 13 & 18 & 3 & 11 & 1 & 31 & 3 &  \\
%             & \methodname{} (ours) & \textbf{98} & \textbf{76} & \textbf{94} & \textbf{77} & \textbf{97} & \textbf{70} & \textbf{88} & \textbf{99} & 93 \\
%             \bottomrule
%         \end{tabular}
%         }
%         \captionof{table}{\textbf{Top} BC-trained MLPs without chunking (MLP-S) cannot perform any of the tasks, and Diffusion Policies (DP) generally outperform MLPs with chunking (MLP-C). \textbf{Bottom} Training our proposed residual policies with RL on top of frozen DP performs the best among the evaluated fine-tuning techniques. \pulkit{there are no error bars -- do we know what the performance is?}}
%         \label{tab:performance_comparison}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.235\textwidth}
%         \vspace{0pt}  % This ensures alignment to the very top
%         \centering
%         \includegraphics[width=\linewidth]{fig/Task overview.png}
%         \caption{Examples of tasks used for method evaluations.\pulkit{Make a separate figure showing the tasks}}
%         \label{fig:task-overview}
%     \end{minipage}
%     \vspace{-15pt}
% \end{figure*}




\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}c@{}lccccccccc@{}}
        \toprule
        & \multirow{2}{*}{Methods} & \multicolumn{2}{c}{\oneleg{}} & \multicolumn{2}{c}{\roundtable{}} & \multicolumn{2}{c}{\lamp{}} & \multicolumn{1}{c}{\mugrack{}} & \multicolumn{1}{c}{\peghole{}} & \multicolumn{1}{c}{\bimaninsert{}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10} \cmidrule(lr){11-11}
        & & Low & Med & Low & Med & Low & Med & Low & Low & Low  \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{IL}}\hspace{0.5em}}
        & MLP-S & 0  &  0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 \\
        & MLP-C & 45 & 10 & 5 & 2 & 8 & 1 & 21 & 2 & 7 \\
        & DP   & \textbf{54} & \textbf{29} & \textbf{12} & 4 & 7 & 2 & \textbf{26} & \textbf{5} & \textbf{33} \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{RL}}\hspace{0.5em}}
        & PPO-C & 70 & 28 & 38 & 6 & 32 & 2 & 23 & 4 & 30 \\
        & IDQL & 52 & 27 & 18 & 3 & 11 & 1 & 31 & 3 & 40 \\
        & \methodname{} (ours) & \textbf{98} & \textbf{76} & \textbf{94} & \textbf{77} & \textbf{97} & \textbf{70} & \textbf{88} & \textbf{99} & \textbf{93} \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Top} BC-trained MLPs without chunking (MLP-S) cannot perform any of the tasks, and Diffusion Policies (DP) generally outperform MLPs with chunking (MLP-C). \textbf{Bottom} Training our proposed residual policies with RL on top of frozen DP performs the best among the evaluated fine-tuning techniques. The best checkpoint is chosen for all methods, and we average over 1024 rollouts to get the success rate.
    }
    \label{tab:performance_comparison}
    % \vspace{-15pt}
\end{table*}

==> Archive/fig_text/main_perf_table_w_succ_fail.tex <==

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}

    % \begin{table}[htbp]
    % \centering
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{One Leg} & \multicolumn{2}{c}{Round Table} & \multicolumn{2}{c}{Lamp} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
     & Low & Med & Low & Med & Low & Med \\
    \midrule
    \multicolumn{7}{l}{\textbf{IL}} \\
    MLP-S & 0  &  0 & 0 & 0 & 0 & 0 \\
    MLP-C & 45 & 10 & 7 & 3 & 8 & 2 \\
    DP   & 55 & 34 & 11 & 3 & 4 & 2 \\
    \midrule
    \multicolumn{7}{l}{\textbf{RL}} \\
    Direct MLP FT & 64 & 20 & & & & \\
    IDQL & 52 & 13 & & & & \\
    Residual Diffusion & 95 & 68 & 48 & 6 & 6 & 2 \\
    \bottomrule
    \end{tabular}
    \vspace{10pt}
    \caption{Performance comparison of IL and RL.}
    \label{tab:performance_comparison}
    % \end{table}

    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/BCFailRLSucc_V1.pdf}
        \caption{\textbf{Left} Representative failures from BC policies. \textbf{Right} Examples showing how the RL policy reduces the frequency of the common errors made by BC-trained policies.}
        \label{fig:bc-failure-rl-success}
    \end{subfigure}
    \caption{Side by side of table and PDF.}
    \label{fig:main-table-fig-bc-vs-rl}
\end{figure}

==> Archive/fig_text/pipeline.tex <==

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/framework_overview.pdf}
    \caption{\textbf{Sim-to-real pipeline.} \textcolor{longcolor}{\textbf{(1)}} Beginning with a policy trained with BC in simulation, \textcolor{rlcolor}{\textbf{(2)}} we train residual policies with RL and sparse rewards. \textcolor{daggercolor}{\textbf{(3)}} We then distill the resulting behaviors into a policy operating from RGB images. \textcolor{bccolor}{\textbf{(4)}} By combining synthetic data with a small set of real demonstrations, \textcolor{cotrain}{\textbf{(5)}} we deploy RGB-based policies in the real world.}
    \label{fig:pipeline}
    \vspace{-15pt}
\end{figure*}

==> Archive/fig_text/real_results_table.tex <==
% % \begin{table*}
% % \centering
% % \resizebox{\linewidth}{!}{%
% % \begin{tabular}{lcccccccccc}
% % \toprule
% % \multirow{2}{*}{Training data} & \multicolumn{2}{c}{Corner} & \multicolumn{2}{c}{Grasp} & \multicolumn{2}{c}{Insert} & \multicolumn{2}{c}{Screw} & \multicolumn{2}{c}{Complete} \\
% % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
% %  & Part & Obs & Part & Obs & Part & Obs & Part & Obs & Part & Obs \\
% % \midrule
% % 10 Real & 5/10 & 5/10 & 5/10 & 7/10 & 2/10 & 3/10 & 0/10 & 2/10 & 0/10 & 2/10 \\
% % 10 Real + 350 Sim & 9/10 & 9/10 & 7/10 & 8/10 & 0/10 & 3/10 & 0/10 & 3/10 & 0/10 & 3/10 \\
% % \addlinespace[.5ex]
% % \hdashline
% % \addlinespace[1ex]
% % 40 Real & 10/10 & 8/10 & 9/10 & 8/10 & 6/10 & 3/10 & 2/10 & 3/10 & 2/10 & 3/10\\
% % 40 Real + 350 Sim & 10/10 & 10/10 & 9/10 & 10/10 & 6/10 & 7/10 & 5/10 & 6/10 & 5/10 & 6/10\\
% % \bottomrule
% % \end{tabular}}
% % \vspace{10pt}
% % \caption{We compare the impact of combining real-world demonstrations with simulation trajectories obtained by rolling our RL-trained residual policies. Co-training with real and synthetic data improves motion quality and success rate on the \oneleg{} task.}
% % \label{tab:real-world-real-cotrain}
% % \vspace{-15pt}
% % \end{table*}


% \begin{figure*}
% \centering
% \begin{minipage}[t]{0.69\textwidth}
% \centering
% \vspace{0pt}
% \raisebox{-\height}{%
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% \multirow{2}{*}{Training data} & \multicolumn{2}{c}{Corner} & \multicolumn{2}{c}{Grasp} & \multicolumn{2}{c}{Insert} & \multicolumn{2}{c}{Screw} & \multicolumn{2}{c}{Complete} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
%  & Part & Obs & Part & Obs & Part & Obs & Part & Obs & Part & Obs \\
% \midrule
% 10 Real & 5/10 & 5/10 & 5/10 & 7/10 & 2/10 & 3/10 & 0/10 & 2/10 & 0/10 & 2/10 \\
% 10 Real + 350 Sim & 9/10 & 9/10 & 7/10 & 8/10 & 0/10 & 3/10 & 0/10 & 3/10 & 0/10 & 3/10 \\
% \addlinespace[.5ex]
% \hdashline
% \addlinespace[1ex]
% 40 Real & 10/10 & 8/10 & 9/10 & 8/10 & 6/10 & 3/10 & 2/10 & 3/10 & 2/10 & 3/10\\
% 40 Real + 350 Sim & 10/10 & 10/10 & 9/10 & 10/10 & 6/10 & 7/10 & 5/10 & 6/10 & 5/10 & 6/10\\
% \bottomrule
% \end{tabular}
% }}
% \captionof{table}{We investigate the effect of combining real-world demonstrations with simulation trajectories from our RL-trained residual policies. Co-training with real and synthetic data improves motion quality and success rate on the \oneleg{} task.}
% \label{tab:real-world-real-cotrain}
% \end{minipage}%
% \hfill
% \begin{minipage}[t]{0.28\textwidth}
% \centering
% \vspace{0pt}
% \includegraphics[width=\linewidth]{fig/online_perturbation_comparison.png}
% \caption{Perturbations highlight \methodname{}'s resilience: 12\% drop vs. 19-26\% for chunked methods. \pulkit{Too many acronyms -- too small of a graph}}
% \vspace{-5pt}
% \label{fig:online_perturbation_comparison}
% \end{minipage}
% \vspace{-10pt}
% \end{figure*}


\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{Training data} & \multicolumn{2}{c}{Corner} & \multicolumn{2}{c}{Grasp} & \multicolumn{2}{c}{Insert} & \multicolumn{2}{c}{Screw} & \multicolumn{2}{c}{Complete} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
     & Part & Obs & Part & Obs & Part & Obs & Part & Obs & Part & Obs \\
    \midrule
    10 Real-Only & 5/10 & 5/10 & 5/10 & 7/10 & 2/10 & 3/10 & 0/10 & 2/10 & 0/10 & 2/10 \\
    10 Real+Sim & 9/10 & 9/10 & 7/10 & 8/10 & 0/10 & 3/10 & 0/10 & 3/10 & 0/10 & 3/10 \\
    \addlinespace[.5ex]
    \hdashline
    \addlinespace[1ex]
    40 Real-Only & 10/10 & 8/10 & 9/10 & 8/10 & 6/10 & 3/10 & 2/10 & 3/10 & 2/10 & 3/10\\
    40 Real+Sim & 10/10 & 10/10 & 9/10 & 10/10 & 6/10 & 7/10 & 5/10 & 6/10 & 5/10 & 6/10\\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparing the effect of combining real-world demonstrations with simulation trajectories from our RL-trained residual policies. Co-training with real and synthetic data improves motion quality and success rate on the \oneleg{} task.}
    \label{tab:real-world-real-cotrain}
    % \vspace{-15pt}
\end{table*}

==> Archive/fig_text/real_results_table_5_trials.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Training data} & \multicolumn{2}{c}{Corner} & \multicolumn{2}{c}{Grasp} & \multicolumn{2}{c}{Insert} & \multicolumn{2}{c}{Screw} & \multicolumn{2}{c}{Complete} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
 % & Med & Low & Med & Low & Med & Low & Med & Low & Med & Low \\
 & Part & Obs & Part & Obs & Part & Obs & Part & Obs & Part & Obs \\
\midrule
10 Real & 3/5  &  2/5 & 2/5 & 4/5 & 2/5 & 1/5 & 0/5 & 1/5 & 0/5 & 1/5 \\
10 Real + 350 Sim & 5/5 & 5/5 & 5/5 & 4/5 & 0/5 & 2/5 & 0/5 & 2/5 & 0/5 & 2/5 \\
\addlinespace[.5ex]
\hdashline
\addlinespace[1ex]
40 Real & 5/5  &  5/5 & 4/5 & 5/5 & 3/5 & 2/5 & 1/5 & 2/5 & 1/5 & 2/5\\
40 Real + 350 Sim & 5/5 & 5/5 & 4/5 & 5/5 & 3/5 & 4/5 & 3/5 & 3/5 & 3/5 & 3/5\\
\bottomrule
\end{tabular}
\vspace{10pt}
\caption{Real world results on \oneleg{} task using varying amounts of real-world demonstrations compared to combining real-world demonstrations and simulation trajectories obtained by rolling out trained RL policies and re-rendering in Isaac Sim with visual domain randomization.}
\label{tab:real-world-real-cotrain}
\end{table}

==> Archive/fig_text/real_world_qual.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\linewidth]{fig/RealWorldSeqs_3.pdf}
%     \caption{\textbf{(A)} Examples of successful real world assembly from RGB. Co-training with simulation data reduces jerkiness and improves insertion robustness, due to data from simulation containing higher diversity of initial part poses and insertion locations (see Table~\ref{tab:real-world-real-cotrain}). \textbf{(B)} Representative failures, primarily due to overfitting to a particular corner location and difficulty adjusting the insertion angle/position when grasps lead to unfamiliar in-hand part poses.}
%     \label{fig:real-world-sequences}
%     \vspace{-15pt}
% \end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/RealWorldSeqs_3.pdf}
    \caption{\textbf{(A)} Examples of successful real world assembly from RGB. Co-training with simulation data reduces jerkiness and improves insertion robustness by containing a higher diversity of part poses and insertion locations (see Table~\ref{tab:real-world-real-cotrain}). \textbf{(B)} Example failure: difficulty adjusting the insertion angle/position when grasps lead to unseen in-hand part poses.}
    \label{fig:real-world-sequences}
    \vspace{-15pt}
\end{figure*}

==> Archive/fig_text/residual_diagram.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
%   \vspace{-15pt}
%   \centering
%   \includegraphics[width=0.4\textwidth]{fig/ResidualDiffusionDiagram.pdf}
%   \caption{Per-timestep residual policies trained with PPO to locally correct action chunks predicted by a BC-trained diffusion policy.} % for sim2real.}
%   \vspace{-10pt}
%   \label{fig:residual-diagram}
% \end{wrapfigure}


\begin{figure}
  % \vspace{-15pt}
  \centering
  \includegraphics[width=0.3\textwidth]{fig/ResidualDiffusionDiagram.pdf}
  \caption{Per-timestep residual policies trained with PPO to locally correct action chunks predicted by a BC-trained diffusion policy.} % for sim2real.}
  % \vspace{-10pt}
  \label{fig:residual-diagram}
\end{figure}

==> Archive/fig_text/sim_renders.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
%   \vspace{-15pt}
%   \centering
%   \includegraphics[width=0.4\textwidth]{fig/SimRenderExamples.pdf}
%   \caption{Rendering successful trajectories with appearance randomization.} % for sim2real.}
%   \vspace{-60pt}
%   \label{fig:sim-render-examples}
% \end{wrapfigure}


\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{fig/SimRenderExamples.pdf}
  \caption{Rendering successful trajectories with appearance randomization.} % for sim2real.}
  \label{fig:sim-render-examples}
\end{figure}

==> Archive/fig_text/state_distillation_scaling.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
%   \centering
%   \vspace{-5pt}
%   \includegraphics[width=0.4\textwidth]{fig/scaling.pdf}
%   \vspace{-20pt}
%   \caption{BC distillation scaling with dataset size.}
%   \vspace{-10pt}
%   \label{fig:distillation-scaling}
% \end{wrapfigure}

\begin{figure}
  \centering
  % \vspace{-5pt}
  \includegraphics[width=0.4\textwidth]{fig/scaling.pdf}
  % \vspace{-20pt}
  \caption{BC distillation scaling with dataset size.}
  % \vspace{-10pt}
  \label{fig:distillation-scaling}
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/resip_comparison.pdf}
% \caption{Comparison of scaling laws for BC and \methodname. Our method achieves significantly higher performance at lower data costs, enabling more efficient learning of precise manipulation skills.}
% \label{fig:resip_comparison}
% \end{figure}

==> Archive/intro.tex <==
\section{Introduction}

Many robotic manipulation tasks, such as assembly, require both long-horizon planning and high-precision control, which remains a significant challenge~\cite{kimble2020benchmarking, suarez2016framework, lee2021ikea, heo_furniturebench_2023, zhao_rss23_aloha}. As an example, consider the furniture assembly task depicted in \autoref{fig:overview} (Left), where the robot needs to perform a sequence of steps: grasp, then re-orient the table leg into the correct pose, insert the leg, and finally screw the leg into place. This representative long-horizon task spans several task stages over hundreds of timesteps, each dependent on the successful completion of the previous. Small imprecisions at any stage can compound and result in task failure, underscoring the need for reliable execution of each skill in the sequence.

Behavior cloning (BC) is a popular approach for teaching robots various manipulation skills~\cite{pomerleau1988alvinn, schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, zhang2018deep, brohan2022rt, jang2022bc, zhao_rss23_aloha, drolet2024comparison, torne2024reconciling_rialto}. Recent innovations in BC, such as diffusion models~\cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking (predicting a sequence of future actions)~\cite{lai2022action, zhao_rss23_aloha, janner_planning_2022, chi_diffusion_2023}, have enabled learning long-horizon, complex behaviors from demonstrations~\cite{ankile2024juicer, drolet2024comparison}. However, our analysis shows fundamental limitations in BC when applied to tasks requiring high precision: performance saturates with increasing data. For example, the success of a diffusion-based BC model on an insertion task shown in \autoref{fig:overview} (Left) plateaus at $\sim$80\% even with 100,000 demonstrations (\autoref{fig:overview}; right). Other recent work finds similar performance saturation~\cite{ross2010efficient, yu2024lucidsim, zhao2024aloha}.


We hypothesize that the performance saturation results from two issues: (i) compounding errors originating from distribution shift as the policy operates on states that increasingly deviate from those seen during training~\cite{ross2010efficient}.
%
(ii) The use of action-chunking which enables long-horizon control at the cost of reactivity necessary for reliable execution by rolling out each action chunk open-loop~\cite{liu2024bidirectional}. Therefore, we posit that chunked BC policies are best considered ``planners'' rather than reactive controllers. For instance, in the \oneleg{} assembly task shown in \autoref{fig:overview} (left), specific ``bottleneck'' states \pulkit{what is bottleneck state is not defined}, like insertions, require precise actions at specific time steps. If these critical moments fall within an action chunk, the BC policy cannot make real-time adjustments to compensate for disturbances during execution or inaccuracies in the planned actions.


Reinforcement Learning (RL) is a standard solution to the suboptimal performance of BC polices~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}. RL fine-tuning effectively overcomes the problem of distribution shifts by generating training data for states visited by the policy. However, recent advancements in BC architectures present new challenges for direct RL fine-tuning. The main issues are that the structure of diffusion models (iterative refinement) and action-chunked policies (resulting in a large action space) make standard RL algorithms unstable (see \autoref{sec:experiments-fine-tuning}) or require significant architectural modifications~\cite{black2023training, drolet2024comparison, ren2024diffusion}.

Instead of invoking RL, one can overcome distribution shift by leveraging an expert and training with supervised learning such as the Dataset Aggregation (DAgger)~\cite{ross2011reduction} algorithm. Our experiments show with roughly ~2000 demonstrations, a DAgger style approach achieves a 90\% success rate on the \oneleg{} task (\autoref{fig:overview})---a significant improvement over pure BC but still 8\% below the expert. One challenge in using DAgger is that it assumes an expert who can be queried on demand, which is usually unavailable. However, another significant challenge is the performance saturation of DAgger, which we attribute to the lack of reactivity because each action chunk is executed in an open-loop fashion. 

Our key insight is that action-chunked BC policies function more like ``trajectory planners'' than reactive controllers. To mitigate both distribution shift and lack of closed-loop control, we use a simple method of augmenting a frozen, chunked BC model with a small, single-step residual policy~\cite{silver2018residual, johannink2019residual, alakuijala2021residual, davchev2022residual, carvalho2022residual, shafiullah2022behavior_bet, haldar2023teach_fish_residual, lee2024behavior_vqbet} trained via on-policy RL (\autoref{fig:residual-diffusion}), termed \methodname{} (\textit{Resi}dual for \textit{P}recise Manipulation). Unlike prior residual frameworks, the BC policy generates trajectory segments at coarse temporal resolution ($\sim$1 second), while the residual predicts closed-loop corrections at each control step ($\sim$0.1 second). 

\methodname{} addresses both challenges faced by BC methods: the RL-trained residual overcomes distribution shifts and by closing the sensorimotor loop more frequently it lends reactivity by enabling precise adjustments that chunked policies cannot provide. Using only a sparse task-completion reward, this approach achieves a 98\% success rate starting with just 50 expert demonstrations on the \oneleg{} task---an 18 percentage point improvement over BC with 100K demonstrations.

Since our method relies on training RL policies, our learning pipeline heavily relies on simulation. Applying our pipeline requires constructing a digital twin of the real-world use case (i.e., real-to-sim~\cite{torne2024reconciling_rialto}), training with \methodname{}, and finally transferring the trained policy to the real world. While our focus in this paper is on \methodname{} and highlighting the performance saturation of purely BC methods, our experiments demonstrate the entire pipeline on several challenging assembly tasks.


==> Archive/intro_old.tex <==
\section{Introduction}
Many robotic manipulation tasks, such as assembly, require both long-horizon planning and high-precision control, which remains a significant challenge~\cite{kimble2020benchmarking, suarez2016framework, lee2021ikea, heo_furniturebench_2023, zhao_rss23_aloha}. As an example, consider the furniture assembly task depicted in \autoref{fig:overview} (Left), where the robot needs to perform a sequence of steps: grasp, re-orient the table leg into the correct pose, insert the leg, and finally screw the leg into place. This representative long-horizon task spans hundreds of timesteps, with each stage dependent on the successful completion of the previous. Small imprecisions at any stage can compound and result in task failure, underscoring the need for reliable execution of each skill in the sequence.

Behavior cloning (BC) is a popular approach for teaching robots various manipulation skills~\cite{pomerleau1988alvinn, schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, zhang2018deep, brohan2022rt, jang2022bc, zhao_rss23_aloha, drolet2024comparison}. Recent innovations in BC, such as diffusion models \cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking \cite{lai2022action, zhao_rss23_aloha, janner_planning_2022, chi_diffusion_2023}, have improved learning long-horizon, complex behaviors from demonstrations~\cite{ankile2024juicer, drolet2024comparison}. However, our analysis shows fundamental limitations in BC when applied to tasks requiring high precision: performance saturates with increasing data. For example, the success of a diffusion-based BC model on an insertion task shown in \autoref{fig:overview} (Left) plateaus at $\sim$80\% even with 100,000 demonstrations (\autoref{fig:overview}; right). Other recent work finds similar performance saturation~\cite{ross2010efficient, yu2024lucidsim, zhao2024aloha}.


We hypothesize that the performance saturation results from two issues: (i) compounding errors originating from distribution shift as the policy operates on states that deviate from those seen during training~\cite{ross2010efficient}. While approaches like Dataset Aggregation (DAgger)~\cite{ross2011reduction} can mitigate distribution shift by collecting on-policy data, such approaches assume an expert who can be queried on demand, which is usually unavailable.
%
(ii) Modern BC policies employ action chunking that predicts a sequence of future actions (i.e., chunk) and executes a sub-sequence of actions open-loop~\cite{liu2024bidirectional} that prevents reactivity necessary for reliable execution. For instance,  in tasks such as furniture assembly, specific ``bottleneck'' states, like insertions, require precise actions at specific time steps. If these critical moments fall within an action chunk, the BC policy cannot make real-time adjustments to compensate for disturbances during execution or inaccuracies in the planned actions. This inability to correct actions can lead to failures in high-precision tasks. Therefore, we posit that chunked BC policies are best thought of as ``planners'' rather than reactive controllers.


% \idan{didn't we talked about removing this paragraph}
% Given these fundamental limitations of BC, one might consider using Reinforcement Learning (RL) instead, as it promises to autonomously learn corrective behaviors through interaction and exploration guided by a reward function~\cite{kober2013reinforcement, schulman_proximal_2017}. RL has been effective in training robust reactive controllers that can handle a wide array of tasks~\cite{andrychowicz2020learning, kalashnikov2018scalable, margolis2024rapid, torne2024reconciling_rialto, chen2023visual}. However, applying RL to solve complex, long-horizon, and precise tasks like robotic assembly requires extensive reward engineering that can be difficult and time-consuming \cite{park2024automatic}.

% Present BC + RL as a possible solution
% A natural way to overcome this is to leverage the strengths of BC and RL together to reduce human effort in obtaining reliable policies. Applying BC to a set of human demonstrations learns a reasonable prior that enables non-zero success rates on the target task, which mitigates the central challenge of exploration during RL training. RL can then leverage this pre-training prior to speed up self-improvement and learning reliable corrective behaviors by collecting on-policy data through trial and failure in the environment. \idan{in this paragraph, you describe how BC can help RL, but isn't it better to focus on how RL can help BC? especially if we remove the previous paragraph}

% A natural way to overcome this is to leverage the complementary strengths of BC and RL together to reduce human effort in obtaining reliable policies. While BC can learn a reasonable prior from human demonstrations, it does not have a mechanism for improving beyond the data distribution. RL addresses this limitation through self-improvement and learning reliable corrective behaviors by collecting on-policy data through trial and error in the environment. At the same time, the BC prior helps mitigate the central challenge of exploration during RL training.

% % State that it's a tried and true recipe, but modern innovations complicate
% While combining BC and RL has a long history \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}, the recent advancements in BC architectures present new challenges for fine-tuning the learned policy with RL. The structure of diffusion models (iterative refinement) and action-chunked policies (large effective action spaces) complicate the application of standard RL algorithms, often leading to instability or requiring significant architectural modifications~\cite{black2023training, drolet2024comparison, ren2024diffusion}.

% A natural way to overcome this is to leverage the complementary strengths of BC and RL together to reduce human effort in obtaining reliable policies. While BC can learn a reasonable prior from human demonstrations, it does not have a mechanism for improving beyond the data distribution. RL addresses this limitation through self-improvement and learning reliable corrective behaviors by collecting on-policy data through trial and error in the environment. At the same time, the BC prior helps mitigate the central challenge of exploration during RL training.

% State that, as we know, fine-tuning BC with RL is a tried-and-true recipe, but modern innovations complicate
A standard solution to the suboptimal performance of a BC policy is to improve the policy with Reinforcement Learning (RL) \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}. RL fine-tuning effectively overcomes the problem of distribution shifts by generating training data for states visited by the policy. However, recent advancements in BC architectures present new challenges for direct RL fine-tuning. The main issues are that the structure of diffusion models (iterative refinement) and action-chunked policies (resulting in a large action space) make standard RL algorithms unstable or require significant architectural modifications~\cite{black2023training, drolet2024comparison, ren2024diffusion}. Even if the action-chunked trajectory planner with RL is successfully improved, each chunk will be executed open-loop, which may still result in failures. \pulkit{Good place to talk about the Figure and results}

To mitigate the effect of open-loop execution of chunks, we use a simple method of augmenting a frozen, chunked BC model with a small, single-step residual policy~\cite{silver2018residual} trained via on-policy RL (\autoref{fig:residual-diffusion}), termed \methodname{} (\textit{Resi}dual for \textit{P}recise Manipulation). The BC policy generates short trajectories at coarse temporal resolution ($\sim$1 second), while the residual provides fine-grained, closed-loop corrections at each control step. This approach naturally addresses both key challenges: the RL-trained residual operates on policy to overcome distribution shift. At the same time, its closed-loop nature enables the precise adjustments that chunked policies cannot provide. The residual policy observes each state and the planned action, making real-time corrections crucial during bottleneck stages like insertions. The system is trained with a sparse task-completion reward, avoiding reward engineering.

% Summarize what this method enables
We evaluate \methodname{} on high-precision manipulation tasks from the challenging FurnitureBench~\cite{heo_furniturebench_2023} and Factory~\cite{yash_factory2022_rss} benchmarks and two hand-designed tasks.
% 
\pulkit{It will be nice to knit these results in the initial paragraphs of the intro itself instead of leaving for the end.} 
Our experiments demonstrate that \methodname{} outperforms pure BC methods and traditional RL fine-tuning, for example, achieving success rates up to $\sim$98\% starting from 50 demonstrations for the \oneleg{} task. At the same time, increasing data for BC saturates at $\sim$80\% success with 100K demonstrations for the same task.
%
We also find that by combining \methodname{} with straightforward applications of teacher-student distillation, visual domain randomization, and co-training, we can transfer policies from simulation to vision-based policies for physical robot hardware.



==> Archive/intro_v4.tex <==
\section{Introduction}

Robotic manipulation tasks that require both long-horizon planning and high-precision control, such as assembly, remain a significant challenge in robotics~\cite{kimble2020benchmarking, suarez2016framework, lee2021ikea, heo_furniturebench_2023, zhao_rss23_aloha}. As an example, consider the furniture assembly task depicted in \autoref{fig:overview} (Left), where a robot performs assembly by sequentially grasping and then re-orienting a table leg into the correct pose, performing a precise insertion, and finally screwing the leg in place. This representative task involves executing a specific sequence of skills over hundreds of timesteps, with each stage dependent on the successful completion of the previous. Small imprecisions anywhere in the chain can lead to task failure, underscoring the need for reliable execution of diverse skills in the sequence.

Behavior cloning (BC) is a popular approach for teaching robots various manipulation skills~\cite{pomerleau1988alvinn, schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, zhang2018deep, brohan2022rt, jang2022bc, zhao_rss23_aloha, drolet2024comparison}. Recent innovations in BC, such as diffusion models \cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking \cite{lai2022action, zhao_rss23_aloha, janner_planning_2022, chi_diffusion_2023}, have improved learning long-horizon, complex behaviors from demonstrations~\cite{ankile2024juicer, drolet2024comparison}.
%
However, our analysis shows fundamental limitations in BC when applied to tasks requiring high precision. For example, in the insertion task shown in \autoref{fig:overview} (Left), a diffusion-based BC model achieves a success rate of $\sim$50\% with a handful of demonstrations, but performance plateaus even when scaling up to large datasets (e.g., 100,000 demonstrations), reaching only about $\sim$80\% success, as seen in \autoref{fig:overview} (Right). Other recent work finds similar performance saturation~\cite{ross2010efficient, yu2024lucidsim, zhao2024aloha}.
%

We hypothesize that this saturation occurs because of two issues: First, BC methods suffer from compounding errors due to distributional shifts; the policy operates on states that deviate from those seen during training, leading to errors that accumulate over time~\cite{ross2010efficient}. While approaches like Dataset Aggregation (DAgger)~\cite{ross2011reduction} can mitigate this error mode by collecting on-policy data, such approaches assume an expert who can be queried on demand, which is usually unavailable.
%
Second, modern BC policies, particularly ones employing action chunking, act more like open-loop ``planners'' than reactive controllers. Chunked BC policies are limited in compensating for noise and disturbances (i.e., non-reactive) because each chunk runs in an open loop. In tasks such as furniture assembly, certain ``bottleneck'' states, like insertions, require precise actions at specific time steps. If these critical moments fall within an action chunk, the BC trajectory planner cannot make real-time adjustments to compensate for inaccuracies in the planned actions. This inability to correct actions leads to task failure in high-precision tasks.

% Present RL as a possible solution
Reinforcement Learning (RL) promises to autonomously learn corrective behaviors through interaction and exploration guided by a reward function~\cite{kober2013reinforcement,schulman_proximal_2017}. RL has been effective in training robust reactive controllers that can handle a wide array of tasks~\cite{andrychowicz2020learning, kalashnikov2018scalable, margolis2024rapid, torne2024reconciling_rialto, chen2023visual}.
However, applying RL to solve complex, long-horizon, and precise tasks like robotic assembly requires extensive reward engineering that can be prohibitively difficult and time-consuming \cite{park2024automatic}. RL requires vast data, which is costly to collect, particularly in real-world settings.
% Present BC + RL as a solution

We present a way to leverage the strengths of BC and RL that reduces human effort in obtaining reliable policies by building on recent advances in BC methods and sim-to-real RL training. BC learns a ``planner'' that predicts trajectory segments (i.e., an action chunk executed open loop) conditioned on the agent's observations from a small set of demonstrations, providing a skeleton for RL training. RL augments the BC-learned planner with a closed-loop controller capable of fine-grained corrections that mitigate the limitations of open-loop action chunk execution and collects on-policy data to ensure reliable plan execution.
% State that it's a tried and true recipe, but modern innovations complicate
While combining BC and RL has a long history \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}, the recent advancements in BC architectures present new challenges for fine-tuning the learned policy with RL.
% Provide an example of why the modern architecture complicates matters
The structure of diffusion models (iterative refinement) and action-chunked policies (large action spaces) complicate the application of standard RL algorithms, often leading to instability or requiring significant architectural modifications~\cite{black2023training, drolet2024comparison, ren2024diffusion}.

% Present our solution
We propose a simple yet effective method to combine the strengths of modern chunked BC and on-policy RL controllers, called \methodname{} (\textit{Resi}dual for \textit{P}recise Manipulation), shown in \autoref{fig:residual-diffusion}. Our key insight is recognizing that modern BC policies function as trajectory planners that generate action sequences but crucially lack the fine-grained reactivity and corrections required for reliable execution. We introduce closed-loop corrections by augmenting a frozen, chunked BC model with a small, single-step residual policy trained via on-policy RL. The residual policy observes each state and action and predicts a corrective action to be added to the action predicted by the  BC model.
%
This design sidesteps the difficulties of fine-tuning complex BC models with RL while addressing BC's limitations. First, the residual RL policy operates on-policy, learning reactive behaviors directly through interaction with the environment, thus overcoming issues of distributional shift. Second, providing closed-loop control enables real-time adjustments during task execution, improving robustness and precision, especially in bottleneck stages like insertions. Finally, the residual training is supervised with a sparse task-completion reward, avoiding reward engineering.

% Summarize what this method enables
We evaluate \methodname{} on a range of high-precision manipulation tasks from the challenging FurnitureBench~\cite{heo_furniturebench_2023} and Factory~\cite{narang2022factory} benchmarks. 
%These tasks involve sequences of precise insertions, rearrangements, and long-horizon multi-part interactions over hundreds of timesteps. 
Our experiments demonstrate that \methodname{} outperforms pure BC methods and traditional RL fine-tuning, achieving success rates up to $\sim$97\% starting from 50 demonstrations while only BC  saturates at $\sim$80\% success with 100K demonstrations.
%
We also find that \methodname{}, combined with straightforward applications of teacher-student distillation, visual domain randomization, and co-training, we can transfer policies from simulation to a real robot using RGB observations.

% Wrap up
%In summary, we highlight the limitations of modern BC methods in precise manipulation tasks. We present a straightforward yet effective solution that leverages the strengths of both chunked BC and closed-loop RL. By augmenting BC-trained local trajectory planners with residual RL controllers, \methodname{} achieves higher performance with less human data, enabling robots to perform complex, high-precision tasks reliably.

\iffalse{}

% === Version after another round of Pulkit's comments

\subsection{Introduction V4}


Robotic systems struggle with tasks simultaneously requiring high precision, robustness to varied initial conditions, and the ability to operate directly from RGB sensors~\cite{kimble2020benchmarking, suarez2016framework, lee2021ikea, heo_furniturebench_2023, zhao_rss23_aloha}.
%
Autonomous assembly exemplifies these challenges, where robots must manipulate and precisely fit together multiple parts without relying on tight and specialized fixtures for precise and consistent positioning.
%
Behavior cloning (BC) is a popular approach for teaching robots complex manipulation tasks~\cite{pomerleau1988alvinn, schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, zhang2018deep, brohan2022rt, jang2022bc, zhao_rss23_aloha, drolet2024comparison}. Recent innovations in BC, such as diffusion models \cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking \cite{lai2022action, zhao_rss23_aloha, janner_planning_2022, chi_diffusion_2023}, have enabled learning long-horizon, complex behaviors from demonstrations that standard policy architectures cannot~\cite{ankile2024juicer, drolet2024comparison}.


Despite its success, BC faces significant challenges in tasks that require precise alignments and precision, like furniture assembly (e.g., \autoref{fig:overview} \textcolor{rlcolor}{\textbf{(A)}}). To achieve the necessary precision, BC models must closely mimic expert policies. For long-horizon tasks, this becomes exceedingly difficult because of compounding errors.
%
While increasing the number of expert demonstrations can help, we observe that performance quickly saturates (\autoref{fig:overview} \textcolor{bccolor}{\textbf{(B)}}), requiring prohibitively large and costly datasets to achieve even moderate success rates~\cite{yu2024lucidsim,zhao2024aloha}.
%
This saturation arises because BC relies solely on imitation but lacks the supervision to learn how to correct mistakes that will inevitably occur.
%
Even with limited environment interaction via DAgger, performance improves beyond what imitation alone achieves, highlighting the need for interactive learning of corrective behaviors (\autoref{fig:overview} \textcolor{bccolor}{\textbf{(B)}}).

\lars{Where's a good place to mention the problem with action-chunked policies being partially open-loop?}


A common way to cheaply achieve high performance and reactive policies is to leverage simulation and reinforcement learning (RL) to autonomously collect and learn from large amounts of data and environment interaction. While combining BC and RL has a long history \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}, the recent advancements in BC architectures present new challenges for direct application of traditional RL methods. For instance, training diffusion with RL can require complex reformulation of the de-noising process to enable policy gradient estimation~\cite{black2023training}. Our experiments corroborate the finding that action chunking makes direct RL fine-tuning harder and unstable due to the expanded action space dimension induced by chunking~\cite{drolet2024comparison}. \lars{Explicitly reference our own experiments with training chunked MLP's and chunked residual models?}


This paper proposes a simple yet effective scheme to augment state-of-the-art BC models with RL, called \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation).
%
The key insight is that by training an unchunked residual policy on top of a frozen chunked BC model, we sidestep the challenges of fine-tuning the complex SoTA BC architectures and can reintroduce fully closed-loop reactivity for action-chunked models.
%
Our approach uses on-policy RL with sparse task rewards to train residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual, zeng2020tossingbot}, starting from a handful of demonstrations.
%
The residual model is a small feed-forward network that observes the current state and the current BC-predicted action and predicts corrections at every timestep. This design preserves the strong BC model's learned behaviors while allowing for stable on-policy RL training. The result is a more reactive, fully closed-loop policy suited for precise manipulation tasks.


We evaluate our method on a set of tasks involving sequences of precise insertions, rearrangements, and long-horizon multi-part interactions like furniture assembly from the challenging FurnitureBench \cite{heo_furniturebench_2023} task suite and peg insertion from the Factory~\cite{narang2022factory} task suite (e.g., \autoref{fig:overview} \textcolor{daggercolor}{\textbf{(C)}}).
%
Our results show that \methodname{} is surprisingly effective and outperforms pure BC and alternative RL fine-tuning approaches across the tested tasks.

To make our approach applicable to real-world manipulation tasks, we first train policies using reinforcement learning (RL) in simulation with access to the full environment state, which facilitates efficient learning. Since this state information is unavailable in real-world scenarios, we distill these learned behaviors into a real-world policy using only RGB observations. This distillation process involves creating a large synthetic dataset of rendered images from the simulation, augmented with a few real-world demonstrations to bridge the perception gap between simulation and reality.

By leveraging the data efficiency of RL in simulation and refining the policy with real-world data, we successfully adapt the learned behaviors for real-world deployment. The resulting policies improve performance over ones trained from real-world demos alone.

In summary, this paper highlights the limitations of BC in learning precise manipulation skills. We present an approach that combines BC and RL's strengths to overcome these limitations using SoTA BC architectures with residual RL. By addressing the limitations of pure BC and enabling RL fine-tuning of modern policy architectures, \methodname{} achieves high-performance, corrective behaviors for complex assembly tasks in simulation and in the real world while requiring modest amounts of human data.

\lars{Should we mention that we find that the low frequency of policy makes it more prone to errors and online perturbations and that MLP as base doesn't work well at all?}


% \iffalse{}

% === Version after a couple of iterations on Pulkit's comments w/ Zhang-Wei's comments ===


Robotic systems struggle with tasks simultaneously requiring high precision, robustness to varied initial conditions, and the ability to operate directly from RGB sensors \zw{is it true? need reference or elaboration}. Autonomous assembly exemplifies these challenges, where robots must manipulate and precisely fit together multiple parts without relying on tight and bespoke \zw{seems a esoteric word haha} fixtures for precise and consistent positioning

Behavior cloning (BC) has re-emerged \zw{again, "re" emerging needs a more context.} as a popular approach for teaching robots complex manipulation tasks~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, jang2022bc, zhao_rss23_aloha}. Recent innovations in BC, such as diffusion models \cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking \cite{zhao_rss23_aloha}, have enabled learning long-horizon, complex behaviors from modest numbers of demonstrations that are infeasible with standard policy architectures \zw{seems an argument about new arch enables more efficient learning - is it necessary to say this? reading this sentence makes me expect a story about data efficiency on the demonstration}. However, BC has limitations for precise manipulation tasks~\cite{ankile2024juicer} \zw{Define "precise" manipulation. It's important since it's the main problem studied in this paper.}.


One of the main challenges with BC is that its performance has been found to saturate with increasing expert demonstrations, and achieving even moderate success rates may require prohibitively large and costly demonstration datasets~\cite{yu2024lucidsim,zhao2024aloha} \zw{Not connected to precise manipulation. The fact that BC has a limitation on precise manipulation doesn't mean that we need more expert demonstration.}. This is particularly problematic since dataset size scales linearly with human effort~\cite{park2024automatic}.
%
Furthermore, our analyses suggest that BC struggles to generalize for precise manipulation tasks as it does not learn to correct mistakes by learning solely from imitating expert actions \zw{now it comes back again to precise manipulation. the argument of performacne saturation got cut off. I suggest building a stronger connection between performance saturation and difficulty of precise manipulation. One idea: Only a few trajectories or policies lead succeess in precise manipulation. For instance, assembling furniture demands precise screw placement, leaving little room for error in positioning. In contrast, placing plates in a drawer is less exact, allowing for more flexibility and mistakes, thus requiring lower precision. In high-precision tasks, models must closely follow expert policies, which is difficult with limited demonstrations. More expert demonstrations can help the BC policy learn precision, but improvement plateaus after a certain number of demos. This may be because BC learning doesn't teach the model to correct its own mistakes. BC models are imperfect and always have irreducible errors due to limited capacity [cite]. If a BC model makes a mistake early in an episode, it enters states the expert never demonstrated, since the expert didn’t make those errors. Therefore, the BC model must learn how to act in those unobserved states. Then introduce DAgger and RL}. Even with moderate environment interaction through DAgger, performance improves beyond what imitation alone enables (see \autoref{fig:overview} (B)).

A common way to cheaply achieve high performance and reactive policies \zw{is mentioning reactive policy important here?} is to leverage simulation and reinforcement learning (RL) to autonomously collect and learn from large amounts of data and environment interaction. While combining BC and RL has a long history \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}, the recent advancements in BC architectures present new challenges for direct application of traditional RL methods. Specifically, innovations like diffusion policies and action chunking, complicate the process of RL fine-tuning~\cite{drolet2024comparison}. \zw{how they make RL complicated is not explained. I suggest you pick one problem that make RL finetuning complicated and then hook on this problem to expand the motivation of using residual policy.}


This paper proposes a simple yet effective scheme to augment state-of-the-art BC models with RL. The approach involves training residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual, zeng2020tossingbot} with on-policy RL and sparse task rewards to improve upon pure BC from a handful of demonstrations. \zw{This says how you implement but didn't say why you implement in this way. The most critical part of the intro is the key insight of your idea -- Why residual policy makes finetuning easier?} The residual model observes the latest state observation and the current predicted action and predicts a correction online.

The approach, which we call \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation), side-steps the challenges of fine-tuning SoTA BC methods altogether by keeping the base model frozen during RL training. This also allows for running the residual policy at a higher frequency than the chunked base model \zw{the low frequency issues of prior works weren't discussed}, resulting in a more reactive, fully closed-loop policy.


We evaluate our method on a set of tasks involving sequences of precise insertions, rearrangements, and long-horizon multi-part interactions like furniture assembly from the challenging FurnitureBench \cite{heo_furniturebench_2023} task suite and peg insertion from the Factory~\cite{narang2022factory} task suite.
%
Our results show that \methodname{} significantly outperforms pure BC and alternative RL fine-tuning approaches across these tasks.

To show the usefulness of our approach, we distill the behaviors learned through RL in simulation into a real-world policy, solving furniture assembly from RGB observations only \zw{seems to presume you learn with full env state in sim and so you need to distill the model to RGB policy so as to deploy in the real world. is that fair to assume all readers of ICRA know this assumption?}. We do this by synthesizing a large set of demonstrations from a simulator-trained RL policy that we combine with a limited set of real-world demonstrations. \zw{again, this is how you implement so can be left in the later sections.} This allows us to leverage the data efficiency of RL and simulation while bridging the sim-to-real gap. The resulting policies enable capabilities not possible from BC alone.

In summary, this paper highlights the limitations of BC in learning precise manipulation skills. We present an approach that combines BC and RL's strengths to overcome these limitations using SoTA BC architectures with residual RL. By addressing the limitations of pure BC and enabling RL fine-tuning of modern policy architectures, \methodname{} achieves high-performance, corrective behaviors for complex assembly tasks in simulation and in the real world while requiring modest amounts of human data.





% === Original version with initial Pulkit's comments ===


\pulkit{Suggestions
\begin{itemize}
    \item Robots struggle to learn tasks robustly and those that require high precision, etc etc.
    \item BC is a popular approach. Our analysis reveals fundamental limitations of BC -- the asymptotic performance is limited, and the cost is too high. Have Figure 1 show this. 
    \item How do we achieve high-asymptotic performance cheaply? Leverage simulation and automatically collect data using RL. 
    \item BC + RL has had a long history. However, with new BC methods past methods can't directly be applied -- explain why. 
    \item We devise a simple scheme (call it simple so that people don't think we are claiming methodological innovation per se) -- that augments the latest and greatest BC models with a residual model trained with RL. 
    \item Explain why we want a residual model and how we overcome other issues typical in RL Problem -- again nothing new here. But good to say explicitly. 
    \item End by referring back to Figure 1 -- saying look at scaling laws now -- we are much better performance at much cheaper. 
    \item Also have an example of the task in this Figure. 
    \item Conclude by saying evaluation is performed on Furniture bench. 
\end{itemize}
}


Despite significant advancements in robot learning, autonomous systems still struggle with manipulation tasks requiring high precision, robustness to a wide array of initial conditions, and operation directly from RGB sensors. 
%
An example of such a challenging scenario is autonomous assembly, where a robot is presented with a set of multiple parts to pick up and precisely fit together.
%

Such systems typically utilize engineered fixtures for consistent initial part positioning, making assembly robots expensive and impractical to adapt across diverse tasks.
%
Learning to perform these tasks from vision can improve the adaptability and robustness of such systems, but the high-precision, contact-rich nature of such tasks poses substantial challenges for current robotic learning frameworks. \pulkit{Not required -- too much details that are known, irrelevant -- come to the point directly} % Learning-based Vision-based control has the potential to

Behavior cloning (BC) has re-emerged as a popular technique for acquiring manipulation control policies~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational,jang2022bc, zhao_rss23_aloha}. This is largely due to the ease of directly specifying complex tasks by providing demonstrations.
%
However, BC requires large amounts of costly demonstration data to enable generalization to different scene configurations~\cite{jang2022bc}.
%
BC-trained policies are also often limited by the nature of human demonstrations that \emph{directly} achieve the task. This can mean such policies never learn to perform \emph{corrective} actions that recover from deviations that inevitably occur during deployment. \pulkit{This point is not made strongly -- say that we show that for precise problems, the scaling is bad -- in fact it saturates, or the amount of data that is required is these many trajectories translating into this much cost XXX amount of dollars. }
%
Reinforcement learning (RL) offers a complementary paradigm, wherein locally corrective behavior can be learned by exploring and discovering action sequences that lead to downstream task success \pulkit{RL doesn't offer locally corrective behavior -- RL is just a way of learning policies.}. 
%
Although RL offers appealing advantages, many of its successes in robotics depend on carefully crafted reward functions that may sacrifice generality across tasks~\cite{kumar2021rma, jiang2024transic_assembly, chen2023visual}. 


A common mitigation is to bootstrap the RL process by starting with a small set of demonstrations~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt} -- by initializing with a policy that occasionally solves the task, supervision from simple sparse rewards can be enough for RL to progress effectively. \pulkit{Again I think we are going off the topic. And also consider citing Gabe's papers too and recent position paper from Younghyo/Gabe} \lars{The position paper added. What Gabe papers would be most relevant here?}
%
However, naively trained BC policies may fail to achieve any meaningful success with a small number of demonstrations in complex tasks like assembly~\cite{ankile2024juicer} \pulkit{Flow is broken}.
%
Innovations in policy design, such as diffusion models~\cite{chi_diffusion_2023} and action chunking~\cite{zhao_rss23_aloha}, can alleviate some of this difficulty and enable non-zero success rates for challenging tasks using a modest number of demonstrations~\cite{ankile2024juicer, heo_furniturebench_2023}. \pulkit{Circular -- we talk BC, then RL and then again BC -- not a good way to frame the paper.}
%
However, introducing these modern architectural components makes it difficult to perform fine-tuning with RL. \pulkit{But is the goal fine-tuning with RL? I think the goal is different -- how to reduce cost of the BC thing and to say the scaling laws are really bad. They can't achieve high performance. We want to both achieve high performance and do it at a low-cost.}
%
For instance, training diffusion with RL can require complex reformulation of the de-noising process to enable policy gradient estimation~\cite{black2023training}. 
%
We also find that action chunking tends to make direct RL fine-tuning harder and unstable due to the expanded action space dimension induced by chunking. \pulkit{Unnecessary emphases on action chunking in my opinion and missing the bigger picture.}


In this paper, we propose adaptations to the BC + RL pipeline that facilitate its application to complex tasks like furniture assembly~\cite{heo_furniturebench_2023} \pulkit{Is this the point of the paper? This benchmark is used to evaluate a hypothesis - - what is the hypothesis?}. Our key contribution is to enable RL fine-tuning to work with modern advancements like diffusion policies and chunked action predictions \pulkit{No this is not the contribution, this is the technical innovation which enabled the contribution. It's also good to clearly acknowledge the vast literature of IL + RL fine-tuning and say what is different here in the technical details. But the main contribution of the paper is not really stated.} \lars{The contribution then is that we show how BC is limited and offer a way to get precision and robustness cheaply?}.
%
We first provide an analysis and empirical evidence supporting the need for action chunking and expressive policy architectures to achieve success rates high enough to bootstrap RL.
%
We then propose training residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual} with on-policy RL and sparse task rewards to improve upon pure BC, an approach we term \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation). These residual models learn to predict corrective actions that more reliably achieve high precision. In this way, we side-step the aforementioned challenges of directly altering the base policy with RL, while improving overall task success. \pulkit{Why residual is not really motivated -- seems arbitrary -- many people have done this before.}
%
Finally, by distilling behaviors learned with RL into a large synthetic dataset of trajectories and combining them with a limited set of real-world demonstrations, we showcase the benefits of our residual learning approach, \methodname, in enabling real-world assembly policies that operate directly from RGB images \pulkit{Again this is a side point, not the main point.} \lars{Should it not feature in the intro?}.

\fi


==> Archive/intro_versions/intro_as.tex <==
\section{Introduction}

% We want precise, long-horizon manipulation that's robust -- Assembly is a helpful testbed due to inherent challenges and has short-term practical value
One of the major remaining challenges in robotics is to perform manipulation tasks with high precision and robustness to diverse initial conditions. 
%
Autonomous assembly is a useful application domain for progressing on this front, as assembly tasks pose several representative difficulties and requirements -- high precision, long horizons, and interaction with objects to achieve user-specified geometric alignments.
%
In addition, developing pipelines for teaching robots to assemble various constructs while allowing parts to arrive with large initial pose variability and not requiring custom-designed part fixtures can also deliver high short-term practical value to the manufacturing industry.
%
However, methods for building such systems are still limited. Existing approaches remain overly specific to particular tasks, objects, and environments and typically require extensive human engineering effort~\cite{prior_work_in_assembly}. 
%
This paper proposes techniques that combine imitation and reinforcement learning to quickly and straightforwardly teach robots new assembly tasks with random initial part pose layouts while operating directly from RGB images in the real world.

% Technical -- IL is powerful and very popular right now, mainly because it's so easy to use to get something up and running, it's so general across tasks, and performance can keep improving as the amount of data increases.  
Imitation learning (IL), and more specifically behavior cloning (BC), has re-emerged as one of the most popular techniques for acquiring manipulation control policies.
%
This is due to factors like technical simplicity, the intuitive user interface offered in programming a robot's behavior by directly performing it oneself, and BC's general applicability to many tasks that remain challenging to achieve using other techniques~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, jang2022bc, zhao_rss23_aloha}.
%
IL has also grown in broader appeal due to its alignment with other data-centric supervised learning methods that have become de-facto pipelines in other areas like Natural Language Processing and Computer Vision, where system performance scales well with the amount of training data that can be obtained~\cite{chinchilla, scaling_laws_papers}.
% 
Substantial effort has recently been applied in robotics and manipulation toward demonstrating that large-scale data collection and imitation learning can power similar performance gains in robotics~\cite{}\lars{RT-1/2/X}.
%
We hypothesize similar performance gains can be attained in assembly tasks via large-scale imitation learning.
%
However, such large-scale data often comes at a very high cost, as humans must set up and reset scenes, and collect expert demonstrations by manually performing the tasks on a physical system many times in the real world.

% V2
Because human-provided demonstrations are expensive at scale, we want to find more scalable sources of expert data for visual manipulation policy learning.
%
One insight is that if we could obtain an ``already proficient agent,'' such as one trained via Reinforcement Learning (RL), rollouts from this agent could be an effectively infinite source of new data.
%
However, this becomes a circular problem, as it is also challenging to obtain such a proficient agent as RL is still only practical in the real world in narrow settings (requires resets, engineered setups for providing reward functions, constrained to real-time data collection, hardware platform limited, etc.).
%
Furthermore, even if we could train these RL agents in the real world, it is also difficult to collect expert data from them, as the agents must be monitored, successful rollouts must be safely collected, environments must be reset, scenes must be set up and randomized, etc.

These difficulties point toward using simulation for two purposes: (1) it is significantly easier to train RL agents in simulation (faster than real-time and parallelized physics engines, privileged state and geometric information, automatic resets, reward computation, and domain randomization), and (2) it is straightforward to obtain trajectory data from RL agents in simulation (faster computation, safely collect successful policy rollouts). 
%
This pipeline still poses challenges associated with the simulation-to-reality (sim2real) transfer of perception and dynamics. Still, progress has recently been rapid with techniques like domain randomization~\cite{tobin2017domain, other_dr_robotics_successes}, improved physics fidelity and photorealistic rendering~\cite{isaac_gym}, and combining with small amounts of real-world data~\cite{torne2024reconciling_rialto, other_co_training}\lars{Do we need to define co-training more thoroughly somewhere?}. Thus, the main idea of the pipeline explored in this paper is to train performant assembly agents via RL in simulation, collect data from the resulting policy, and train vision-based policies by combining this synthetic data with a small number of real-world demonstrations.

What are the technical challenges? Long horizons, sparse rewards, exploration, and precision still make learning these policies with pure RL in simulation infeasible. However, prior work has shown that behavior cloning combined with SOTA policy architectures, e.g., diffusion policies~\citep{chi_diffusion_2023}, can achieve non-zero success rates on such tasks from small initial demonstration budgets~\cite{ankile2024juicer, heo_furniturebench_2023}. This motivates using BC-trained diffusion policies as a prior to \emph{fine tune} with RL. \anthony{Maybe need to state that directly training diffusion models with RL is not easy? Before saying anything about residual PPO.}\lars{Or something about residual policies being BC policy agnostic and potentially more stable and sample-efficient to train?}
%
We find standard policy gradient reinforcement learning~\cite{schulman_proximal_2017} with residual policies~\cite{silver2018residual, davchev2022residual} can achieve this, even with sparse rewards and long-horizon tasks requiring high precision. 
%
Regarding sim2real difficulties, in assembly settings, CAD models of the objects to be used are often already available from the designers who created the parts, making the requirements of simulation-based content creation less difficult.
%

Overall, our contributions are the following: (1) a technique for fine-tuning diffusion policies trained with behavior cloning using residual policies and imitation-bootstrapped PPO with sparse rewards and (2) a demonstration of a pipeline for converting an RL policy operating on privileged state information into a large, diverse dataset for distilling the learned behaviors into an image-based policy in assembly manipulation domains \anthony{Should reference teacher-student earlier, then contribution (2) becomes ``we demonstrate teacher-student RL + distillation working well for assembly, maybe also combined with sim2real with images}. We compare and evaluate the performance of PPO-trained residual policies with other techniques for fine-tuning BC-trained policies in terms of the final task success rate and coverage of the resulting datasets that can be synthesized. We also analyze how final vision policy performance scales with the amount of data that is used for assembly tasks.
%
Finally, we demonstrate real-world assembly from RGB images by combining datasets synthesized from our pipeline with a small amount of real-world demonstration data.

==> Archive/intro_versions/intro_as2.tex <==
\section{Introduction}

\pulkit{Suggestions
\begin{itemize}
    \item Robots struggle to learn tasks robustly and those that require high precision, etc etc.
    \item BC is a popular new approach. Our analysis reveals fundamental limitations of BC -- the asymptotic performance is limited and the cost is too high. Have Figure 1 -- showing this. 
    \item How do achieve high-asymptotic performance cheaply? Leverage simulation and automatically collect data using RL. 
    \item BC + RL has had a long history. However, with new BC methods past methods can't directly be applied -- explain why. 
    \item We devise a simple scheme (call it simple so that people don't think we are claiming methodological innovation per se) -- that augments the latest and greatest BC models with a residual model trained with RL. 
    \item Explain why we want a residual model and how we overcome other issues typical in RL Problem -- again nothing new here. But good to say explicitly. 
    \item End by referring back to Figure 1 -- saying look at scaling laws now -- we are much better performance at much cheaper. 
    \item Also have an example of the task in this Figure. 
    \item Conclude by saying evaluation is performed on Furniture bench. 
\end{itemize}
}

Despite significant advancements in robot learning, autonomous systems still struggle with manipulation tasks requiring high precision, robustness to a wide array of initial conditions, and operation directly from RGB sensors. 
%
An example of such a challenging scenario is autonomous assembly, where a robot is presented with a set of multiple parts to pick up and precisely fit together.
%
% Such systems typically utilize engineered fixtures for consistent initial part positioning, rather than relying on vision to handle part layouts that may vary and require adaptable grasping and insertion behaviors.
Such systems typically utilize engineered fixtures for consistent initial part positioning, making assembly robots expensive and impractical to adapt across diverse tasks. % , rather than using vision to handle varying part layouts.  % and require adaptable grasping and insertion behaviors.
%
Learning to perform these tasks from vision can improve the adaptability and robustness of such systems, but the high-precision, contact-rich nature of such tasks poses substantial challenges for current robotic learning frameworks. \pulkit{Not required -- too much details that are known, irrelevant -- come to the point directly} % Learning-based Vision-based control has the potential to

Behavior cloning (BC), has re-emerged as a popular technique for acquiring manipulation control policies~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational,jang2022bc, zhao_rss23_aloha}. This is largely due to the ease of directly specifying complex tasks by providing demonstrations. % without requiring simulation environments or real-world RL~\cite{ibarz2021train, dulac2019challenges_real_rl, zhu2020ingredients}.
%
However, BC requires large amounts of costly demonstration data to enable generalization to different scene configurations~\cite{jang2022bc}.
%
% Performance obtained purely by imitating human experts can also be limited if demonstrators fail to provide examples of precise and \emph{corrective} actions that recover from the slight deviations that inevitably occur during deployment.
BC-trained policies are also often limited by the nature of human demonstrations that \emph{directly} achieve the task. This can mean such policies never learn to perform \emph{corrective} actions that recover from deviations that inevitably occur during deployment. \pulkit{This point is not made strongly -- say that we show that for precise problems the scaling is bad -- infact it saturates or the amount of data that is required is these many trajectories translating into this much cost XXX amount of dollars. }
%
Reinforcement learning (RL) offers a complementary paradigm, wherein locally corrective behavior can be learned by exploring and discovering action sequences that lead to downstream task success \pulkit{RL doesn't offer locally corrective behavior -- RL is just a way of learning policies.}. 
%
% A common framework involves training agents with RL in simulation and then distilling the learned behaviors into a perception-based policy with BC.
%
% One such common framework is teacher-student distillation. Typically, a teacher policy is trained in a simulated environment using Reinforcement Learning (RL), benefiting from access to complete state information and the capability to parallelize trials.
% One such common framework is teacher-student distillation. Typically, a teacher policy is trained in a simulated environment using Reinforcement Learning (RL), benefiting from access to complete state information and modern simulators' ability to perform highly parallelized episodic data collection.
%
% This policy then generates successful trajectories to train a sensor-based student policy through Behavior Cloning (BC). 
% The sensor-based student can then be deployed in the real world using sim-to-real techniques. 

% Although it offers appealing advantages, many RL successes in robotics depend on carefully crafted reward functions that may sacrifice generality across tasks in favor of providing sufficiently dense supervision to guide proper task execution~\cite{kumar2021rma, jiang2024transic_assembly, chen2023visual}. % deploying this framework effectively in complex manipulation tasks like assembly remains challenging, as 
% Although RL offers appealing advantages, many of its successes in robotics sacrifice generality across tasks in favor of providing sufficiently dense reward supervision to guide proper task execution~\cite{kumar2021rma, jiang2024transic_assembly, chen2023visual}. % deploying this framework effectively in complex manipulation tasks like assembly remains challenging, as 
Although RL offers appealing advantages, many of its successes in robotics depend on carefully crafted reward functions that may sacrifice generality across tasks~\cite{kumar2021rma, jiang2024transic_assembly, chen2023visual}. 

% deploying this framework effectively in complex manipulation tasks like assembly remains challenging, as 
%
% To mitigate these issues, it is common to leverage a small set of initial human demonstrations to bootstrap the RL process~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt} -- by starting with a policy that occasionally solves the task, supervision from simple sparse rewards can be enough for RL to progress effectively.
% To mitigate these issues, it is common to initialize with a small set of demonstrations to bootstrap the RL process~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt} -- by starting with a policy that occasionally solves the task, supervision from simple sparse rewards can be enough for RL to progress effectively.
A common mitigation is to bootstrap the RL process by starting with a small set of demonstrations~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt} -- by initializing with a policy that occasionally solves the task, supervision from simple sparse rewards can be enough for RL to progress effectively. \pulkit{Again I think we are going off the topic. And also consider citing Gabe's papers too and recent position paper from Younghyo/Gabe}
%
% But for complex manipulation tasks like assembly, naively trained BC policies may fail to achieve any meaningful success with a small number of demonstrations~\cite{ankile2024juicer}. % small number of demonstrations typically fails to achieve any meaningful success. 
However, naively trained BC policies may fail to achieve any meaningful success with a small number of demonstrations in complex tasks like assembly~\cite{ankile2024juicer} \pulkit{Flow is broken}. % small number of demonstrations typically fails to achieve any meaningful success. 
%
% Recent innovations in BC policy design, such as diffusion models~\cite{chi_diffusion_2023} and action chunking~\cite{zhao_rss23_aloha}, have begun to show promise, achieving non-zero success rates  even in challenging conditions~\cite{ankile2024juicer, heo_furniturebench_2023}.
Innovations in policy design, such as diffusion models~\cite{chi_diffusion_2023} and action chunking~\cite{zhao_rss23_aloha}, can alleviate some of this difficulty and enable non-zero success rates for challenging tasks using a modest number of demonstrations~\cite{ankile2024juicer, heo_furniturebench_2023}. \pulkit{Circular -- we talk BC, then RL and then again BC -- not a good way to frame the paper.}
%
% Yet, integrating these advanced BC policies with RL to further enhance their capabilities presents a new set of challenges~\cite{black_training_nodate}. \anthony{want to strengthen the end of this a bit more, probably here is good place to say a bit about the specific technical challenges of finetuning diffusion/models with action chunking using RL?} % n imperfect policy, % which are more general and easy to specify across tasks 
However, introducing these modern architectural components makes it difficult to perform fine-tuning with RL. \pulkit{But is the goal fine-tuning with RL? I think the goal is different -- how to reduce cost of the BC thing and to say the scaling laws are really bad. They can't achieve high performance. We want to both achieve high performance and do it at a low-cost.} % fine-tune these policies with RL.
%
% For instance, training diffusion models with policy gradients can require complex multi-step MDP formulations of the diffusion de-noising process~\cite{black_training_nodate}. % to deal with final action log probabilities being unavailable from standard diffusion model predictions.
For instance, training diffusion with RL can require complex reformulation of the de-noising process to enable policy gradient estimation~\cite{black2023training}. 
%
We also find that action chunking tends to make direct RL fine-tuning harder and unstable due to the expanded action space dimension induced by chunking. \pulkit{Unnecessary emphases on action chunking in my opinion and missing the bigger picture.}
% Action chunking also creates challenges by artificially expanding the action space dimension, which we find tends to make RL training much more sensitive and unstable. 
% requires   such as requiring  these advanced BC policies with RL to further enhance their capabilities presents a new set of challenges~\cite{black_training_nodate}. \anthony{want to strengthen the end of this a bit more, probably here is good place to say a bit about the specific technical challenges of finetuning diffusion/models with action chunking using RL?} % n imperfect policy, % which are more general and easy to specify across tasks 

% In this paper, we explore adaptations to the teacher-student pipeline that incorporate modern advancements like diffusion policies and demonstrate their application in the complex domain of furniture assembly~\cite{heo_furniturebench_2023}.
% In this paper, we propose adaptations to the BC + RL pipeline that enable it to work with modern advancements like diffusion policies and chunked action predictions and demonstrate their application in the complex domain of furniture assembly~\cite{heo_furniturebench_2023}.
In this paper, we propose adaptations to the BC + RL pipeline that facilitate its application to complex tasks like furniture assembly~\cite{heo_furniturebench_2023} \pulkit{Is this the point of the paper? This benchmark is used to evaluate a hypothesis - - what is the hypothesis?}. Our key contribution is to enable RL fine-tuning to work with modern advancements like diffusion policies and chunked action predictions \pulkit{No this is not the contribution, this is the technical innovation which enabled the contribution. Its also good to clearly acknowledge the vast literature of IL + RL fine-tuning and say what is different here in the technical details too. But the main contribution of the paper is not really stated.}. % and demonstrate their application in the complex domain of furniture assembly~\cite{heo_furniturebench_2023}.
%
% We first provide a detailed analysis and empirical evidence supporting the effectiveness of diffusion policies and action chunking in complex task acquisition through BC.
We first provide an analysis and empirical evidence supporting the need for action chunking and expressive policy architectures for achieving success rates that are high enough to bootstrap RL. %from sparse rewards. %  diffusion policies and action chunking
%
% We then show how we can use residual policies for RL to tune the diffusion policies from sparse task rewards, which predict corrective actions rather than altering the base policy directly.
% We then show how we can use residual policies and on-policy RL to tune the diffusion policy behavior from sparse task rewards, by training the residual to predict corrective actions rather than altering the base policy directly.
We then propose training residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual} with on-policy RL and sparse task rewards to improve upon pure BC, an approach we term \methodname\space (\textit{Resi}dual for \textit{P}recise manipulation). These residual models learn to predict corrective actions that more reliably achieve high precision. In this way, we side-step the aforementioned challenges of directly altering the base policy with RL, while improving overall task success. \pulkit{Why residual is not really motivated -- seems arbitrary -- many people have done this before.}
% We then show how on-policy RL from sparse rewards can improve the base model performance by learning residual policies that output locally corrective actions on top of the frozen diffusion policy. we can train residual policies on-policy RL to tune the diffusion policies from sparse task rewards, which predict corrective actions rather than altering the base policy directly.
%
% These residual policies address the deficiencies in initial BC models, offering fine-tuned adjustments necessary for high-precision and contact-rich tasks.
%
% Finally, we also demonstrate practical applications in real-world settings. By integrating limited real-world demonstration data with extensive synthetic datasets, we showcase the practical viability of our approach, enabling robots to perform intricate assembly tasks from RGB images with enhanced accuracy and efficiency.
Finally, by distilling behaviors learned with RL into a large synthetic dataset of trajectories and combining them with a limited set of real-world demonstrations, we showcase the benefits of our residual learning approach, \methodname, in enabling real-world assembly policies that operate directly from RGB images \pulkit{Again this is a side point, not the main point.}.

% By integrating a limited amount of real-world demonstration data with a large set of from our RL-trained policies, we showcase in the real world. large in the context of RGB-based ``teacher-student'' distillation and sim-to-real transfer. By collecting  
% Finally, we demonstrate  application of our residual learning approach to perform multi-step assembly directly from RGB images in the real world. real-world assembly  settings using the ``teacher-student'' distillation paradigm. By integrating limited real-world demonstration data with extensive synthetic datasets, we showcase the practical viability of our approach, enabling robots to perform intricate assembly tasks from RGB images with enhanced accuracy and efficiency.



==> Archive/intro_versions/intro_idan.tex <==
\section{Introduction}

Although there have been impressive developments in robot learning in recent years, many tasks remain challenging to learn - especially those involving long horizon, contact rich, and high precision. An example of such a task is autonomous assembly, where a robot must put together different parts precisely \pulkit{Its not clear if the task is necessarily long-horizon, since most assembly can divided into substeps}. 
%
Solving such a task using existing methods requires enormous human effort - either by collecting large demonstrations for Imitation Learning (IL) or carefully constructing a reward function for Reinforcement Learning (RL).
%
%
Our goal is to create a framework to teach a robot to perform contact-rich and precise tasks while minimizing human involvement. 

 
Imitation learning (IL), and more specifically behavior cloning (BC), has re-emerged as a popular technique for acquiring manipulation control policies.
%
This is due to factors like technical simplicity, the intuitive user interface offered in programming a robot's behavior by directly performing it oneself \pulkit{giving teleop demos may not be intuitive}, and BC's general applicability to many tasks that remain challenging to achieve using other techniques~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational,jang2022bc, zhao_rss23_aloha} \pulkit{Its good be balanced here --thereare many tasks that remain challenging for BC too -- it suffices to stress that its easy to demonstrate tasks without the need to setup simulation or perform real-world RL}.
%
Substantial effort has recently been applied in robotics and manipulation toward demonstrating that large-scale data collection and imitation learning can power similar performance gains in simple manipulation tasks~\cite{}\lars{RT-1/2/X} \pulkit{Unclear / unnecessary -- large scale data collection is not something we are doing, nor are we concerned with generalization across tasks -- but mostly the precision and robustness to task-variations}.
%
We hypothesize similar performance gains can be attained in more challenging robotic tasks via large-scale imitation learning.
%
However, such large-scale data often comes at a very high cost since humans need to manually collect expert demonstrations and perform the tasks on a physical system many times in the real world.
\pulkit{Good to say previous couple of lines in just one line. Also, good to emphasize why large data is required to get demos for different configuration and corrections. }
%

Because human-provided demonstrations are expensive at scale, a popular alternative pipeline is to create a performant agent in a simulated environment and use it as a data source. \pulkit{Its not just expensive -- but also the kind of data required -- corrections and precision.}
Usually, the simulated agent is trained using Reinforcement Learning (RL), and deployed in reality. Recent progress in sim-to-real techniques like domain randomization~\cite{tobin2017domain, other_dr_robotics_successes}, improved physics fidelity and photorealistic rendering~\cite{isaac_gym}, and combination of small amounts of real-world data~\cite{torne2024reconciling_rialto, other_co_training} made this approach popular. However, training RL in simulation heavily relies on successful reward design and setting up the simulation \pulkit{good to cite gabe/younghyo's position paper}. For challenging tasks such as assembly, finding the right reward function is not trivial and requires many iterations and trials, leading to significant human effort. Ideally, we would like to use a simple success or fail signal as the reward, but doing RL from a sparse binary reward is known to be challenging \pulkit{General advice -- make this succinct -- this is mostly background and we would love to come to the main point of the paper more quickly}.
%

\pulkit{Our main insight is really about the use of residuals, and not combining BC and RL -- consider framing like -- learning precise, contact-rich tasks requires corrective behaviors. Collecting such teleoperation data is hard. RL can, nut requires reward design/simulation setup. Idea explored in prior works is to use BC + RL, but we can't extend that to modern architectures like diffusion models due to fundamental limitations. We overcome by proposing residual.}

Our main insight is that by using a small number of human demonstrations, we can get the agent to a level of performance where it can train further using RL with only task success reward \pulkit{This is not the main insight -- this is something many papers have said before}. Then, a large number of rollouts from this trained agent can be collected in simulation and distilled to create the real-world policy.  
However, performing BC from a small amount of demonstrations is not trivial. Motivated by prior work~\cite{ankile2024juicer, heo_furniturebench_2023} we perform BC with modern policy architectures, e.g., diffusion policies~\citep{chi_diffusion_2023}, that can achieve non-zero success rates on hard tasks from small initial demonstration budgets. To perform RL over the diffusion policy, we use policy gradient reinforcement learning~\cite{schulman_proximal_2017} with residual policies~\cite{silver2018residual, davchev2022residual} and demonstrate that it can achieve high performance, even with sparse rewards.

\idan{didn't touch that part yet}
Overall, our contributions are the following: (1) a technique for fine-tuning diffusion policies trained with behavior cloning using residual policies and imitation-bootstrapped PPO with sparse rewards and (2) a demonstration of a pipeline for converting an RL policy operating on privileged state information into a large, diverse dataset for distilling the learned behaviors into an image-based policy in assembly manipulation domains \anthony{Should reference teacher-student earlier, then contribution (2) becomes ``we demonstrate teacher-student RL + distillation working well for assembly, maybe also combined with sim2real with images}. We compare and evaluate the performance of PPO-trained residual policies with other techniques for fine-tuning BC-trained policies in terms of the final task success rate and coverage of the resulting datasets that can be synthesized. We also analyze how final vision policy performance scales with the amount of data that is used for assembly tasks.
%
Finally, we demonstrate real-world assembly from RGB images by combining datasets synthesized from our pipeline with a small amount of real-world demonstration data.

==> Archive/intro_versions/intro_idan_2.tex <==
\section{Introduction}

Despite significant advancements in robot learning, autonomous systems still struggle with complex manipulation tasks, especially those that are contact-rich and require high precision.
%
An example of such a challenging scenario is autonomous assembly, where a robot must precisely fit various parts together while relying solely on visual inputs from cameras. 
%
Performing such tasks presents substantial challenges for traditional robotic learning frameworks.

One such common framework is teacher-student distillation. Typically, a teacher policy is trained in a simulated environment using Reinforcement Learning (RL), benefiting from access to complete state information and the capability to parallelize trials.
%
This policy then generates successful trajectories to train a sensor-based student policy through Behavior Cloning (BC). The sensor-based student can then be deployed in the real world using sim-to-real techniques. Despite its advantages, deploying this framework effectively in hard tasks, such as assembly, remains arduous. Pure RL approaches to these tasks can be particularly challenging due to the complexity of crafting effective reward functions that are both generalizable and sufficiently detailed to guide proper task execution. 

To mitigate these issues, it is common to leverage a small set of initial human demonstrations to bootstrap the RL process. The underlying idea is that starting with an imperfect policy, which can occasionally solve the task, might suffice for RL training when using a sparse task success reward. However, for complex tasks like assembly, a small number of demonstrations typically fail to achieve any meaningful success.  Innovations in BC, such as diffusion policies and action chunking, have begun to show promise, achieving non-zero success rates even in challenging conditions~\cite{ankile2024juicer, heo_furniturebench_2023}. Yet, integrating these advanced BC policies with RL to further enhance their capabilities presents a new set of challenges~\cite{black_training_nodate}.

In this paper, we explore adaptations to the teacher-student pipeline that incorporate modern advancements like diffusion policies and demonstrate their application in the complex domain of furniture assembly~\cite{heo_furniturebench_2023}. We first provide a detailed analysis and empirical evidence supporting the effectiveness of diffusion policies and action chunking in complex task acquisition through BC. We then show how we can use residual policies for RL to tune the diffusion policies from sparse task rewards, which predict corrective actions rather than altering the base policy directly. These residual policies address the deficiencies in initial BC models, offering fine-tuned adjustments necessary for high-precision and contact-rich tasks.

Finally, we also demonstrate practical applications in real-world settings. By integrating limited real-world demonstration data with extensive synthetic datasets, we showcase the practical viability of our approach, enabling robots to perform intricate assembly tasks from RGB images with enhanced accuracy and efficiency.



==> Archive/intro_versions/intro_v3.tex <==
\section{Introduction}


% ==== New version of intro ====



Robotic systems struggle with tasks simultaneously requiring high precision, robustness to varied initial conditions, and the ability to operate directly from RGB sensors \zw{is it true? need reference or elaboration}. Autonomous assembly exemplifies these challenges, where robots must manipulate and precisely fit together multiple parts without relying on tight and bespoke \zw{seems a esoteric word haha} fixtures for precise and consistent positioning.% Such tasks demand not only accurate execution but also the ability to perform corrective actions when deviations inevitably occur.

% \idan{poor transition from first to second paragraph}
Behavior cloning (BC) has re-emerged \zw{again, "re" emerging needs a more context.} as a popular approach for teaching robots complex manipulation tasks~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, jang2022bc, zhao_rss23_aloha}. Recent innovations in BC, such as diffusion models \cite{janner_planning_2022,ajay_is_2023,chi_diffusion_2023,pearce_imitating_2023} and action chunking \cite{zhao_rss23_aloha}, have enabled learning long-horizon, complex behaviors from modest numbers of demonstrations that are infeasible with standard policy architectures \zw{seems an argument about new arch enables more efficient learning - is it necessary to say this? reading this sentence makes me expect a story about data efficiency on the demonstration}. However, BC has limitations for precise manipulation tasks~\cite{ankile2024juicer} \zw{Define "precise" manipulation. It's important since it's the main problem studied in this paper.}.


One of the main challenges with BC is that its performance has been found to saturate with increasing expert demonstrations, and achieving even moderate success rates may require prohibitively large and costly demonstration datasets~\cite{yu2024lucidsim,zhao2024aloha} \zw{Not connected to precise manipulation. The fact that BC has a limitation on precise manipulation doesn't mean that we need more expert demonstration.}. This is particularly problematic since dataset size scales linearly with human effort~\cite{park2024automatic}.
%
% For example, as illustrated in \autoref{fig:overview} (B), our analysis shows that for a single assembly task, achieving an 80\% success rate would require approximately 5000 demonstrations, translating to 75 hours of human effort \pulkit{more important point is saturation in performance.}.
%
Furthermore, our analyses suggest that BC struggles to generalize for precise manipulation tasks as it does not learn to correct mistakes by learning solely from imitating expert actions \zw{now it comes back again to precise manipulation. the argument of performacne saturation got cut off. I suggest building a stronger connection between performance saturation and difficulty of precise manipulation. One idea: Only a few trajectories or policies lead succeess in precise manipulation. For instance, assembling furniture demands precise screw placement, leaving little room for error in positioning. In contrast, placing plates in a drawer is less exact, allowing for more flexibility and mistakes, thus requiring lower precision. In high-precision tasks, models must closely follow expert policies, which is difficult with limited demonstrations. More expert demonstrations can help the BC policy learn precision, but improvement plateaus after a certain number of demos. This may be because BC learning doesn't teach the model to correct its own mistakes. BC models are imperfect and always have irreducible errors due to limited capacity [cite]. If a BC model makes a mistake early in an episode, it enters states the expert never demonstrated, since the expert didn’t make those errors. Therefore, the BC model must learn how to act in those unobserved states. Then introduce DAgger and RL}. Even with moderate environment interaction through DAgger, performance improves beyond what imitation alone enables (see \autoref{fig:overview} (B)).% DAgger does, however, require the existence of an expert policy.

% \lars{Should we mention DAgger being very effective somewhere here? If so, the point would be that interactive learning is very effective but requires an expert teacher. Where do we get that from? Impractical for humans $\rightarrow$ use RL.} \idan{I think it distract from the story, but for sure something is missing in the transition to the next paragraph. We talk about how BC saturates, but didn't say why. We should come up with a "why" that motivates RL}


A common way to cheaply achieve high performance and reactive policies \zw{is mentioning reactive policy important here?} is to leverage simulation and reinforcement learning (RL) to autonomously collect and learn from large amounts of data and environment interaction. While combining BC and RL has a long history \cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt, ball2023efficient, schaal1996learning, nair2018overcoming, nakamoto2024cal, uchendu2023jump, hu2023imitation, zheng2022online, kober2010imitation, ramrakhya2023pirlnav, singh2020parrot}, the recent advancements in BC architectures present new challenges for direct application of traditional RL methods. Specifically, innovations like diffusion policies and action chunking, complicate the process of RL fine-tuning~\cite{drolet2024comparison}. \zw{how they make RL complicated is not explained. I suggest you pick one problem that make RL finetuning complicated and then hook on this problem to expand the motivation of using residual policy.}


This paper proposes a simple yet effective scheme to augment state-of-the-art BC models with RL. The approach involves training residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual, zeng2020tossingbot} with on-policy RL and sparse task rewards to improve upon pure BC from a handful of demonstrations. \zw{This says how you implement but didn't say why you implement in this way. The most critical part of the intro is the key insight of your idea -- Why residual policy makes finetuning easier?} The residual model observes the latest state observation and the current predicted action and predicts a correction online.
% \lars{It enables online RL with modern BC architectures like diffusion policies and chunked action predictions. Learn RL in a higher frequency, easier to learn, and more reactive policy.}


% Differences to other residual methods:
% \cite{silver2018residual}: Predict on every step, base is not learned, residual does not observe base
% \cite{davchev2022residual}: Base is learned as a DMP, base predicts in 100Hz, residual in 10Hz
% \cite{johannink2019residual}: Base is a traditional controller, they operate at same frequency, residual does not take base action as input
% \cite{zeng2020tossingbot}: Physics-based, analytical base, same frequency


% We have found action chunking critical for BC policies to achieve any non-zero task success required for bootstrapping RL. This, however, means that the resulting policy will operate partially open-loop for most of the trajectory, making it less reactive. Therefore, we find that having the residual operate on a different frequency than the base combines both partial open-loop strengths of action chunking with online reactivity.

% Second, we find that DP is important

% \idan{citation and maybe a one-line explanation about what it is}. 

% \idan{so far it was really nice. a clear story that roughly says modern BC is good $\rightarrow$ but it saturates $\rightarrow$ BC+RL is the solution but unclear how to do with modern BC $\rightarrow$ we have a solution. The next few paragraphs become quite repetitive and too detailed. Try to think what the most important points from the experiment section a reader should know}

The approach, which we call \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation), side-steps the challenges of fine-tuning SoTA BC methods altogether by keeping the base model frozen during RL training. This also allows for running the residual policy at a higher frequency than the chunked base model \zw{the low frequency issues of prior works weren't discussed}, resulting in a more reactive, fully closed-loop policy.

% Learn RL in a higher frequency, easier to learn, and more reactive policy

% \begin{enumerate}
%     \item It enables online RL with modern BC architectures like diffusion policies and chunked action predictions.
%     \item It reintroduces a fully closed-loop reactivity to action-chunked policies for better reactivity.
%     \item It maintains the benefits of the pre-trained BC policy, like multi-modality, while enabling learning local, corrective behaviors and mitigates common RL issues such as instability~\cite{kumar2020conservative,schulman2015trust}, mode collapse, and catastrophic forgetting~\cite{wolczyk2024fine}. \lars{Overclaim, take out?}
% \end{enumerate}

% Say that we learned that it's important to have different frequencies on policies 

%\autoref{fig:distillation-scaling}
% Summarize results, then go back to explaining what we do, weird flow

% \autoref{fig:overview} (B) shows that \methodname{} performs better than pure BC while requiring less data. As such, our method enables robots to learn precise manipulation and corrective behaviors crucial for tasks like assembly. %By combining a strong prior from BC with the exploratory capabilities of RL, we achieve a 73\% improvement in success rate for low-randomness tasks and a 64\% improvement for medium-randomness tasks compared to BC alone.

We evaluate our method on a set of tasks involving sequences of precise insertions, rearrangements, and long-horizon multi-part interactions like furniture assembly from the challenging FurnitureBench \cite{heo_furniturebench_2023} task suite and peg insertion from the Factory~\cite{narang2022factory} task suite.
%
% We also show how scanning real-world objects can slacken the assumption of access to CAD models and pre-defined goal poses with a custom mug-hanging task.
%
Our results show that \methodname{} significantly outperforms pure BC and alternative RL fine-tuning approaches across these tasks.

To show the usefulness of our approach, we distill the behaviors learned through RL in simulation into a real-world policy, solving furniture assembly from RGB observations only \zw{seems to presume you learn with full env state in sim and so you need to distill the model to RGB policy so as to deploy in the real world. is that fair to assume all readers of ICRA know this assumption?}. We do this by synthesizing a large set of demonstrations from a simulator-trained RL policy that we combine with a limited set of real-world demonstrations. \zw{again, this is how you implement so can be left in the later sections.} This allows us to leverage the data efficiency of RL and simulation while bridging the sim-to-real gap. The resulting policies enable capabilities not possible from BC alone.

In summary, this paper highlights the limitations of BC in learning precise manipulation skills. We present an approach that combines BC and RL's strengths to overcome these limitations using SoTA BC architectures with residual RL. By addressing the limitations of pure BC and enabling RL fine-tuning of modern policy architectures, \methodname{} achieves high-performance, corrective behaviors for complex assembly tasks in simulation and in the real world while requiring modest amounts of human data.



\iffalse{}


\pulkit{Suggestions
\begin{itemize}
    \item Robots struggle to learn tasks robustly and those that require high precision, etc etc.
    \item BC is a popular approach. Our analysis reveals fundamental limitations of BC -- the asymptotic performance is limited, and the cost is too high. Have Figure 1 show this. 
    \item How do we achieve high-asymptotic performance cheaply? Leverage simulation and automatically collect data using RL. 
    \item BC + RL has had a long history. However, with new BC methods past methods can't directly be applied -- explain why. 
    \item We devise a simple scheme (call it simple so that people don't think we are claiming methodological innovation per se) -- that augments the latest and greatest BC models with a residual model trained with RL. 
    \item Explain why we want a residual model and how we overcome other issues typical in RL Problem -- again nothing new here. But good to say explicitly. 
    \item End by referring back to Figure 1 -- saying look at scaling laws now -- we are much better performance at much cheaper. 
    \item Also have an example of the task in this Figure. 
    \item Conclude by saying evaluation is performed on Furniture bench. 
\end{itemize}
}




\subsection{Original version w/ comments}

Despite significant advancements in robot learning, autonomous systems still struggle with manipulation tasks requiring high precision, robustness to a wide array of initial conditions, and operation directly from RGB sensors. 
%
An example of such a challenging scenario is autonomous assembly, where a robot is presented with a set of multiple parts to pick up and precisely fit together.
%

Such systems typically utilize engineered fixtures for consistent initial part positioning, making assembly robots expensive and impractical to adapt across diverse tasks.
%
Learning to perform these tasks from vision can improve the adaptability and robustness of such systems, but the high-precision, contact-rich nature of such tasks poses substantial challenges for current robotic learning frameworks. \pulkit{Not required -- too much details that are known, irrelevant -- come to the point directly} % Learning-based Vision-based control has the potential to

Behavior cloning (BC) has re-emerged as a popular technique for acquiring manipulation control policies~\cite{schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational,jang2022bc, zhao_rss23_aloha}. This is largely due to the ease of directly specifying complex tasks by providing demonstrations.
%
However, BC requires large amounts of costly demonstration data to enable generalization to different scene configurations~\cite{jang2022bc}.
%
BC-trained policies are also often limited by the nature of human demonstrations that \emph{directly} achieve the task. This can mean such policies never learn to perform \emph{corrective} actions that recover from deviations that inevitably occur during deployment. \pulkit{This point is not made strongly -- say that we show that for precise problems, the scaling is bad -- in fact it saturates, or the amount of data that is required is these many trajectories translating into this much cost XXX amount of dollars. }
%
Reinforcement learning (RL) offers a complementary paradigm, wherein locally corrective behavior can be learned by exploring and discovering action sequences that lead to downstream task success \pulkit{RL doesn't offer locally corrective behavior -- RL is just a way of learning policies.}. 
%
Although RL offers appealing advantages, many of its successes in robotics depend on carefully crafted reward functions that may sacrifice generality across tasks~\cite{kumar2021rma, jiang2024transic_assembly, chen2023visual}. 


A common mitigation is to bootstrap the RL process by starting with a small set of demonstrations~\cite{Rajeswaran-RSS-18_dapg, james2022q, lu2022aw_opt} -- by initializing with a policy that occasionally solves the task, supervision from simple sparse rewards can be enough for RL to progress effectively. \pulkit{Again I think we are going off the topic. And also consider citing Gabe's papers too and recent position paper from Younghyo/Gabe} \lars{The position paper added. What Gabe papers would be most relevant here?}
%
However, naively trained BC policies may fail to achieve any meaningful success with a small number of demonstrations in complex tasks like assembly~\cite{ankile2024juicer} \pulkit{Flow is broken}.
%
Innovations in policy design, such as diffusion models~\cite{chi_diffusion_2023} and action chunking~\cite{zhao_rss23_aloha}, can alleviate some of this difficulty and enable non-zero success rates for challenging tasks using a modest number of demonstrations~\cite{ankile2024juicer, heo_furniturebench_2023}. \pulkit{Circular -- we talk BC, then RL and then again BC -- not a good way to frame the paper.}
%
However, introducing these modern architectural components makes it difficult to perform fine-tuning with RL. \pulkit{But is the goal fine-tuning with RL? I think the goal is different -- how to reduce cost of the BC thing and to say the scaling laws are really bad. They can't achieve high performance. We want to both achieve high performance and do it at a low-cost.}
%
For instance, training diffusion with RL can require complex reformulation of the de-noising process to enable policy gradient estimation~\cite{black2023training}. 
%
We also find that action chunking tends to make direct RL fine-tuning harder and unstable due to the expanded action space dimension induced by chunking. \pulkit{Unnecessary emphases on action chunking in my opinion and missing the bigger picture.}


In this paper, we propose adaptations to the BC + RL pipeline that facilitate its application to complex tasks like furniture assembly~\cite{heo_furniturebench_2023} \pulkit{Is this the point of the paper? This benchmark is used to evaluate a hypothesis - - what is the hypothesis?}. Our key contribution is to enable RL fine-tuning to work with modern advancements like diffusion policies and chunked action predictions \pulkit{No this is not the contribution, this is the technical innovation which enabled the contribution. It's also good to clearly acknowledge the vast literature of IL + RL fine-tuning and say what is different here in the technical details. But the main contribution of the paper is not really stated.} \lars{The contribution then is that we show how BC is limited and offer a way to get precision and robustness cheaply?}.
%
We first provide an analysis and empirical evidence supporting the need for action chunking and expressive policy architectures to achieve success rates high enough to bootstrap RL.
%
We then propose training residual policies~\cite{silver2018residual, davchev2022residual, johannink2019residual} with on-policy RL and sparse task rewards to improve upon pure BC, an approach we term \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation). These residual models learn to predict corrective actions that more reliably achieve high precision. In this way, we side-step the aforementioned challenges of directly altering the base policy with RL, while improving overall task success. \pulkit{Why residual is not really motivated -- seems arbitrary -- many people have done this before.}
%
Finally, by distilling behaviors learned with RL into a large synthetic dataset of trajectories and combining them with a limited set of real-world demonstrations, we showcase the benefits of our residual learning approach, \methodname, in enabling real-world assembly policies that operate directly from RGB images \pulkit{Again this is a side point, not the main point.} \lars{Should it not feature in the intro?}.

\fi




% \subsection{Draft updated version wrt/ comments}




==> Archive/method.tex <==
\section{Method}
Our method applies to any task that can be simulated using already available assets (e.g., CAD models) or by digitizing real-world ~\cite{torne2024reconciling_rialto, villasevil2024scaling}. While this paper focuses on assembly tasks for which CAD models are already available for constructing simulation environments, our method applies to many tasks of practical interest. Note that our method requires CAD models only for training and not during deployment. 

Our approach from task definition to deployable vision policy consists of three key components (see \autoref{fig:pipeline} for an overview). First, we train a base policy using behavior cloning (BC) on a small set of demonstrations (\autoref{sec:behavior-cloning}) in simulation. Then, we improve this policy's precision by training a residual component with reinforcement learning that makes closed-loop corrections to the base policy's actions (\autoref{sec:reactive-control}). Finally, we learn a real-world deployable policy with policy distillation and co-training with a few real-world demonstrations (\autoref{sec:sim-to-real-pipeline-method}). 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/framework_overview.pdf}
    \caption{\textbf{Sim-to-real pipeline.} \textcolor{longcolor}{\textbf{(1)}} Beginning with a policy trained with BC in simulation, \textcolor{rlcolor}{\textbf{(2)}} we train residual policies with RL and sparse rewards. \textcolor{daggercolor}{\textbf{(3)}} We then distill the resulting behaviors into a policy operating from RGB images. \textcolor{bccolor}{\textbf{(4)}} By combining synthetic data with a small set of real demonstrations, \textcolor{cotrain}{\textbf{(5)}} we deploy RGB-based policies in the real world.}
    \label{fig:pipeline}
    \vspace{-15pt}
\end{figure*}

\subsection{Problem Formulation}
\label{sec:problem-formulation}
We formulate the target task as a discrete-time sequential decision-making problem. At each timestep $t$, the robot receives an observation $o_t \in \mathcal{O}$ corresponding to the underlying state $s_t \in \mathcal{S}$ of the robot and environment. Given the observation, the policy outputs an action $a_t \in \mathcal{A}$ that is executed in the environment. The action space $\mathcal{A}$ consists of end-effector poses in $\sethree{}$ and gripper commands. The state space includes the robot's configuration (end-effector pose, velocity, and gripper state) and the poses of all objects in the scene. Task completion is defined through sparse task completion rewards.  We define this reward as an instantaneous signal that provides 1 at the timestep when a pair of objects achieves a pre-defined relative pose corresponding to successful assembly and 0 otherwise, including after the alignment is maintained. See more details about the environments in \appref{app:tasks-details}.


\subsection{Base Policy Learning via Behavior Cloning}
\label{sec:behavior-cloning}
For each task, we collect a dataset of 50 demonstrations in simulation by teleoperating the robot, $\mathcal{D}_{\text{sim}}:\ \{\tau_1, ..., \tau_N\}$. Each trajectory, $\tau$, contains system states $s_{t}$, and robot actions $a_{t}$, i.e., $\tau_i=\{(s_t, a_1), ..., (s_T, a_T)\}$, with $T$ being the trajectory length. We use $\mathcal{D}_{\text{sim}}$ to first train base policy $\pi_{\text{base}}$ with Behavior Cloning (BC), i.e., $\pi_{base} =\ \argmax_{\pi_{\text{base}}}\ \mathbb{E}_{(a_t,s_t)\sim\mathcal{D}_{\text{sim}}} \left[\log\pi_{\text{base}}(a_t|s_t) \right]$ using the Diffusion Policy (DP) architecture~\cite{chi_diffusion_2023}, which serves as the starting point for RL training. Consistent with state-of-the-art in BC training~\cite{chi_diffusion_2023, zhao_rss23_aloha}, we use action chunks that predict a set of multiple future actions instead of a single action at every timestep. This chunking approach effectively reduces the task horizon, enabling better performance on long-horizon tasks, but as our results will show (\autoref{sec:resip-ablations}), it sacrifices the ability to make closed-loop corrections. We denote the length of future action sequences predicted by the policy as $T_a$, the output as $\actchunk = [a_t^{\text{base}}, ..., a_{t+T_a}^{\text{base}}]$. When predicting an action chunk $\actchunk$ of length $T_a$, we only execute a subset $[a_{t}^{\text{base}},...,a_{t+T_{\text{exec}}}^{\text{base}}]$, with execution horizon $T_{\text{exec}} \leq T_a$. Similar to~\cite{chi_diffusion_2023}, we use $T_{\text{exec}} = 8$, and $T_a = 32$ instead of their 16 as we empirically found it performs better.

\subsection{Reactive Control via \methodname{}}
\label{sec:reactive-control}


Given the initial chunked base policy $\pi_{\text{base}}$ obtained by Behavior Cloning described above, we want to improve the policy to overcome the issues of distribution shift and the lack of reactivity.
%
One way to mitigate the adverse effects of distribution shifts is to fine-tune the BC pre-trained policy with RL~\cite{pomerleau1988alvinn, schaal_learning_1996, schaal1999imitation, ratliff2007imitation, agrawal2018computational, zhang2018deep, brohan2022rt, jang2022bc, zhao_rss23_aloha, drolet2024comparison, torne2024reconciling_rialto}. We side-step the complications of direct RL fine-tuning of action-chunked policies (see discussion in \autoref{app:tasks-details}) by training a residual~\cite{silver2018residual, johannink2019residual, alakuijala2021residual, davchev2022residual, carvalho2022residual, shafiullah2022behavior_bet, haldar2023teach_fish_residual, lee2024behavior_vqbet} Gaussian Multi-Layer Perceptron (MLP)\cite{rumelhart1986learning} policy $\pi_{\text{res}}$ using PPO\cite{schulman_proximal_2017}. Our key design choice is that while this residual framework can address distribution shift through either chunk-level or timestep-level corrections (see \autoref{sec:closed-loop-ablation} for analysis), the latter enables crucial reactive behavior necessary for precise manipulation.


For each timestep $i = 0, ..., T_a - 1$ within the base policy's action chunk, we form the residual's observation by concatenating the full simulation state (robot proprioceptive information and object poses) with the base policy's predicted action, $s_{t+i}^\text{res}=[s_{t+i},a^\text{base}{t+i}]$. The residual policy then produces corrective actions $a_{t+i}^{\text{res}} \sim \pi_{\text{res}}(\cdot | s_{t+i}^\text{res})$ that modify the base actions: $a_{t+i} = a_{t+i}^{\text{base}} + a_{t+i}^{\text{res}}$. The resulting fine-tuned policy is a combination of the pre-trained BC policy $\pi_\text{base}$ and the correction policy $\pi_\text{res}$, denoted $\boldsymbol{\pi}$. As demonstrated in \autoref{sec:closed-loop-results}, this per-timestep correction capability is crucial for achieving reliable performance in precision-critical tasks.



During training, as in any RL fine-tuning, one needs to adjust the exploration noise to provide sufficient stochasticity to discover new behaviors while maintaining enough precision for task success (see \appref{app:alpha-ablation} for detailed analyses of design choices). The residual policy uses orthogonal initialization~\cite{saxe2013exact} with a small gain factor on the final layer, ensuring uncorrelated initial corrections centered around zero---a design choice that aligns with our assumption that the base policy's errors are unbiased in expectation. Since most task failures stem from slight imprecisions in the base policy's actions, this architecture naturally leads to learning small, targeted corrections around the base policy's behavior.


\begin{figure}
    \vspace{5pt}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/Synthetic_Data.pdf}
    \caption{Photorealistic rendering and domain randomization for sim-to-real transfer. In the first row, we show our nominal experiment setting of rendering parts in the original white color while varying the position, brightness, and hue of the lighting in the scene. In the bottom row, we also introduce variations in the part colors to see how that can help the final policy adapt to unseen part appearances without collecting any additional data.}
    \label{fig:synthetic-data}
    \vspace{-15pt}
\end{figure}

The policy observation for simulation training, $\mathcal{S}$ contains the 6 DoF end-effector pose $\xform$, spatial velocity $\mathbf{V}$, and gripper width $w_{\text{g}}$, along with the 6-DoF poses of all the parts in the environment $\{\xform{}^{\text{part}_{i}}\}_{i=1}^{\text{num\_parts}}$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/Task_overview_2.png}
    \caption{Initial and goal states for our 6 tasks. The first three tasks, \oneleg{}, \roundtable{}, and \lamp{}, come from the FurnitureBench~\cite{heo_furniturebench_2023} task suite. \mugrack{} we created by scanning objects and importing them into the simulation. \peghole{} is from the Factory~\cite{yash_factory2022_rss} task suite. \bimaninsert{} we created using the simulation-based teleoperation system DART~\cite{park2024dexhub}. Our task suite exhibits diverse challenges like long horizons, tight tolerances, bimanual control, and multi-modal success criteria.}
    \label{fig:task-overview}
    \vspace{-15pt}
\end{figure*}

\subsection{Sim-to-Real Transfer}
\label{sec:sim-to-real-pipeline-method}


We treat $\pi_{res}$ trained in simulation using privileged state information, $\mathcal{S}$, as a teacher policy $\pi_\text{teacher}$ to distill into a student policy $\pi_\text{student}$ that takes as input sensory observations and can therefore be deployed in the real world~\cite{lee2020learning, kumar2021rma, chen2023visual, torne2024reconciling_rialto}. The real world observation space $\mathcal{O}$ contains the robot end-effector pose $\xform{} \in $ \sethree{}, robot end-effector spatial velocity $\mathbf{V} \in \mathbb{R}^{6}$, the gripper width $w_{\text{g}}$, and RGB images from a fixed front-view camera ($I^{\text{front}} \in \mathbb{R}^{h \times w \times 3}$) and a wrist-mounted camera ($I^{\text{wrist}} \in \mathbb{R}^{h \times w \times 3}$), each with uncalibrated camera poses.

For teacher-student distillation, we collect a large dataset of successful trajectories $\mathcal{D}_{\text{synth}}=\{\tau_{\text{synth},1}, ..., \tau_{\text{synth},N}\}$, $\tau_{\text{synth},i}=\{(s_1, a_1), ..., (s_T, a_T)\}$, from $\pi_{teacher}$ initialized with a diverse set of initial object poses.
%
To bridge the sim-to-real gap, we convert the trajectory dataset with only state information ($\mathcal{S}$) into trajectories with sensory observations (($\mathcal{O}$)) by re-rendering the trajectories to realistic-looking image observations (see \autoref{fig:synthetic-data} for examples). This rendering process allows us to introduce environmental variations---including object colors, textures, lighting conditions, and camera perspectives---that would be impractical to obtain through standard image augmentations or real-world data collection (see \appref{app:sim-to-real-analysis} for examples and details). We denote this rendered dataset as $\mathcal{D}_{\text{synth-render}}$.


$\pi_\text{student}$ is represented with a Diffusion Policy architecture that uses ResNet18\cite{he2016deep} vision encoder pre-trained on robotic manipulation data~\cite{nair_r3m_2022} (see \appref{app:rgb-policy-implementation-details} for implementation details). To minimize the sim-to-real gap, we combine a small set of real-world demonstrations $\mathcal{D}_{\text{real}}$ (10-40 trajectories) collected directly on the robot with synthetic rendered trajectories from $\mathcal{D}_{\text{synth-render}}$ (approximately 400 demonstrations)~\cite{torne2024reconciling_rialto}. This synthetic-to-real data ratio provides increased domain coverage while not washing out real-world demonstrations. The real demonstrations contain only RGB observations and no ground-truth pose information. This combined dataset $\mathcal{D}_{\text{real}} \cup \mathcal{D}_{\text{synth-render}}$ is used to train the student policy $\pi_\text{student}$ with the same Behavior Cloning loss as in the simulation-based experiments.



==> Archive/method_v1.tex <==

\section{Methods}

% \input{fig_text/pipeline}

\subsection{Imitation Learning}

%Given the simulation environment containing the 3D assets representing the objects relevant to the given task, we wish to learn a policy in simulation that can solve desired tasks from a wide variety of configurations and environmental conditions. While this can, in principle, be achieved by training policies from scratch using RL, this would typically require extensive reward engineering\lars{Cite some works that do extensive reward engineering?}. Instead, we aim to only provide sparse rewards to the agent that indicate when two parts in the assembly have reached their desired relative alignment. Such sparse reward supervision makes exploration exceedingly difficult in applying RL from scratch. Therefore, we adopt the paradigm of pre-training a policy on a set of manually collected demonstrations that achieve non-zero success rates and then using RL to fine-tune and automatically improve this policy using the sparse task reward.\lars{Mention that this is more task-agnostic than reward engineering -- can apply the same approach for any task?}

%
% To train the initial ``base'' policy, we collect a demonstration dataset in simulation $\mathcal{D}_{\text{sim}}$. This dataset contains trajectories, e.g., $\mathcal D=\{\tau_1, ..., \tau_N\}$, where each trajectory contains environment observations $o_{t}$, full environment and robot state information $s_{t}$, and robot actions $a_{t}$, i.e., $\tau_i=\{(o_1, s_t, a_1), ..., (o_T, s_T, a_T)\}$, with $T$ being the trajectory length. We obtain these trajectories by teleoperating the simulated robot to complete the task and recording the resulting states, images, and expert actions taken.% 
The first step in the pipeline \idan{need to remove the use of "pipeline" across this section, it is not a pipeline paper anymore} is to use a small number of human demonstrations to train a ``base'' policy that serves as the starting point for RL training. For each task, we collect a dataset of 50 demonstrations in simulation, $\mathcal{D}_{\text{sim}}$. This dataset contains trajectories, e.g., $\mathcal D=\{\tau_1, ..., \tau_N\}$, where each trajectory contains the system states $s_{t}$, and robot actions $a_{t}$, i.e., $\tau_i=\{(s_t, a_1), ..., (s_T, a_T)\}$, with $T$ being the trajectory length. We obtain these trajectories by teleoperating the simulated robot to complete the task.

% we collect two datasets of trajectories, one in simulation $\mathcal{D}_{\text{sim}}$ and $\mathcal{D}_{\text{real}}$. Each dataset contains trajectories, e.g., $\mathcal D=\{\tau_1, ..., \tau_N\}$, where each trajectory contains environment observations $o_{t}$ and robot actions $a_{t}$, i.e., $\tau_i=\{(o_1, a_1), ..., (o_T, a_T)\}$, with $T$ being the trajectory length. We obtain these trajectories via robot teleoperation in both the simulator and the real world.


%\subsection{Imitation Learning}
% Given simulation dataset $\mathcal{D}_{\text{sim}}$,
%
% To train $\pi$, we use Behavior Cloning (BC), i.e., finding parameters $\theta$ that maximize the likelihood of the data, $\underset{\theta}{\text{argmax}}\ \mathbb E_{(a_t,o_t)\sim\mathcal D} \left[\log\pi_\theta(a_t|o_t) \right]$. 

% Given simulation dataset $\mathcal{D}_{\text{sim}}$, we train the base policy $\pi_{\theta}$ with Behavior Cloning (BC), i.e., we optimize $\theta$ to maximize the likelihood of the data, $\text{argmax}_\theta\ \mathbb E_{(a_t,s_t,o_t)\sim\mathcal D} \left[\log\pi_\theta(a_t|o_t, s_t) \right]$.
Using the simulation dataset $\mathcal{D}_{\text{sim}}$, we train the base policy $\pi_{\text{base}}$ with Behavior Cloning (BC), i.e., we maximize the likelihood of the data by optimizing $\max_{\pi}\ \mathbb{E}_{(a_t,s_t)\sim\mathcal{D}_{\text{sim}}} \left[\log\pi(a_t|s_t) \right]$. We use a Diffusion Policy~\cite{chi_diffusion_2023} as the base model, which has shown strong empirical performance in handling difficult manipulation tasks with relatively small datasets~\cite{ankile2024juicer}.
%
Consistent with recent advancements~\cite{chi_diffusion_2023, zhao_rss23_aloha, ankile2024juicer}, our policy framework enhances its performance by predicting multiple future actions in chunks, as opposed to individual actions at each timestep.
We denote the length of future action sequences predicted by the policy as $T_a$, the output as $\actchunk = [a_t, ..., a_{t+T_a}]$. When predicting an action chunk $\actchunk$ of length $T_a$, we only execute a subset $[a_{t},...,a_{t+T_{\text{exec}}}]$, with execution horizon $T_{\text{exec}} \leq T_a$.


\subsection{Online Reinforcement Learning with Residual Policies}

% \lars{I've added some thoughts on the problems of fine-tuning diffusion and other chunked methods -- please take a critical look.}

%With the high precision requirements, initial state randomness, and long horizons of the assembly tasks, it is infeasible to achieve perfect performance from only 50 demonstrations. However, the policies are strong enough to achieve non-zero success rates. Prior work has explored using a converged BC policy to perform more rollouts for successful trajectory dataset expansion~\citep{ankile2024juicer}. We find, however, that performance saturates with this approach, as there is no clear mechanism for \emph{policy improvement} via exploration.

Given the initial base policy $\pi_{\text{base}}$, we aim to improve it using RL. However, directly fine-tuning diffusion models with RL is an active area of research~\cite{fan2023optimizing,fan2023dpok,black2023training,li2024learning_diffusion_pg}, made difficult because of the multi-step inference process and unavailability of the policy action log-probabilities. % of the policy actions.
%
% Other popular BC architectures, like the Action-Chunked Transformer (ACT)~\cite{zhao_rss23_aloha}, could side-step this issue.
%
\iffalse{}
% However, policy gradients with chunks also introduce two effects that can make the optimization harder.
Furthermore, action chunks can also make optimization with policy gradients more difficult.
%
% First, the effective action space increases significantly; for example, a chunk size of 8 increases the dimensions from 10 to 80.
This is partly due to chunking increasing the effective action space (e.g., chunks of 8 actions increase the dimension by $\times$8), which we find to increase RL training instability (see \autoref{sec:experiments-fine-tuning}). %  the effective action space increases significantly; for example, a chunk size of 8 increases the dimensions from 10 to 80.
%
This means fine-tuning other popular BC architectures, like the Action-Chunked Transformer (ACT)~\cite{zhao_rss23_aloha}, also brings technical challenges.
\fi
%
% Second, chunking reduces the resulting environment interactions by the same factor, i.e., an episode of 1000 environment interactions will effectively become $1000 / 8 = 125$.
% Chunking also reduces the resulting environment interactions by the same factor, i.e., an episode of 1000 environment interactions will effectively become $1000 / 8 = 125$.
%
%
% A common way to combine complex policy architectures, like diffusion models or transformers, with RL is to perform offline RL with Q-function-based importance sampling~\cite{hansen-estruch_idql_2023}, do Advantage Weighted Regression~\cite{goo2022know,peng2019advantage}, or change the objective into a supervised learning problem with return conditioning~\cite{chen2021decision,ajay_is_2023,janner_planning_2022}, augmenting the diffusion objective with a Q-function~\cite{wang2022diffusion}, or iteratively changing the dataset with Q-functions~\cite{yang2023policy,li2024learning_diffusion_pg}.
Another category of methods upweight high-quality model outputs via importance sampling, return conditioning, or augmenting the original de-noising objective with a loss term for maximizing a Q-function~\cite{hansen-estruch_idql_2023, goo2022know, chen2021decision, ajay_is_2023, wang2022diffusion}.
%
However, these methods mainly enable better \textit{extraction} of high-quality behavior in the data, while we are more concerned with learning new, \textit{corrective} behaviors.
%
% However, policy gradients with chunks also introduce two effects that can make the optimization harder.
Action chunks can also make optimization with policy gradients more difficult.
%
% First, the effective action space increases significantly; for example, a chunk size of 8 increases the dimensions from 10 to 80.
This is partly due to chunking increasing the effective action space (e.g., chunks of 8 actions increase the dimension 8$\times$), which we find to increase RL training instability (see \autoref{sec:experiments-fine-tuning}). This means fine-tuning other popular BC architectures, like the Action-Chunked Transformer (ACT)~\cite{zhao_rss23_aloha}, also brings technical challenges. \idan{in addition to crrective you need to highlight that it doesn't allow for reactive behavior (to link it to the intro). Also maybe move this discussion to Problem Setup?}
%
Furthermore, recent work has shown that fine-tuning large pre-trained models can lead to forgetting of capabilities if the agent does not visit states seen during pre-training frequently enough~\cite{wolczyk2024fine}. % visits certain states infrequently during online fine-tuning~\cite{wolczyk2024fine}.

% \idan{expand that}
% \anthony{possibility to mention challenges of direct fine-tuning with action chunks, ACTs}

%Therefore, we aim to incorporate sparse ``task success'' reward signals that can be obtained by detecting when two parts of the assembly are brought into their desired relative configuration and use this reward signal to further train the policy to achieve higher success rates than what can be achieved with BC alone.

\input{fig_text/residual_diagram}
%\lars{Other modern architectures are deep and large, making fine-tuning with policy gradients very unstable; we might need a source for this or mention the MLP fine-tuning experiments}.
%We also find that MLP policies that do not employ action-chunking are wholly unable to perform these tasks. This means that direct fine-tuning entails performing policy gradients over whole action chunks. The resulting optimization becomes more difficult and unstable as using action chunks increases the effective action dimension many-fold.
%
We side-step these complications by training a residual Gaussian MLP policy $\pi_{\text{res}}$. This policy takes as input both the system state and the action predicted by the diffusion policy $\pi_{\text{base}}$ and produces an ``action correction'' that modifies the action as $a_{t} = a_{t}^{\text{base}} + \alpha \cdot a_{t}^{\text{res}}$, with $\alpha\leq 1$ being a coefficient controlling what scale the residual policy operates on. \lars{The method is not sensitive to this hyperparameter as shown in \autoref{sec:alpha-ablation}}. We denote the resulting combined policy $\boldsymbol{\pi}$. 
%
This decoupling has several advantages. First, we can regard the diffusion model as a black box and not change its parameters~\cite{silver2018residual}\footnote{This decoupling also implies that the ACT or any other strong BC or offline RL method can straightforwardly serve as the base model without changing anything else in the pipeline, an advantage of residual policy learning emphasized by other prior work in robotics~\cite{silver2018residual,davchev2022residual}.}.
%
This also allows the use of different prediction horizons $T_a$ for the two policies. This flexibility in action horizon is helpful as most RL algorithms optimize single-action policies.
%
% It also removes the need for explicitly regularizing the learned policy to the base policy, which is often necessary to achieve stable optimization~\cite{nair2020awac,rajeswaran2017learning}.
It also removes the need to explicitly regularize the fine-tuned policy to stay near the pre-trained policy, which is often necessary to achieve stable optimization~\cite{nair2020awac,rajeswaran2017learning}.
%
% This decoupling also implies that the ACT or any other strong BC or offline RL method can straightforwardly serve as the base model without changing anything else in the pipeline.
%

Given the above, we train the $\pi_{\text{res}}$ using standard PPO~\cite{schulman_proximal_2017} with the alternation that we augment the state space with the base action. The base model observes the current state $s_t$ and outputs a chunk of actions $\actchunk{}$. For each action in the chunk, we concatenate it with the current observation $s_{t+i}^\text{res}=[s_{t+i},a^\text{base}_{t+i}]$, and predict the correction $a_{t+i}^{\text{res}} \sim \pi^{\text{res}}(\cdot | s_{t+i}^\text{res})$ for $i = 0, ..., T_a - 1$.
%
Besides the technical convenience, one can look at residual policy as a way to incorporate an inductive bias that the policy should only learn \emph{locally} corrective actions~\cite{davchev2022residual}. This is motivated by our qualitative observations that most of the base BC policy failures are due to slight imprecision near ``bottleneck'' transitions when performing skills like grasping and insertion (see %\autoref{fig:bc-failure-rl-success}
\autoref{fig:overview} (A)).



%This approach brings about several advantages:

%\begin{itemize}[leftmargin=*]
    %\myitem This allows us to use different prediction horizon $\actchunk$ for the two policies. This is useful as most RL algorithms are built for $\actchunk=1$.
    %\myitem Training the residual policy with standard policy gradient techniques, e.g., PPO, is much simpler.
    %\myitem We incorporate an inductive bias that the policy should only learn \emph{locally} corrective actions, based on qualitative observations that the majority of the base BC policy failures are due to slight imprecision near ``bottleneck'' transitions when performing skills like grasping and insertion.
    %\myitem It removes the need for an explicit regularization of the learned policy to the base policy, that have been shown necessary to achieve stable optimization~\cite{nair2020awac, rajeswaran2017learning}.
%\end{itemize}


\subsection{Distillation for RGB-based Visual Policy}

\idan{Maybe we should move this to the experiment section where you describe the sim-2-real experiment? it draw the attention from the main method. If the paper is too long it can also just go to the appendix} Once the RL training has converged, the policy exhibits significantly higher success rates than the initial base policy. We aim to distill this enhanced performance from the state-based policy into a vision-based policy that operates solely on RGB images. Following the established teacher-student distillation paradigm~\cite{chen2023visual, lee2020learning, kumar2021rma}, we generate a dataset of successful trajectories, $\mathcal{D}_{\text{synth}}$, where the environment's observations, $o_t$, replace the states, i.e., $\mathcal{D}_{\text{synth}}=\{\tau_{\text{synth},1}, ..., \tau_{\text{synth},N}\}$ and $\tau_{\text{synth},i}=\{(o_1, a_1), ..., (o_T, a_T)\}$. We utilize this dataset to train a final image-conditioned diffusion policy with BC.
%
% \input{fig_text/sim_renders}

For real-world transfer, we enhance the synthetic dataset $\mathcal{D}_{\text{synth}}$ by re-rendering its trajectories in Isaac Sim. This process improves image quality and introduces variability in environmental conditions such as object and table colors, textures, lighting, and camera perspectives, many of which cannot easily be done with standard image augmentation techniques. We denote this refined dataset as $\mathcal{D}_{\text{synth-render}}$.
%
% While directly transferring this vision policy to the real world has been demonstrated in previous simulation-based RL studies~\cite{sim2real_refs}, we encounter significant challenges due to the perceptual domain gap in high-precision tasks from vision.
% While directly transferring this vision policy to the real world has been demonstrated in previous simulation-based RL studies~\cite{sim2real_refs}, we encounter significant challenges due to the perceptual domain gap in high-precision tasks from vision.
%
% To address this, we opt for a co-training approach, integrating the synthetic dataset with a small set of real-world task demonstrations, $\mathcal{D}_{\text{real}}$, which similarly comprises only environmental observations without ground truth poses.
To ease the difficulty of zero-shot sim-to-real with RGB images, we opt for a co-training approach, integrating the synthetic dataset with a small set of real-world task demonstrations, $\mathcal{D}_{\text{real}}$, which similarly comprises only environmental observations without ground truth poses.
%
This combined dataset, $\mathcal{D}_{\text{real}} \cup \mathcal{D}_{\text{synth-render}}$, is used to train the final student policy through BC. While loss reweighting or upsampling may be helpful given the imbalanced dataset sizes, we find that simply mixing the two datasets still provides performance improvement beyond training purely with real data (see Fig.~\ref{tab:real-world-real-cotrain}). % balance b  We find naively mixing the two datasets enables % , even without specific loss reweighting or upsampling schemes. % We experiment with various loss weighting schemes to balance the disparate volumes of simulation and real-world data, ranging from hundreds to thousands of simulated trajectories versus merely tens of real ones. \lars{This is kind of just hanging now -- should we expand on it (we found naively mixing without weighting worked) or maybe axing it?}

==> Archive/old_abstract.tex <==
\begin{abstract}
Behavior cloning (BC) has re-emerged \zw{"re"-emerge reads a bit weird. seems to say it was popular but deprecated at some point and then now come back -- maybe not true? even if it's true, I guess the readers may not have the enough context to grasp the point behind I feel}as a popular approach for teaching robots complex manipulation tasks, with recent innovations enabling learning of long-horizon behaviors from modest numbers of demonstrations. \zw{I was expecting some story about long horizon when seeing this. it's a minor issue but seems distracting me a bit.}
%
However, BC struggles with precise manipulation tasks \zw{"precise" is not defined}, showing performance saturation with increasing expert demonstrations and difficulty in learning to correct mistakes \zw{performance saturation is not clearly defined and also its relationship to precise manipulation is not defined}.
%
Reinforcement learning (RL) can mitigate these limitations by allowing policies to acquire locally corrective behaviors \zw{what does "locally" mean here?} through task reward supervision and exploration.
%
\zw{wait, seems the story is like "taking the best of both world" story  but the limitation of RL is not presented. also I think even if it's not intended to make best of both world story. the wording "re-emerging" still alludes me to think that some alternative (maybe RL) had taken over BC and BC is winning again. Reads a bit incoherent.}
This paper proposes \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation), a simple yet effective scheme to augment state-of-the-art BC models with RL.
%
Our approach involves training residual policies with on-policy RL and sparse task rewards to improve upon pure BC from a handful of demonstrations. \zw{Seems like old recipe. Maybe make readers bored. Cutting to the key insight directly in the abstract.}
%
By keeping the base model frozen during RL training and running the residual policy at a higher frequency \zw{too much details}, we sidestep challenges in fine-tuning modern BC architectures while achieving a more reactive, fully closed-loop policy. \zw{I think the main issue is that these are all old recipes -- starting with BC and finetuning with RL. Combining residual policy for finetuning BC seems new, though not too surprising. Focusing on why residual policy is a good idea to finetune policy is better. Also I will say make the story center around "precision" more. Now it reads like you say precision is a problem for BC, RL can mitigate it, and so you do BC+RL. BC+RL is an old recipe. To make it more exciting, it requires to communicate the trivial combination of BC+RL is not working and one needs your recipe of residual RL. Then say one sentence why residual is better.}
%
Our experimental results demonstrate that this residual learning framework can significantly improve success rates beyond the base BC-trained models in high-precision assembly tasks by learning corrective actions \zw{again, corrective actions seems vague. avoid they if no clear context.}. We also show that by combining \methodname{} with teacher-student distillation and visual domain randomization, our method can enable learning real-world policies for robotic assembly directly from RGB images.
%
Find videos and code at \url{https://residual-assembly.github.io}.
\end{abstract}


\begin{abstract}
\pulkit{Abstract is not updated.}
\lars{Abstract is TBD until the rest of the story is sorted.}
Behavior cloning (BC) is a dominant paradigm for learning real-world visual manipulation. 
%
However, learning robust policies from human demonstrations remains challenging in tasks that require locally corrective behaviors, such as multi-part assembly.
%
Reinforcement learning (RL) can mitigate these limitations by allowing policies to acquire locally corrective behaviors through task reward supervision and exploration.
%
This paper explores using RL fine-tuning to improve BC-trained policies in precise manipulation tasks.
%
We analyze and overcome technical challenges using RL to directly train policy networks incorporating modern architectural components like diffusion models and action chunking.
%
We propose training residual policies on top of frozen BC-trained diffusion models using standard policy gradient methods and sparse rewards, an approach we call \methodname{} (\textit{Resi}dual for \textit{P}recise manipulation).
%
Our experimental results demonstrate that this residual learning framework can significantly improve success rates beyond the base BC-trained models in high-precision assembly tasks by learning corrective actions. We also show that by combining \methodname{} with teacher-student distillation and visual domain randomization, our method can enable learning real-world policies for robotic assembly directly from RGB images.
%
Find videos and code at \url{https://residual-assembly.github.io}.
\end{abstract}

==> Archive/prelim_v1.tex <==
\section{Problem Setup and Approach Overview}


% We wish to propose a generic and scalable pipeline for training robots that do not require immense amounts of human effort.
Our goal is to develop a pipeline that enables robots to perform precise manipulation tasks without requiring massive amounts of manual human effort.
%
% We will demonstrate the usefulness of our pipeline over the task of high-precision multi-step assembly directly from vision.
% We apply our pipeline to the task of multi-step assembly directly from RGB images.
While our pipeline can be applied to many tasks, we focus on applications to the domain of multi-step assembly directly from RGB images.
%
% Here, we detail the specific assumptions of our problem setup and overview the main ideas of the pipeline that we propose. 
Here, we introduce the specific assumptions of our problem setup and detail the main ideas of the pipeline that we propose. 

\paragraph{Assumptions and System Components}

% The pipeline's high-level goal is to synthesize a large dataset of high-quality, successful task trajectories from a policy trained via Reinforcement Learning (RL) and combine this dataset with a small set of real-world demonstrations to train a vision-based manipulation policy able to solve the task with high precision from a diverse set of initial scene layouts.
%
% We assume an assembly task is specified via a mid-sized ($\sim$50-100) set of expert demonstrations.
We assume an assembly task is specified to the robot via a mid-sized ($\sim$50) set of expert demonstrations. The tasks each have an underlying success criterion depending on a set of required alignments between the parts. \idan{This doesn't align with the new story. We should say here again that we want to use human demonstrations for learning robotic manipulation, but scaling it doesn't seem to help (also cite the other paper that shows that). Then say that since it doesn't help, we only require mid-sized set of expert demonstrations.}
%
Each task consists of a fixed set of rigid object parts for which we can access CAD models (either given for an assembly or scanned real-world object). Thus, both the parts and the entire assembly process can be accurately simulated.
%
Each task may have long horizons (up to $\sim$750-1000 steps at 10Hz) and require sequencing of behaviors such as corner alignment, 6-DoF grasping, reorientation, insertion, and screwing.
%
Multi-part assembly interactions are simulated using the SDF-based collision geometry representations featured in the Factory~\cite{narang2022factory} extension of NVIDIA's Isaac Gym simulator.
%
We use the tasks \oneleg{}, \roundtable{}, and \lamp{} from the FurnitureBench~\cite{heo_furniturebench_2023} task suite, the \peghole{} task from~\cite{narang2022factory}, and a self-defined mug-hanging task called \mugrack{}. See detailed descriptions of all tasks in \autoref{app:tasks-and-environment} \lars{Fix the appendix references}.

%
\textbf{Preliminaries}. We formulate the robot's task as a discrete-time sequential decision-making problem. In each time step $t$, the robot receives either an observation $o_{t}\in\mathcal{O}$ if it operates in the real world or the state of the system $s_{t}\in\mathcal{S}$ if it operates in simulation. 
%
After receiving it, the agent produces an action $a_t$ to execute in the environment. % that is being executed.
%
The action space in both simulation and the real world is the desired end-effector pose $\xform{}^{\text{des}} \in$ \sethree{}.
%
We use a differential inverse kinematics controller to convert the desired end-effector pose commands into joint position targets, tracked with a low-level PD controller.  
%
The real world observation space $\mathcal{O}$ contains the robot end-effector pose $\xform{} \in $ \sethree{}, robot end-effector spatial velocity $\mathbf{V} \in \mathbb{R}^{6}$, the gripper width $w_{\text{g}}$, and RGB images from a fixed front-view camera ($I^{\text{front}} \in \mathbb{R}^{h \times w \times 3}$) and a wrist-mounted camera ($I^{\text{wrist}} \in \mathbb{R}^{h \times w \times 3}$), each with unknown camera poses. 
%
In the simulated task variants, the system states space $\mathcal{S}$ contains the same end-effector pose $\xform$, spatial velocity $\mathbf{V}$, and gripper width $w_{\text{g}}$, along with the 6-DoF poses of all the parts in the environment $\{\xform{}^{\text{part}_{i}}\}_{i=1}^{\text{num\_parts}}$. 
%
In addition to the state/observation, the simulated agent receives a binary reward signal from the environment, indicating whether two parts of the assembly have achieved their required geometric alignment.

\paragraph{BC + RL Teacher-Student Distillation Pipeline}
%
\idan{I don't think we need this part any more. It draws focus from the main contribution as we currently present it (way to overcome problems in modern BC) to the sim-to-real part. I would suggest writing a new section here of 1-2 paragraph about our hypothesis on the limitations of modern BC. basically what you said in the introduction but a bit more detailed.}
The pipeline's high-level goal is to leverage a small amount of human demonstrations and the availability of a simulator to develop a vision-based manipulation policy. %This policy aims to achieve high precision in solving tasks from a diverse range of initial scene layouts.
%
To this end, the pipeline consists of two phases:
\begin{itemize}[leftmargin=*]
    \item \textbf{Phase one:} We train an agent to perform the task in a simulated environment using RL. To overcome the need for manual reward engineering, we start with an initial policy pretrained with behavior cloning on a limited set of demonstrations collected in the simulation. We then fine-tune the policy with RL, with only a sparse reward signal provided upon successful task completion.
    \item \textbf{Phase two:} Next, we distill the fine-tuned RL expert policy into a dataset of high-quality RGB image observations and corresponding actions for vision-based policy distillation (using BC). This dataset is combined with a small set of real-world task demonstrations, which helps bridge the simulation-to-reality gap for the final vision-based manipulation policy.
\end{itemize}

% \textbf{Phase one} trains an agent to perform a manipulation task in simulation using RL. Due to the high precision requirements of the task, the high randomness in the initial state distribution, and the long episode lengths, we begin with an initial policy trained with behavior cloning on a small set of demonstrations collected in simulation and use RL to fine-tune it with only supervision from a sparse reward received at successful task completion.
% \textbf{Phase two} then involves distilling the resulting RL policy into a diverse dataset of high-quality RGB image observations and actions. This dataset is then combined with a small number of real-world visual manipulation demonstrations to help overcome the sim2real gap for the final real-world vision-based manipulation policy. We describe the main components and design decisions for each phase in the following sections.
%
%We describe the main components and design decisions for each phase in the following sections.

==> Archive/related.tex <==
\section{Related Works}
\label{sec:related}

\paragraph{Training diffusion models with reinforcement learning}
Recent work has explored various approaches to combining diffusion models with RL~\cite{fan2023optimizing, fan2023dpok, black2023training, li2024learning_diffusion_pg, ren2024diffusion}.
%
The approach in~\cite{black2023training,fan2023dpok} studied how to cast diffusion de-noising as a Markov Decision Process, enabling preference-aligned image generation with policy gradient RL. However, this method is unstable and difficult to tune. \cite{ren2024diffusion} introduced a framework for direct diffusion policy fine-tuning, which avoids this instability, but the method is architecture-specific and does not introduce closed-loop control.
%
Other ways to combine diffusion architectures with RL include Q-function-based importance sampling~\cite{hansen-estruch_idql_2023}, advantage weighted regression~\cite{goo2022know}, or changing the objective into a supervised learning problem with return conditioning~\cite{chen2021decision,ajay_is_2023, janner_planning_2022}. Some have also explored augmenting the de-noising training objective with a Q-function maximization objective~\cite{wang2022diffusion} and iteratively changing the dataset with Q-functions~\cite{yang2023policy}. However, these approaches mainly enable better \textit{extraction} of high-quality behavior already present in the data while we focus on learning new, \textit{corrective} behaviors.
%
Recent work developed techniques for training diffusion policies from scratch~\cite{li2024learning_diffusion_pg}, leveraging unsupervised clustering and Q-learning ensembles to encourage multi-modal behavior discovery.
%
Our method avoids such complexity involved with directly optimizing diffusion models by using standard PPO to train simple residual policies that correct for errors made by the base policy.


Action chunking introduces additional challenges for RL fine-tuning by significantly increasing the effective action space. For example, chunks of 8 actions increase the action dimension 8-fold, increasing training instability. Fine-tuning other popular BC architectures like ACT~\cite{zhao_rss23_aloha} also brings technical challenges~\cite{drolet2024comparison}. Furthermore, recent work has shown that fine-tuning large pre-trained models can lead to forgetting of capabilities if the agent does not visit states seen during pre-training frequently enough~\cite{wolczyk2024fine}. Our method avoids such complexity involved with directly optimizing diffusion models by using standard PPO to train simple residual policies that correct for errors made by the base policy.

\paragraph{Residual learning in robotics}






Learning corrective residual components in conjunction with learned or non-learned ``base'' models has been widely successful in robotics.
%
Common frameworks include learning residual policies that correct for errors made by a nominal behavior policy~\cite{silver2018residual, johannink2019residual, alakuijala2021residual, davchev2022residual, carvalho2022residual, shafiullah2022behavior_bet, haldar2023teach_fish_residual, lee2024behavior_vqbet} and combining learned components to correct for inaccuracies in analytical models for physical dynamics~\cite{ajay2018augmenting, kloss2022combining, zeng2020tossingbot} or sensor observations~\cite{kaufmann2023champion_residual}. Unlike prior residual policy learning approaches, our method uniquely combines RL-based training with running the base at a lower frequency and the residual provides corrections at every control step.
%
Residual policies have been used in insertion applications~\cite{schoettler2020deep_residual_insertion}, and recent work has applied residual policy learning to the same FurnitureBench task suite we study in this paper~\cite{jiang2024transic_assembly}. Their approach uses the residual component to model online human-provided corrections via supervised learning, whereas we train our residual policy from scratch with RL using task rewards in simulation.

\iffalse{}
\paragraph{Learning Robotic Assembly Skills}
Robotic assembly has been used by many as a problem setting for various behavior learning techniques~\cite{tang2023industreal, zhang2022learning_assembly, davchev2022residual, spector2021insertionnet1, tian2023asap}. Enabling robot assembly that captures multi-skill sequencing (e.g., fixturing $\rightarrow$ grasping $\rightarrow$ insertion $\rightarrow$ screwing) directly from RGB images has remained challenging.
% \emph{without} explicitly defining sub-skill boundaries and while operating  from imitation and rein is a longstanding application area that 
% FurnitureBench~\cite{heo_furniturebench_2023}, others using furniture bench~\cite{jiang2024transic_assembly}.
% Factory~\cite{narang2022factory}. IndustREAL~\cite{tang2023industreal}. ASAP and others~\cite{tian2023asap, tian2022assemble_them_all, zakka2020form2fit}. Others~\cite{zhang2022learning_assembly, spector2021insertionnet1, spector2022insertionnet2}.
% Functional Manipulation Benchmark (FMB)? \cite{luo2024fmb}
\fi

\iffalse{}
\paragraph{Complementary combinations of behavior cloning and reinforcement learning}
Various combinations of learning from demonstrations/behavior cloning and reinforcement learning have begun maturing into standard tools in the learning-based control development paradigm~\cite{lu2022aw_opt, Rajeswaran-RSS-18_dapg}. 
%
For instance, demonstrations are often used to support RL in overcoming exploration difficulty and improving sample efficiency~\cite{hu_imitation_2023_bootstrapped, torne2024reconciling_rialto, luo_serl_2024}. RL can also act as a robustification operator to improve upon base BC behaviors~\cite{lu2022aw_opt, torne2024reconciling_rialto}, paralleling the RL fine-tuning paradigm that has powered much of the recent advancement in other areas like NLP~\cite{llm_fine_tuning} and vision~\cite{black_training_nodate}.
%
Additionally, many successful robotics deployments~\cite{chen2023visual, lee2020learning, kumar2021rma} have been powered by the ``teacher-student distillation'' paradigm, wherein perception-based ``student'' policies are trained to clone behaviors produced by a state-based ``teacher'' policy, which is typically trained via RL in simulation.
%
We demonstrate that our residual RL approach for fine-tuning modern diffusion policy architectures can allow each of these complementary ways to combine BC and RL to come together and enable precise manipulation directly from RGB images.
\fi


